Nearest Neighbor Classifiers over Incomplete Information: From Certain Answers to Certain Predictions

Machine learning (ML) applications have been thriving recently, largely attributed to the increasing availability of data. However, inconsistency and incomplete information are ubiquitous in real-world datasets, and their impact on ML applications remains elusive. In this paper, we present a formal study of this impact by extending the notion of Certain Answers for Codd tables, which has been explored by the database research community for decades, into the field of machine learning. Specifically, we focus on classification problems and propose the notion of "Certain Predictions" (CP) -- a test data example can be certainly predicted (CP'ed) if all possible classifiers trained on top of all possible worlds induced by the incompleteness of data would yield the same prediction. We study two fundamental CP queries: (Q1) checking query that determines whether a data example can be CP'ed; and (Q2) counting query that computes the number of classifiers that support a particular prediction (i.e., label). Given that general solutions to CP queries are, not surprisingly, hard without assumption over the type of classifier, we further present a case study in the context of nearest neighbor (NN) classifiers, where efficient solutions to CP queries can be developed -- we show that it is possible to answer both queries in linear or polynomial time over exponentially many possible worlds. We demonstrate one example use case of CP in the important application of "data cleaning for machine learning (DC for ML)." We show that our proposed CPClean approach built based on CP can often significantly outperform existing techniques in terms of classification accuracy with mild manual cleaning effort.

==> [arXiv] Certain Prediction/Algorithms.tex <==

\begin{figure}[t!]
\centering
%\scriptsize
\small
\begin{tabular}{cccccc}
\hline
$K$ & $|\mathcal{Y}|$ & Query & Alg. & Complexity
in $O(-)$&  Section \\
\hline 
1 & 2 & Q1/Q2 & SS & $NM \log NM$ &  3.1.2 \\
$K$ & 2 & Q1 & MM & $NM$ &  3.2 \\
$K$ & $|\mathcal{Y}|$ & Q1/Q2 & SS & $NM (\log(NM) +  K\update{^2} \log N$) &  3.1.3 \\
\hline
\end{tabular}
\vspace{-0.5em}
\caption{Summary of results ($K$ and $|\mathcal{Y}|$ are constants).
}
\label{fig:summary_of_result}
\end{figure}

% !TEX root = CC.tex
%\section{Answering CP Queries for KNN}\label{sec:cc-knn}
\section{Efficient Solutions for CP Queries}\label{sec:cc-knn}

%\textcolor{red}{Xu: some suggestions: (1) for Q1, only introduce MinMax, no need to differentiate between K = 1 and K > 1; (2) for Q2, introduce the SortScan based algorithm for counting; (3) need graphics and better flow in introducing the technical details; (4) I suggest move Q3 to a standalone section}

% The challenge in searching for general exact solutions to CC queries leads us to instead look into specific classifiers.
% In this section, we provide such a case study by focusing on $K$-NN classifiers, which have been widely used in various applications.

Given our definition of certain prediction,
not surprisingly, both queries are  
hard if we do not assume any structure
of the classifier. In this section, we 
focus on a specific classifier that is
popularly used in practice, namely the 
$K$-Nearest Neighbor (KNN) classifier.
As we will see, for a KNN classifier,
we are able to answer both CP queries
in \textit{polynomial} time, even though we are
reasoning over \textit{exponentially} many
possible worlds!


\vspace{0.5em}
\noindent
{\bf \emph{$K$-Nearest Neighbor Classifiers.}} 
A textbook KNN classifier works in the following way, as illustrated in 
Figure~\ref{fig:knn-similarity}(a): Given a training set 
$D = \{(x_i, y_i)\}$ and a test example 
$t$, we first calculate the similarity
between $t$ and each $x_i$: $s_i =  \kappa(x_i, t)$.
This similarity can be calculated 
using different kernel functions $\kappa$
such as linear kernel, RBF kernel, etc.
Given all these similarity scores
$\{s_i\}$, we pick the top $K$ training
examples with the largest similarity score:
$x_{\sigma_1}, ..., x_{\sigma_K}$
along with corresponding labels
$\{y_{\sigma_i}\}_{i\in[K]}$.
We then take the majority 
label among $\{y_{\sigma_i}\}_{i\in[K]}$ and return 
it as the prediction for the test example
$t$.

%For regular training datasets, the $K$-NN classifier takes each data point $x_i$ and computes a similarity score based on some kernel function $\kappa : \mathcal{X} \times \mathcal{X} \rightarrow \mathbb{R}$ between every $x_i \in D$ and the test example $x_t$, producing a similarity vector $s \subset \mathbb{R}^N$ defined as $s = [\kappa(x_i, x_t)]_i$. When predicting the label for $x_t$, the $K$-NN classifier simply selects a subset of $K$ data points with the highest similarity score. The most frequently occurring label among those top $K$ data points is returned as the predicted label.

\vspace{0.5em}
\noindent
{\bf \emph{Summary of Results.}} 
In this paper, we focus on designing
efficient algorithms to support a KNN
classifier for both CP queries.
In general, all these results 
are based on two algorithms,
namely SS (SortScan) and MM (MinMax).
SS is a generic algorithm that
can be used to answer 
both queries, while MM can only be used
to answer $Q1$. However, on the other
hand, MM permits lower complexity 
than SS when applicable.
Figure~\ref{fig:summary_of_result} summarizes the result.

\vspace{0.5em}
\noindent
{\bf \emph{Structure of This Section.}} 
In Section~\ref{sec:ss}
we will focus on the SS 
algorithm as it is more 
generic. We will
explain a simplified version
of the SS algorithm for 
the special case ($K=1$, $|\mathcal{Y}|=2$)
in greater details as it conveys
the intuition behind this algorithm.
We will follow by describing the
SS algorithm in its general form.
We will summarize the
MM algorithm
in Section~\ref{sec:mm}, which
can be significantly more efficient than SS
in some cases, but leave
the full details to the appendix.
%\ww{We perhaps can move Section 3.2 to the appendix and give a very short summary of MM after Section 3.1.}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/\figfmt/knn-similarity-s}
    % \vspace{-1.5em}
    \caption{Illustration of KNN classifiers.}
    \label{fig:knn-similarity}
\end{figure}

\subsection{SS Algorithm}\label{sec:ss}

We now describe the SS algorithm.
The idea behind SS is that we can calculate
the similarity between all
candidates $\cup_i \mathcal{C}_i$ in an incomplete 
dataset and a test example $t$.
Without loss of generaility,
assume that $|\mathcal{C}_i| = M$, this leads to $N \times M$
similarity scores $s_{i, j}$.
We can then sort and scan these
similarity scores.
%and scan it 
%from the least similar scores
%to the most similar scores.

The core of the SS algorithm
is a dynamic programming 
procedure. 
We will first describe 
a set of basic building blocks of this problem, and
then introduce
a simplified version of SS
for the special case of
$K=1$ and $|\mathcal{Y}|=2$, to explain the
intuition behind SS.
We follow this by the general version of the SS algorithm.

\subsubsection{Two Building Blocks} \label{sec:alg:ss:two-building-blocks}

In our problem, we can construct two 
building blocks efficiently. We start by
articulating the settings precisely.
In the next section, we will use these
two building blocks for our SS algorithm.

%and 
%then introduce these two building blocks.
%In the next section, we will use these
%building blocks for our SS algorithm.

\paragraph*{Setup} We are given 
an incomplete dataset $\mathcal{D}=\{(\mathcal{C}_i, y_i)\}$.
Without loss of generality, we 
assume that each $\mathcal{C}_i$
only contains $M$ elements, i.e.,
$|\mathcal{C}_i| = M$.
We call $\mathcal{C}_i = \{x_{i,j}\}_{j \in [M]}$ the 
$i^{th}$ incomplete data example, and $x_{i, j}$
the $j^{th}$ candidate value 
for the $i^{th}$ incomplete data example.
This defines $M^N$ many possible worlds:
\[
\mathcal{I}_{\mathcal{D}} = \{D=\{(x_i^D, y_i^D)\}: 
 |D| = |\mathcal{D}| \wedge 
 y_i^D = y_i \wedge x_i^D \in \mathcal{C}_i
 \}.
\]
% We assume that
% a possible world $D$ would pick $x_{i, j_{i, D}}$
% for the $i^{th}$ data point.
We use $x_{i, j_{i, D}}$ to denote the candidate value for the $i^{th}$ data point in $D$.
Given a test example $t$, we can calculate the
similarity between each candidate value $x_{i, j}$
and $t$: $s_{i, j} = \kappa(x_{i, j}, t)$. We
call these values \textit{similarity candidates}, as shown in Figure~\ref{fig:knn-similarity} (b). We assume that
there are no ties in these similarities scores (we can always break a tie by favoring a smaller
$i$ and $j$ or a pre-defined random order).

Furthermore, given a candidate value $x_{i, j}$, we 
count, for each candidate set, how many 
candidate values are less similar to the 
test example than $x_{i, j}$. This gives
us what we call the 
{\em similarity tally} $\alpha$.
For each candidate set $\mathcal{C}_n$,
we have
\[
\alpha_{i, j}[n] = \sum\nolimits_{m=1}^M \mathbb{I}[s_{n, m} \leq s_{i, j}].
\] 

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/\figfmt/alg-sort-count-k1-s}
    % \vspace{-1.5em}
    \caption{Illustration of SS when $K=1$ for $Q2$.}
    \label{fig:alg-sort-count-k1}
\end{figure}


\begin{example} 
In Figure~\ref{fig:alg-sort-count-k1} we can see an example of a similarity tally $\alpha_{2,2}$ with respect to the data point $x_{2,2}$. For 
$i^{th}$ incomplete
data example, it contains the number of candidate values $x_{i,j} \in \mathcal{C}_i$ that have the similarity value no greater than $s_{2,2}$. Visually, in Figure~\ref{fig:alg-sort-count-k1}, this represents all the candidates that lie left of the vertical yellow line. We can see that only one candidate from $\mathcal{C}_{1}$, two candidates from $\mathcal{C}_{2}$, and none of the candidates from $\mathcal{C}_{3}$ satisfy this property. This gives us $\alpha_{2,2}[1]=1$, $\alpha_{2,2}[2]=2$, and $\alpha_{2,2}[3]=0$.
\end{example}

\paragraph*{KNN over Possible World $D$}
Given one possible world $D$, running a KNN classifier
to get the prediction for a test example $t$ 
involves multiple stages. 
First, we obtain
{\em Top-K Set}, the set of $K$ examples in $D$
that are in the K-nearest neighbor set
\[
Top(K, D, t) \subseteq [N],
\]
which has the following property
\[
|Top(K, D, t)| = K,
\]
\begin{eqnarray*}
\forall i, i' \in [N].~~~i \in Top(K, D, t) \wedge i' \not
\in Top(K, D, t) 
\implies  s_{i, j_{i, D}} > s_{i', j_{i', D}}.
\end{eqnarray*}

Given the top-K set, we then tally the corresponding
labels by counting how many 
examples in the top-K set support a given label.
We call it the {\em label tally} $\gamma^D$:
\[
\gamma^D \in \mathbb{N}^{|\mathcal{Y}|}: \gamma_l^D = 
    \sum\nolimits_{i \in Top(K, D, t)} \mathbb{I}[l = y_i].
\]
Finally, we pick the label with the largest
count:
\[
y^*_D = \arg\max_l \gamma_l^D.
\]

\begin{example}
For $K=1$, the Top-K Set contains only one element $x_i$ which is most similar to $t$. The label tally then is a $|\mathcal{Y}|$-dimensional binary vector with all elements being equal to zero except for the element corresponding to the label $y_i$ being equal to one. Clearly, there are $|\mathcal{Y}|$ possible such label tally vectors.
%The label that is predicted by voting is also trivially equal to $y_i$.
\end{example}

\paragraph*{Building Block 1: Boundary Set}
The first building block answers the 
following question: {\em 
Out of all possible worlds that picked 
the value $x_{i, j}$ for $\mathcal{C}_i$,
how many of them have $x_{i,j}$ as the
least similar item in the Top-K set?}
We call all possible worlds that satisfy
this condition the {\em Boundary Set}
of $x_{i, j}$:
\begin{equation*}
BSet(i, j; K)  = 
\{D: j_{i, D} = j \wedge i \in Top(K, D, t)
\wedge 
     i \not \in Top(K-1, D, t) \}.  
\end{equation*}
We call the size of the boundary 
set the {\em Boundary Count}.

We can enumerate all $N \choose (K - 1)$ 
possible configurations of the top-(K-1)
set to compute the boundary count.
Specifically, let $\mathcal{S}(K-1, [N])$ be 
all subsets of $[N]$ with size $K-1$. We have 
\[
|BSet(i, j; K)| = \sum_{\substack{S \in \mathcal{S}(K-1, [N]) \\
                i \not \in S}}
    \left(\prod_{n \not \in S} \alpha_{i, j}[n]\right) 
    \cdot 
    \left(\prod_{n \in S} (M - \alpha_{i, j}[n])\right).
\] 

The idea behind this is the following --- we
enumerate all possible settings of the
top-(K-1) set: $\mathcal{S}(K-1, [N])$.
For each specific top-(K-1)
setting $S$, every candidate set in 
$S$ needs to pick a value that is
more similar than $x_{i, j}$, while
every candidate set not in $S$ needs
to pick a value that is less similar
than $x_{i, j}$. Since the choices of
value between different candidate sets
are independent, we can calculate 
this by multiplying different entries of 
the similarity tally vector $\alpha$.

We observe that calculating the 
boundary count for a value $x_{i, j}$
can be efficient when $K$ is small.
For example, if we use a 1-NN
classifier, the only $S$ that we 
consider is the empty set, and thus, 
the boundary count merely
equals $\prod_{n \in [N], n \ne i} \alpha_{i, j}[n]$.

\begin{example}
We can see this, in Figure~\ref{fig:alg-sort-count-k1} from Step 3 to Step 4,  where the size of the boundary set $|BSet(2, 2; 1)|$ is computed as the product over elements of $\alpha$, excluding $\alpha[2]$. Here, the boundary set for $x_{2,2}$ is actually empty. This happens because both candidates from $\mathcal{C}_3$ are more similar to $t$ than $x_{2,2}$ is, that is, $\alpha_{2,2}[3]=0$. Consequently, since every possible world must contain one element from $\mathcal{C}_3$, we can see that $x_{2,2}$ will never be in the Top-$1$, which is why its boundary set contains zero elements.

If we had tried to construct the boundary set for $x_{3,1}$, we would have seen that it contains two possible worlds. One contains $x_{2,1}$ and the other contains $x_{2,2}$, because both are less similar to $t$ than $x_{3,1}$ is, so they cannot interfere with its Top-$1$ position. On the other hand, both possible worlds have to contain $x_{1,1}$ because selecting $x_{1,2}$ would prevent $x_{3,1}$ from being the Top-$1$ example.
\end{example}


\paragraph*{Building Block 2: Label Support}
To get the prediction of a KNN classifier,
we can reason about the label tally vector 
$\gamma$, and not necessarily the specific 
configurations of the top-K set.
It answers the following question:
{\em 
Given a specific configuration of the 
label tally vector $\gamma$, how many
possible worlds in the boundary set of
$x_{i,j}$ support this $\gamma$?
}
We call this the {\em Support} of the
label tally vector $\gamma$:
\[
Support(i, j, \gamma) = |\{D: \gamma^D = \gamma \wedge 
D \in BSet(i, j; K)\}|.
\]

\begin{example}
For example, when $K=3$ and $|\mathcal{Y}|=2$, we have $4$ possible label tallies: $\gamma \in \{ [0,3], [1,2], [2,1], [3,0] \}$. Each tally defines a distinct partition of the boundary set of $x_{i,j}$ and the size of this partition is the support for that tally. Note that one of these tallies 
always has support 0,
which happens when $\gamma_l = 0$ for the label $l=y_i$, thus excluding $x_{i,j}$ from the top-$K$ set. 

For $K=1$, a label tally can only have one non-zero value that is equal to $1$ only for a single label $l$. Therefore, all the elements in the boundary set of $x_{i,j}$ can support only one label tally vector that has $\gamma_l=1$ where $l=y_{i}$. 
This label tally 
vector will always have
the support equal 
to the boundary count of $x_{i,j}$.
\end{example}

% \update{
% The situation gets more interesting when $K > 1$. Here each element of $\gamma_l^D$ can take any value between $0$ and $K$, as long all elements of $\gamma^D$ sum up to $K$. 
% }

% \update{
% For example the tally $[1,2]$ contains all possible worlds from the boundary set of $x_{i,j}$ with exactly $1$ example with label $0$ in the top-$K$ and exactly $2$ such examples with label $1$. We can decompose the computation of the support for this tally by partitioning all examples $x_i \in D$ based on their label $y_i$, compute the label support for both labels $0$ and $1$ individually, and then multiply them together.
% }

Calculating the support can be done with 
dynamic programming. First,
we can partition the whole incomplete
dataset into $|\mathcal{Y}|$ many 
subsets, each of which only contains
incomplete data points
(candidate sets) of the same label $l \in |\mathcal{Y}|$:
\[
\mathcal{D}_l = \{(\mathcal{C}_i, y_i): y_i = l \wedge 
(\mathcal{C}_i, y_i) \in \mathcal{D}\}.
\]
Clearly, if we want a possible world $D$ that
supports the label tally vector $\gamma$, 
its top-K set needs to have 
$\gamma_1$ candidate sets from $\mathcal{D}_1$,
$\gamma_2$ candidate sets from $\mathcal{D}_2$,
and so on.
{\em 
Given that $x_{i, j}$ is on the boundry, how many 
ways do we have to pick 
$\gamma_l$ many candidate sets from $\mathcal{D}_l$
in the top-K set?} We can represent this value
as $C^{i, j}_l(\gamma_l, N)$, with the following 
recursive structure:
\begin{equation*}
C_l^{i, j}(c,n) =
\begin{cases}
C^{i, j}_l(c, n-1), \quad \text{if} \ y_n \neq l, \\
\update{C^{i, j}_l(c-1, n-1), \quad \text{if} \ x_n=x_i}, \text{otherwise} \\
\alpha_{i, j}[n] \cdot C^{i, j}_l(c, n-1) + (M-\alpha_{i, j}[n]) \cdot C^{i, j}_l(c-1,n-1).
\end{cases}    
\end{equation*}
This recursion defines a process in which one
scans all candidate sets from $(\mathcal{C}_1, y_1)$ 
to $(\mathcal{C}_N, y_N)$.
At candidate set $(\mathcal{C}_n, y_n)$:
\begin{enumerate}
\item If $y_n$ is not equal to our target label $l$,
the candidate set $(\mathcal{C}_n, y_n)$ will 
not have any impact on the count.
\item If $x_n$ happens to be $x_i$, this will 
not have any impact on the count as 
$x_i$ is always in the top-K set, by definition. \update{However, this means that we have to decrement the number of available slots $c$.}
\item Otherwise, we have two choices to make:
\begin{enumerate}
\item Put $(\mathcal{C}_n, y_n)$ into the
top-K set, and there are $(M - \alpha_{i, j}[n])$
many possible candidates to choose from.
\item Do not put $(\mathcal{C}_n, y_n)$ into the
top-K set, and there are $\alpha_{i, j}[n]$
many possible candidates to choose from.
\end{enumerate}
\end{enumerate}

It is clear that this recursion can be 
computed as a dynamic program in $\mathcal{O}(N \cdot M)$ time. This DP is defined for $c \in \{0...K\}$ which is the exact number of candidates we want to have in the top-$K$, and $n \in \{1...N\}$ which defines the subset of examples $x_i : i \in \{1...N\}$ we are considering. The boundary conditions of this DP are $C_l^{i, j}(-1,n)=0$ and $C_l^{i, j}(c,\update{0})=1$.

Given the result of this dynamic programming 
algorithm for different values of $l$, we 
can calculate the support of label tally
$\gamma$:
\[
Support(i, j, \gamma) = \prod\nolimits_{l \in \mathcal{Y}}
C_{l}^{i, j}(\gamma_l, N),
\]
which can be computed in $\mathcal{O}(NM|\mathcal{Y}|)$.
%\update{We use the indicator function $\mathbb{I}[\gamma_{y_i} \geq 1]$ to ensure that the tally vector $\gamma$ accounted for at least one instance of label $l=y_i$ in the top-$K$.}

\begin{example}
If we assume the situation shown in Figure~\ref{fig:alg-sort-count-k1}, we can try for example to compute the value of $Support(3,1,\gamma)$ where $\gamma=[1,0]$. 
We would have $C_0^{3,1}(1,N)=1$ because $x_{3}$ (the subset of $D$ with label 0) must be in the top-$K$, which happens only when $x_3=x_{3,1}$. On the other hand we would have $C_1^{3,1}(0,N)=2$ because both $x_{1}$ and $x_{2}$ (the subset of $D$ with label 1) must be out of the top-$K$, which happens when $x_1=x_{1,1}$ while $x_2$ can be either  equal to $x_{2,1}$ or $x_{2,2}$. Their mutual product is equal to $2$, which we can see below the tally column under $x_{3,1}$.
\end{example}

\subsubsection{$K=1$, $|\mathcal{Y}|=2$}

Given the above two building blocks, 
it is easy to develop an algorithm 
for the case $K=1$ and $|\mathcal{Y}|=2$.
In SS, we use the result of $Q2$ 
to answer both $Q1$ and $Q2$. Later we will
introduce the MM algorithm that is dedicated to
$Q1$ only.

We simply compute the number of possible 
worlds that support the prediction label being 1.
We do this by enumerating all possible 
candidate values $x_{i, j}$. If this 
candidate has label $y_i = 1$, we count
how many possible worlds have 
$x_{i, j}$ as the top-1 example, i.e.,
the boundry count of $x_{i, j}$.
We have
\[
Q2(\mathcal{D}, t, l) = \sum_{i \in [N]}
\sum_{j \in [M]} \mathbb{I}[y_i = l] \cdot |BSet(i, j; K=1)|, 
\]
which simplifies to 
\[
Q2(\mathcal{D}, t, l) = \sum_{i \in [N]}
\sum_{j \in [M]} \mathbb{I}[y_i = l] \cdot \prod_{n \in [N], n \ne i} \alpha_{i, j}[n].
\]

If we pre-compute the whole
$\alpha$ matrix, it is clear that 
a naive implementation would calculate the above value 
in $\mathcal{O}(N^2M)$.
However,
as we will see later, we can do much better.


%\begin{figure}
%    \centering
%    \includegraphics[width=1.0\columnwidth]{Figures/png/knn-similarity-extended}
%    \vspace{-1.5em}
%    \caption{Example of the basic procedures used for answering Q1 and Q2 for KNN classifiers.}
%    \label{fig:knn-similarity-extended}
%\end{figure}




\paragraph*{Efficient Implementation}
We can design a much more efficient 
algorithm to calculate this value.
The idea is to first sort all
$x_{i, j}$ pairs by their similarity
to $t$, $s_{i, j}$, from the smallest to the largest, and then scan them in this order.
%in the order of least similar 
%to most similar. 
In this way, we
can incrementally maintain the 
$\alpha_{i, j}$ vector during the scan.

Let $(i, j)$ be the current candidate 
value being scanned, and 
$(i', j')$ be the candidate 
value right before $(i, j)$ in the sort order, we have
\begin{equation}
\label{eqn:alpha}
\begin{split}
\alpha_{i, j}[n] & = \begin{cases}
\alpha_{i', j'}[n] + 1~~~~\text{if}~n = i', \\
\alpha_{i', j'}[n]. 
\end{cases}    
\end{split}
\end{equation}
Therefore, we are able to 
compute, for each $(i, j)$, its
\begin{equation}
\label{eqn:alphaprod}
\prod\nolimits_{n \in [N], n \ne i} \alpha_{i, j}[n]   
\end{equation}
in $\mathcal{O}(1)$ time, {\em without
pre-computing the whole $\alpha$.}
This will give us an algorithm 
with complexity $\mathcal{O}(MN\log MN)$!

\begin{example}
In Figure~\ref{fig:alg-sort-count-k1} we depict exactly this algorithm. We iterate over the candidates $x_{i,j}$ in
an order of increasing similarity with the test example $t$ (Step 1). In each iteration we try to compute the number of possible worlds supporting $x_{i,j}$ to be the top-$1$ data point (Step 2). We update the tally vector $\alpha$ according to Equation~\ref{eqn:alpha} (Step 3) and multiply its elements according to Equation~\ref{eqn:alphaprod} (Step 4) to obtain the boundary cont. Since $K=1$, the label support for the label $l=y_i$ is trivially equal to the boundary count and zero for $l \neq y_i$ (Step 5). We can see that the label $0$ is supported by $2$ possible worlds when $x_3=x_{3,1}$ and $4$ possible worlds when $x_3=x_{3,2}$. On the other hand, label $1$ has non-zero support only when $x_1=x_{1,2}$. Finally, the number of possible worlds that will predict label $l$ is obtained by summing up all the label supports in each iteration where $l=y_i$ (Step 6). For label $0$ this number is $2+4=6$, and for label $1$ it is $0+0+0+2=2$.
\end{example}

%Figure~\ref{fig:alg-sort-count-k1}
%illustrates this algorithm. 
%We will provide the algorithm for the more general
%case in the next section. 
%\xc{This Figure does not seem to reflect the text, may have been created based on previous description. Also, a description of the figure should be added.}

\subsubsection{$K \geq 1$, $|\mathcal{Y}| \geq 2$}

In the general case, the algorithm follows a 
similar intuition as the case of
$K = 1$ and $|\mathcal{Y}| = 2$. 
We enumerate each possible candidate value
$x_{i, j}$. For each candidate value,
we enumerate all possible values of the
label tally vector; for each such vector,
we compute its support. 
Let $\Gamma$ be the set of all possible 
label tally vectors, we have
\[
Q2(\mathcal{D}, t, l) =
   \sum_{i \in [N]} \sum_{j \in [M]}
   \sum_{\gamma \in \Gamma}
     \mathbb{I}[l = \argmax(\gamma)] 
     \cdot    
     Support (i, j, \gamma).
\]
We know that there are $|\Gamma| = \mathcal{O}\left({|\mathcal{Y}|+K-1 \choose K}\right)$
many possible configurations of the label 
tally vector, and for each of them,
we can compute the support 
$Support (i, j, \gamma)$ in $\mathcal{O}(NM|\mathcal{Y}|)$
time. As a result, a naive implementation of
the above algorithm would take 
$\mathcal{O}(N^2M^2|\mathcal{Y}|{|\mathcal{Y}|+K-1 \choose K})$ time.

\begin{algorithm}[t!]
\small
\caption{Algorithm \textbf{SS} for Answering Q2 with $K$-NN.} \label{alg:sort-count:dp:binary}
\label{alg:q2}
\begin{algorithmic}[1]
\REQUIRE {$\mathcal{D}$, incomplete dataset; $t$, target data point.}
\ENSURE {$r$, integer vector, s.t. $r[y]=Q2(\mathcal{D}, t, y), \forall y \in \mathcal{Y}$.}

\STATE $s \gets \mathtt{kernel} (\mathcal{D}, t)$;
\STATE $\alpha \gets \emph{zeros}(|\mathcal{D}|)$;
\STATE $r \gets \emph{zeros}(|\mathcal{Y}|)$;
%
\FORALL{$(i,j) \in \mathtt{argsort}(s)$}
    \STATE $\alpha[i] \gets \alpha[i] + 1$; ~~~~~// (See Equation~(\ref{eqn:alpha}))
    
    \FORALL{$l \in \mathcal{Y}$}
        \FORALL{$k \in [K]$}
        \STATE Compute $C^{i, j}_l(k, N)$.
        \ENDFOR
    \ENDFOR
    
    \FORALL{possible valid tally vectors $\gamma \in \Gamma$}
        \STATE $y_p \gets \mathtt{argmax} (\gamma)$;
        \STATE Compute 
        $Support(i, j, \gamma) = \mathbb{I}[\gamma_{y_i} \geq 1] \cdot \prod_{l \in \mathcal{Y}}C^{i, j}_l(\gamma_l, N)$;
        \STATE $r[y_p] \gets r[y_p] + Support(i, j, \gamma)$;
    \ENDFOR

\ENDFOR

\RETURN $r$;
\end{algorithmic}
\end{algorithm}


\paragraph*{Efficient Implementation}
We can implement the above procedure in a 
more efficient way, as illustrated in 
Algorithm~\ref{alg:q2}.
Similar to the case of $K=1$, we
iterate over all values $x_{i, j}$ in 
the order of increasing similarity (line 4). 
This way, we are able to maintain, efficiently,
the similarity tally vector $\alpha_{i, j}$ 
(line 5).
We then pre-compute the result of 
$K|\mathcal{Y}|$ many dynamic programming
procedures (lines 6-8), which will be used to
compute the support for each possible
tally vector later. 
We iterate over all valid label tally vectors, where a valid tally vector 
$\gamma \in \Gamma$ contains all integer vectors 
whose entries sum up to $K$ (line 9).
For each tally vector, we
get its prediction $y_p$ (line 10).
We then calculate its support (line 11) and
add it to the number of possible worlds
with $y_p$ as the prediction (line 12).


\vspace{0.5em}
\noindent
\textbf{(Complexity)}
We analyze the complexity of Algorithm~\ref{alg:q2}:
\begin{itemize}
\item The sorting procedure requires $\mathcal{O} (N \cdot M \log N \cdot M)$ steps as it sorts all elements of $S$.
\item The outer loop iterates over $\mathcal{O} (N \cdot M)$ elements.
\item In each inner iteration, we need to compute $|\mathcal{Y}|$
sets of dynamic programs, each of which
has a combined state space of size $N \cdot K$.
\item Furthermore, in each iteration, we iterate over all possible label assignments, which requires $\mathcal{O}\left({|\mathcal{Y}|+K-1 \choose K}\right)$ operations. 
%For small $|\mathcal{Y}|$ we can consider this to be a relatively small quantity. For binary classification problems where $|\mathcal{Y}|=2$, this reduces to $\mathcal{O}(K)$.
\item For each label assignment, we need $\mathcal{O}(|\mathcal{Y}|)$ multiplications.
\end{itemize}
The time complexity is therefore the sum of $\mathcal{O} (N \cdot M \log (N \cdot M))$ and $\mathcal{O} (N \cdot M \cdot (N \cdot K + |\mathcal{Y}| + {|\mathcal{Y}|+K-1 \choose K}))$. 

\paragraph*{Further Optimizations}
We can make this even faster by observing that: (1) all the states relevant for each iteration of the outer loop are stored in $\alpha$, and (2) between two iterations, only one element of $\alpha$ is updated. We can take advantage of these observations to reduce the cost of computing the dynamic program by employing 
divide-and-conquer. We recursively divide the elements of $\alpha$ into two subsets and maintain the DP result for each subset. The joint result for the two subsets is obtained by a simple sum-of-products formula with $O(K)$ complexity. We can see that this enables us to maintain a binary tree structure of DP results and in each iteration we need to update $O(\log N)$ elements. This enables us to compute the dynamic program in $O(K \log N)$ instead of $O(KN)$ time, which renders the overall complexity as $\mathcal{O} (N \cdot M \cdot (\log(N\cdot M) +  K\update{^2} \cdot \log N ))$. 
We leave the details for the appendix.




\subsection{MM Algorithm}\label{sec:mm}

One can do significantly better for $Q_1$ in certain cases.
Instead of using the SS algorithm, we can develop an algorithm that deals with the binary 
classification case ($|\mathcal{Y}|=2$) with time complexity
$\mathcal{O} \left(N \cdot M + (N \log K + K) \right)$. 

This algorithm, illustrated in Figure~\ref{fig:alg-min-max-k1}, relies on a key observation that for each label $l$, we can greedily construct a possible world that has the best chance of predicting label $l$. We call this possible world the $l$-extreme world and construct it by selecting from each candidate set $\mathcal{C}_i$ either the candidate most similar to the test example $t$ when $y_i=l$, or the candidate least similar to $t$ when $y_i \neq l$. We can show
that the $l$-extreme world predicts label $l$
if and only if there exists a possible world that predicts label $l$.
This means we can use it as a condition for checking the possibility of predicting label $l$. Since the construction of the $l$-extreme world can be done in $\mathcal{O} \left(N \cdot M \right)$ time, this leads us to a efficient algorithm for $Q1$.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/\figfmt/alg-min-max-k1}
    % \vspace{-1.5em}
    \caption{Illustration of MM when $K=1$ for $Q1$.}
    \label{fig:alg-min-max-k1}
\end{figure}

% \iffalse

We first
describe the key idea behind 
the MM algorithm, and then 
describe the MM algorithm
which is listed in Algorithm~\ref{alg:min-max:k-nn}.

\paragraph*{Key Idea}
For \textit{binary classification} ($|\mathcal{Y}| = 2$), we have the following
observation --- given a possible world
$D = \{(x_{i, j_{i, D}}, y_i)\}$
that produces prediction $l \in \mathcal{Y}$
with a top-K set $Top(K, D, t)$,
consider a different possible 
world, which we call the
{\em $l$-extreme world} of $D$
as $E_{l, D}$. In $E_{l, D}$,
we replace,
for all candidate sets with 
$y_i = l$, the 
$x_{i, j_{i, D}}$ candidate in 
$D$ with the candidate in the candidate 
set $\mathcal{C}_i$ that is most 
similar to the test example
\[
j_{i, E_{l, D}} = \arg\max_j \kappa(x_{i, j}, t)
\]
and replace, for all candidate sets
with $y_i \ne l$,
the 
$x_{i, j_{i, D}}$ candidate in 
$D$ with the candidate in the candidate 
set $\mathcal{C}_i$ that is least 
similar to the test example
\[
j_{i, E_{l, D}} = \arg\min_j \kappa(x_{i, j}, t).
\]
We have
\[
D~\text{predicts}~l \implies E_{l, D}~\text{predicts}~l.
\]
To see why, note that (1) 
replacing all candidate values for
candidate set whose label $y_i \ne l$
by something less similar to the
test example $t$ will only make it
more likely to predict $l$; (2) 
replacing all candidate
values for candidate set whose label $y_i = l$
by something more similar to $t$ will only make it
more likely to predict $l$.

Another powerful observation is that
for all possible worlds $D$ they all 
have the \textit{same} $l$-extreme
worlds $E_{l, D}$ since the construction
of the latter only relies on the most
and least similar items in each candidate
sets. We can then write 
$E_l$ as the $l$-extreme world
for all possible world $D$.
We now have
\[
\exists D.~D~\text{predicts}~l \implies E_{l}~\text{predicts}~l,
\]
and, trivially
\[
E_{l}~\text{predicts}~l  \implies \exists D.~D~\text{predicts}~l, 
\]
by simply taking $D = E_{l}$. As a result,
\[
\exists D.~D~\text{predicts}~l \Leftrightarrow E_{l}~\text{predicts}~l.
\]
One can use this observation to check whether 
$Q1(\mathcal{D}, t, l)$ evaluates to true:
this is equivalent to checking 
whether there exists any possible world
$D$ that predicts a label $l' \ne l$.
To achieve this, we can simply check
the $l'$- extreme world $E_{l'}$.

\begin{algorithm}[t!]
\small
\caption{Algorithm \textbf{MM} for answering Q1 with $K$-NN.} \label{alg:min-max:k-nn}
\begin{algorithmic}[1]
\REQUIRE {$\mathcal{D}$, incomplete dataset; $t$, target data point.}
\ENSURE {$r$, Boolean vector, s.t. $r[y]=Q1(\mathcal{D}, t, y), \forall y \in \mathcal{Y}$.}

\STATE $S \gets \mathtt{kernel} (\mathcal{D}, x_t)$

\FORALL{$i \in 1,...,|\mathcal{D}|$}
    \STATE $s_i^{\min} \gets \min\{S_{i,j}\}_{j=1}^M$, $s_i^{\max} \gets \max\{S_{i,j}\}_{j=1}^M$;
\ENDFOR

\FORALL{$l\in\mathcal{Y}$}
    \STATE $s \gets \mathtt{zeros} ( |\mathcal{D}|)$;
    \FORALL{$i \in 1,...,|\mathcal{D}|$}
        \STATE $s[i]$ $\gets$ $s_i^{\max}$ $\mathbf{if}$ $(y_i = l)$ $\mathbf{else}$ $s_i^{\min}$;
    \ENDFOR
    
    \STATE $I_K \gets \mathtt{argmax\_k} (s, K)$;
    \STATE $v \gets \mathtt{vote}( \{  y_i : i \in I_K  \} ) $;
    \IF{$\mathtt{argmax} (v) = l$}
        \STATE $r[l] \gets \mathtt{true}$;
    \ELSE
        \STATE $r[l] \gets \mathtt{false}$;
    \ENDIF
\ENDFOR

\RETURN $r$;

\end{algorithmic}
\end{algorithm}


% \begin{algorithm}[t!]
% \caption{Algorithm \textbf{MinMax} for answering Q1 with $K$-NN.} \label{alg:min-max:k-nn}
% \begin{algorithmic}[1]
% \REQUIRE {$\mathcal{D}$, incomplete dataset; $t$, target data point.}
% \ENSURE {$r$, Boolean vector, s.t. $r[y]=Q1(\mathcal{D}, t, y), \forall y \in \mathcal{Y}$.}

% \STATE $S \gets \mathtt{kernel} (\mathcal{D}, x_t)$

% \FORALL{$i \in 1,...,|\mathcal{D}|$}
%     \STATE $s_i^{\min} \gets \min\{S_{i,j}\}_{j=1}^M$, $s_i^{\max} \gets \max\{S_{i,j}\}_{j=1}^M$;
% \ENDFOR

% \FORALL{$l\in\mathcal{Y}$}
%     \STATE $s \gets \mathtt{zeros} ( |\mathcal{D}|)$;
%     \FORALL{$i \in 1,...,|\mathcal{D}|$}
%         \STATE $s[i]$ $\gets$ $s_i^{\max}$ $\mathbf{if}$ $(y_i = l)$ $\mathbf{else}$ $s_i^{\min}$;
%     \ENDFOR
    
%     \STATE $I_K \gets \mathtt{argmax\_k} (s, K)$;
%     \STATE $v \gets \mathtt{vote}( \{  y_i : i \in I_K  \} ) $;
%     \IF{$\mathtt{argmax} (v) = l$}
%         \STATE $r[l] \gets \mathtt{true}$;
%     \ELSE
%         \STATE $r[l] \gets \mathtt{false}$;
%     \ENDIF
% \ENDFOR

% \RETURN $r$;

% \end{algorithmic}
% \end{algorithm}


\paragraph*{Proof in Appendix} 
This idea might look simple
and natural, however, a formal proof 
is actually quite 
engaged (e.g., without a formal proof, it is not 
immediately clear why this algorithm cannot
handle cases in which $|\mathcal{Y}| > 2$).
We leave the full, formal proof to the
appendix of this paper.
% \xc{I think MM should work for any number of classes.}

\paragraph*{Efficient Algorithm} 
The above intuition gives us a very efficient 
algorithm to answer the query $Q1(\mathcal{D}, t, l)$,
as illustrated in Algorithm~\ref{alg:min-max:k-nn}.
We first calculate 
the similarity matrix (line 1), compute the extreme similarities that we use later (lines 2-3), and then
try to construct the $l$-extreme world
for each $l \in \mathcal{Y}$ (lines 4-7).
We then calculate the top-K set
of the $l$-extreme world (line 8)
and tally the labels to get the prediction
in the $l$-extreme world (line 9).

To answer the query $Q1(\mathcal{D}, t, l)$
(lines 10-13),
we check all $l'$-extreme worlds where $l' \ne l$
to see if any of these $l'$-extreme worlds 
predicts their corresponding $l'$. If yes,
then $Q1(\mathcal{D}, t, l) = \texttt{false}$;
otherwise, $Q1(\mathcal{D}, t, l) = \texttt{true}$.

\vspace{0.5em}
\noindent
\textbf{(Complexity)}
We analyze the complexity of Algorithm~\ref{alg:min-max:k-nn} as follows:
\begin{itemize}
\item We first precompute the similarity matrix, as well as the minimum and maximum similarities, both of which can be done in $\mathcal{O}(N \cdot M)$ time.
\item The outer loop is executed $|\mathcal{Y}|$ times.
\item The optimal world construction loop (lines 6-7) is executed $N$ times. In each iteration we retrieve the precomputed maximal or minimal values.
\item The $\mathtt{argmax\_k}$ function implemented as a heap requires $\mathcal{O} (N \log K)$ steps.
\item The $\mathtt{vote}$ function requires $\mathcal{O}(K)$ steps. The $\mathtt{argmax}$ takes $\mathcal{O}(|\mathcal{Y}|)$, although these two steps can be implemented jointly and run in $\mathcal{O}(K)$ time.
\end{itemize}
The time complexity is therefore $\mathcal{O} \left(N \cdot M + |\mathcal{Y}| \cdot (N \log K + K) \right)$.

%\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse


\subsubsection{The Special Case of $K = 1$}

When $K=1$, the data point $\mathbf{x}_{\max}$ in $D$ with the maximum similarity of $\mathbf{x}$ is the nearest neighbor and the 1-NN classifier returns the label of $\mathbf{x}_{\max}$ as its prediction.
As a result, the key to development of efficient algorithms to answer Q1 exactly is to understand when a data point can become the maximum in terms of similarity in the clean world.
In the following, we propose two algorithms based on this intuition.

\vspace{0.5em}
\noindent
\textbf{(Formulation)}
Without loss of generality, we assume that, for each $(\textbf{x}_i, y_i)\in D$, the possible world $\mathcal{C}_i$ of $\textbf{x}_i$ is of size $m$, i.e., $\mathcal{C}_i=\{\textbf{x}_{i1},...,\textbf{x}_{im}\}$ for $1\leq i\leq n$.
For any two $\mathbf{x}, \mathbf{x}'\in\mathcal{X}$, we use $s(\mathbf{x}, \mathbf{x}')$ to represent the similarity between $\mathbf{x}$ and $\mathbf{x}'$. Note that we do not assume any properties of the similarity function $s(-,-)$.


Given $D=\{(\mathbf{x}_i, y_i)\}_{i=1}^n$ and an unseen $\mathbf{x}\in\mathcal{X}$, we define the \emph{similarity matrix} as an $n\times m$ matrix $\mathbf{S}$ such that $\mathbf{S}_{ij}=s(\mathbf{x}_{ij},\mathbf{x})$, for $1\leq i \leq n$ and $1\leq j\leq m$.
Figure~\ref{fig:knn-similarity} illustrates the similarity matrix in more detail.



\vspace{0.5em}
\noindent
\textbf{(SortScan)}
Algorithm~\ref{alg:sort-scan:1-nn} outlines the \textbf{SortScan} algorithm for solving Q1 exactly.
It starts by an initialization phase (lines 2 to 5) where we maintain three fields for each $\mathbf{M}_{ij}$ that corresponds to $\mathbf{x}_{ij}$: (1) its similarity \underline{score} $s(\mathbf{x}_{ij}, \mathbf{x})$; (2) its row \underline{index} $i$; and (3) its corresponding \underline{label} $y_i$.
We convert the $n\times m$ matrix $\mathbf{M}$ into a one-dimensional array $\mathbf{A}$ with $nm$ elements, by simply concatenating the $n$ rows of $\mathbf{M}$ (line 6).
We then \emph{sort} the elements in $\mathbf{A}$ with respect to their similarity scores (line 7).
Finally, we \emph{scan} the sorted array $\mathbf{A}$ (lines 9 to 15) and perform the following:
\begin{itemize}
    \vspace{-0.5em}
    \item We keep a running \textbf{counter} with $n$ elements such that \textbf{counter}$[i]$ records the number of elements in the possible world $\mathcal{C}_i$ (corresponding to $\mathbf{x}_i$) with similarity score smaller than that of the current $\mathbf{A}[t]$ (line 9).
    \vspace{-0.5em}
    \item For each element $\mathbf{A}[t]$, we check whether all elements in the current snapshot of \textbf{counter} are nonzero (lines 10 to 12). If so, we then check whether the \underline{label} of $\mathbf{A}[t]$ is the same as the \underline{label} of $\mathbf{A}[n\cdot m]$ (line 8 and line 13), and if no, we simply return \verb|false| (line 14) since we have found evidence showing that $\mathbf{x}$ cannot be consistently classified.
    \vspace{-0.5em}
    \item We simply return \verb|true| if no evidence of inconsistency is identified after scanning $\mathbf{A}$.
\end{itemize}

\begin{algorithm}[t]
\caption{Algorithm \textbf{SortScan} for Q1 with 1-NN.} \label{alg:sort-scan:1-nn}
\begin{algorithmic}[1]
\REQUIRE {$\mathbf{S}$, the similarity matrix; $\{y_i\}_{i=1}^n$, where $(\mathbf{x}_i, y_i)\in D$.}
\ENSURE {\verb|true|, if consistently classifiable; \verb|false|, otherwise. }
\STATE $\mathbf{M} \gets m\times n$ matrix;
\FORALL{$i\in[n], j\in[m]$}
    \STATE $\mathbf{M}_{ij}.\text{\underline{score}} \gets \mathbf{S}_{ij}$;
    \STATE $\mathbf{M}_{ij}.\text{\underline{index}} \gets i$;
    \STATE $\mathbf{M}_{ij}.\text{\underline{label}} \gets y_i$;
\ENDFOR
\STATE Convert $\mathbf{M}$ into an array $\mathbf{A}$ by concatenating the $n$ rows;%, i.e., $A[i\cdot n + j]=\mathbf{M}_{ij}$;
\STATE Sort elements in $\mathbf{A}$ by the `\underline{score}' field in ascending order;
\STATE \emph{ccLabel} $\gets\mathbf{A}[n\cdot m].\text{\underline{label}}$; 
\STATE \textbf{counter} $\gets$ \emph{zeros}($n$);
\FORALL{$\mathbf{A}[t] \in \mathbf{A}$}
    \STATE \textbf{counter}[$\mathbf{A}[t].\text{\underline{index}}$] += 1;
    \IF{all elements of \textbf{counter} are nonzero}
        \IF{$\mathbf{A}[t].\text{\underline{label}} \neq $ \emph{ccLabel}}
            \RETURN \verb|false|;
        \ENDIF
    \ENDIF
\ENDFOR
\RETURN \verb|true|;
\end{algorithmic}
\end{algorithm}

\begin{lemma}\label{lemma:evidence}
For any $\mathbf{A}[t]$ such that all elements of \textbf{counter} are nonzero, then there is some $D\in\mathcal{D}$ such that the 1-NN $h$ trained on top of $D$ returns $h(\mathbf{x})=\mathbf{A}[t].$\underline{label}.
\end{lemma}

\begin{theorem}\label{theorem:alg:sort-scan:1-nn:correctness}
Algorithm~\ref{alg:sort-scan:1-nn} correctly answers $Q1$ for 1-NN.
\end{theorem}

The proofs of Lemma~\ref{lemma:evidence} and Theorem~\ref{theorem:alg:sort-scan:1-nn:correctness} are included in Appendices~\ref{proof:lemma:evidence} and~\ref{proof:theorem:alg:sort-scan:1-nn:correctness}, respectively. The time complexity of Algorithm~\ref{alg:sort-scan:1-nn} is dominated by sorting the array $\mathbf{A}$, which results in $O(nm\log(nm))$ = $O(nm(\log m + \log n))$.
For 1-NN classifiers, the sorting is in fact unnecessary.
We next propose the following \textbf{MinMax} algorithm that can reduce the complexity to linear time.

\vspace{0.5em}
\noindent
\textbf{(MinMax)}
The idea behind the \textbf{MinMax} algorithm is the following.
Rather than going through each $\mathbf{x}_{ij}$ and checking its label for consistency, as what the \textbf{SortScan} algorithm does, we can instead go through each label $y\in\mathcal{Y}$ and check whether this label can be the ``consensus'' label.
Algorithm~\ref{alg:min-max:1-nn} presents the details.

\begin{algorithm}
\caption{Algorithm \textbf{MinMax} for Q1 with 1-NN.} \label{alg:min-max:1-nn}
\begin{algorithmic}[1]
\REQUIRE {$\mathbf{S}$, the similarity matrix; $\{y_i\}_{i=1}^n$, where $(\mathbf{x}_i, y_i)\in D$.}
\ENSURE {\verb|true|, if consistently classifiable; \verb|false|, otherwise. }
\FORALL{$i\in[n]$}
    \STATE $s_i^{\min} \gets \min\{\mathbf{S}_{ij}\}_{j=1}^m$, $s_i^{\max} \gets \max\{\mathbf{S}_{ij}\}_{j=1}^m$;
\ENDFOR
\FORALL{$i\in[n]$}
    \IF{$\forall k\neq i$, $s_i^{\min} \geq s_k^{\max}$}
        \RETURN \verb|true|;
    \ENDIF
\ENDFOR
\RETURN \verb|false|;
\end{algorithmic}
\end{algorithm}

In Algorithm~\ref{alg:min-max:1-nn}, for each possible world $\mathcal{C}_i$ of $\mathbf{x}_i$ that corresponds to the $i$-th row of $\mathbf{S}$, we first identify the minimum and maximum similarity scores $s_i^{\min}$ and $s_i^{\max}$ (lines 1 to 2).
We then go through each $s_i^{\min}$ and check whether it dominates \emph{all} other $s_k^{\max}$'s whenever $k\neq i$ (lines 3 to 4). If there exists such a case, then we can return \verb|true| (line 5); otherwise we return \verb|false| (line 6).
Figure~\ref{fig:alg-min-max-k1} presents an example to illustrate how Algorithm~\ref{alg:min-max:1-nn} works.



\begin{theorem}\label{theorem:alg:min-max:1-nn:correctness}
Algorithm~\ref{alg:min-max:1-nn} correctly answers $Q1$ for 1-NN.
\end{theorem}
The poof is included in Appendix~\ref{proof:theorem:alg:min-max:1-nn:correctness}. We now analyze the time complexity of Algorithm~\ref{alg:min-max:1-nn}:
\begin{itemize}
    \item It takes $O(nm)$ to scan the $n\times m$ matrix $\mathbf{S}$ once to compute the minimum and maximum scores for each row.
    \item To perform the check in lines 3 to 6, a naive implementation would take $O(n^2)$. However, we can further optimize it by grouping the $y_i$'s. That is, we compute the minimum and maximum scores for each distinct $y\in\mathcal{Y}$. Formally, $s_y^{\min} = \min_{y_i=y}\{ s_i^{\min}\}$, and $s_y^{\max} = \max_{y_i=y}\{ s_i^{\max}\}$. It clearly only takes $O(n)$ time to compute these quantities. We then simply need to check whether there is some $y\in\mathcal{Y}$ such that $s_y^{\min} \geq s_{y'}^{\max}$ for all $y'\neq y$. The correctness follows from a similar reasoning as that in the proof of Theorem~\ref{theorem:alg:sort-scan:1-nn:correctness}, and it only takes $O(|\mathcal{Y}|^2)=O(1)$ time to check this condition.
\end{itemize}
As a result, we can conclude that the time complexity of Algorithm~\ref{alg:min-max:1-nn} is $O(nm)$.

\subsubsection{The General Case when $K>1$}

We now extend the \textbf{MinMax} algorithm to deal with $Q1$ for the general case when $K$ $>$ 1.
While we can also extend the \textbf{SortScan} algorithm, we postpone its discussion to Section~\ref{sec:cc-knn:q2} since the same algorithm will be used to address $Q2$.

When $K$ $>$ 1, Algorithm~\ref{alg:min-max:1-nn} no longer works, because we now need a majority (i.e., the most frequent) vote rather than a single vote (from the point with the minimum/maximum similarity score) to determine the ``consensus'' label.
Nonetheless, the idea that backs up the extension remains the same -- we are still interested in the question that whether a label $y\in\mathcal{Y}$ can be the ``consensus'' label.
However, rather than considering the ``worst-case'' scenario where the minimum similarity score of $y$ would still dominate the maximum similarity scores of the other labels, we instead consider the ``best-case'' scenario where the points with label $y$ would take their maximum scores whereas the points with other labels would take their minimum scores.
Algorithm~\ref{alg:min-max:k-nn} presents the details.  %of this idea.

\begin{algorithm}
\caption{Algorithm \textbf{MinMax} for Q1 with $K$-NN ($K>1$).} \label{alg:min-max:k-nn}
\begin{algorithmic}[1]
\REQUIRE {$\mathbf{S}$, the similarity matrix; $\{y_i\}_{i=1}^n$, where $(\mathbf{x}_i, y_i)\in D$.}
\ENSURE {\verb|true|, if consistently classifiable; \verb|false|, otherwise. }
\FORALL{$i\in[n]$}
    \STATE $s_i^{\min} \gets \min\{\mathbf{S}_{ij}\}_{j=1}^m$, $s_i^{\max} \gets \max\{\mathbf{S}_{ij}\}_{j=1}^m$;
\ENDFOR
\STATE Group $\{\mathbf{x}_i\}_{i=1}^n$ by $y_i$. Let $\mathcal{G}_y$ be the group with label $y$.
\STATE \textbf{ccLabel} $\gets$ a Boolean array with $|\mathcal{Y}|$ elements;
\FORALL{$y\in\mathcal{Y}$}
    \STATE \textbf{ccLabel}[$y$] $\gets$ \verb|false|;
\ENDFOR
\FORALL{$y\in\mathcal{Y}$}
    \STATE $\mathbf{z}$ $\gets$ \emph{zeros}($n$);
    \FORALL{$i\in[n]$}
        \STATE $\mathbf{z}_i$.\underline{label} $\gets$ $y_i$;
        \IF{$\mathbf{x}_i\in\mathcal{G}_y$}
            \STATE $\mathbf{z}_i$.\underline{score} $\gets$ $s_i^{\max}$;
        \ELSE
            \STATE $\mathbf{z}_i$.\underline{score} $\gets$ $s_i^{\min}$;
        \ENDIF
    \ENDFOR
    \STATE $\mathcal{L}_y$ $\gets$ top $K$ elements of $\mathbf{z}$ with respect to $\mathbf{z}_i$.\underline{score};
    \IF{$y$ is the most frequent label in $\mathcal{L}_y$}
        \STATE \textbf{ccLabel}[$y$] $\gets$ \verb|true|;
    \ENDIF
\ENDFOR
\IF{there is exactly one $y\in\mathcal{Y}$ s.t. \textbf{ccLabel}[$y$] is true}
    \RETURN \verb|true|;
\ENDIF
\RETURN \verb|false|;
\end{algorithmic}
\end{algorithm}

In Algorithm~\ref{alg:min-max:k-nn}, we start by computing the minimum and maximum similarity scores for each possible world $\mathcal{C}_i$ that corresponds to $\mathbf{x}_i$ (lines 1 to 2), the same as Algorithm~\ref{alg:min-max:1-nn}.
We then group the $\mathbf{x}_i$'s by their labels, and for $y\in\mathcal{Y}$ we use $\mathcal{G}_y$ to denote the corresponding group with label $y$ (line 3).
For each $y\in\mathcal{Y}$, we check whether it can be the final ``consensus'' label (lines 4 to 17).
If so, there must exist \emph{some} $D_y\in\mathcal{D}$ such that $y$ is the most frequent label among the top $K$ $\mathcal{x}_i$'s with highest similarity scores.
We can therefore simply check the \emph{best case} of such $D_y$ --- all $\mathbf{x}_i\in\mathcal{G}_y$ takes $s_i^{\max}$ (i.e., the maximum similarity score from $\mathcal{C}_i$) whereas all other $\mathbf{x}_i$ with $y_i\neq y$ takes $s_i^{\min}$ (lines 9 to 14).
We then collect the labels of the top $K$ elements in this best $D_y$ (line 15).
If $y$ turns out to be the most frequent one among the top $K$ labels, $y$ then can be one candidate of the ``consensus'' label (lines 16 to 17).
Finally, if there is \emph{one and only one} candidate for the ``consensus'' label, $\mathbf{x}$ can then be consistently classified (lines 18 to 19); otherwise $\mathbf{x}$ is not consistently classifiable (line 20).
Figure~\ref{fig:alg-min-max-k3} illustrates Algorithm~\ref{alg:min-max:k-nn} with an example when $K=3$.



\begin{theorem}\label{theorem:alg:min-max:k-nn:correctness}
Algorithm~\ref{alg:min-max:k-nn} correctly returns answers to Q1 for $K$-NN when $K>1$.
\end{theorem}
The proof is included in Appendix~\ref{proof:theorem:alg:min-max:k-nn:correctness}. We analyze the time complexity of Algorithm~\ref{alg:min-max:k-nn} in the following:
\begin{itemize}
    \item Compute $s_i^{\min}$ and $s_i^{\max}$ (lines 1 to 2) -- it takes $O(nm)$ time since we have to scan the $n\times m$ similarity matrix $\mathbf{S}$ once;
    \item Group $\mathbf{x}_i$'s by their labels (line 3) -- it takes $O(n)$ time;
    \item Determine whether each $y\in\mathcal{Y}$ can be an anchor label (lines 7 to 17) -- it takes $O(|\mathcal{Y}|(n + n\log K)=O(|\mathcal{Y}|n(1+\log K)$ time, because for each $y\in\mathcal{Y}$ we need $O(n)$ time to construct its anchor world $D_y$ (lines 9 to 14) and $O(n\log K)$ to find the top $K$ from $D_y$ (using a min-heap).
\end{itemize}
Summing up the above terms, the time complexity of Algorithm~\ref{alg:min-max:k-nn} is therefore $O(n(m + |\mathcal{Y}|(1+\log K))$, which reduces to $O(nm)$ if we assume $|\mathcal{Y}|\ll\min\{n, m\}$ and $K\ll\min\{n, m\}$.

%Let $x_{ij}$ denote the $i$-th example in $D_j$. Let $S_{ij}$ denote the similarity between $x_{ij}$ and $x$.
%$$f_{D_j}(x) = y_{\arg\max\limits_i S_{ij}} $$

\subsection{Counting Query (Q2)}\label{sec:cc-knn:q2}

%We provide different solutions to Q2 with respect to its different semantics defined in Section~\ref{sec:cc:query:q2}.
%First, consider the \emph{representative semantics}, where we return one $D\in\mathcal{D}_y$ for each $y\in\mathcal{Y}$ when $\mathbf{x}$ cannot be consistently classified. We only need to slightly modify Algorithm~\ref{alg:min-max:k-nn} for this purpose: Instead of checking the existence and uniqueness of anchor label, we simply return the anchor world $D_y$ constructed for each $y\in\mathcal{Y}$.
%We next consider the \emph{counting semantics} and \emph{enumeration semantics} in the rest of this section.

%\subsubsection{Counting Semantics}

%We establish the basic framework first and then discuss potential optimizations.
%By counting semantics, 
We need to return the cardinality $|\mathcal{D}_y|$ of the inconsistency region $\mathcal{D}_y$ for each $y\in\mathcal{Y}$.
We now develop a \textbf{SortCount} algorithm piggybacking on the \textbf{SortScan} algorithm presented in Algorithm~\ref{alg:sort-scan:1-nn}.
Algorithm~\ref{alg:sort-count} presents the details.

We first obtain the same sorted array $\mathbf{A}$ as in Algorithm\ref{alg:sort-scan:1-nn} (line 1).
We next again scan this array $\mathbf{A}$.
Instead of maintaining one single counter (the \textbf{counter} array in Algorithm~\ref{alg:sort-scan:1-nn}) that counts for each $\mathbf{x}_i$ the number of possible worlds with smaller similarity scores than the current element $\mathbf{A}[t]$ in $\mathbf{A}$, we maintain two counters -- the one with smaller similarity sores remains the same ($\textbf{counter}_{\alpha}$), with an additional one that counts possible worlds with larger similarity scores ($\textbf{counter}_{\beta}$).
Initially, all entries in $\textbf{counter}_{\alpha}$ are zero, whereas all entries in $\textbf{counter}_{\beta}$ are $m$ (i.e., the total number of possible worlds for each $\mathbf{x}_i$).


Now consider the current entry $\mathbf{A}[t]$ being examined (line 5).
Suppose that it corresponds to $\mathbf{x}_i$.
Our strategy is to count the number of possible worlds $\mathcal{D}_t\subseteq\mathcal{D}$ such that $\mathbf{A}[t]$, the current possible version of $\mathbf{x}_i$, has the $K$-th largest similarity score.
Clearly, $\{\mathcal{D}_t\}_{t=1}^{nm}$ is a \emph{partition} of $\mathcal{D}$, i.e., $\mathcal{D}_t\cap\mathcal{D}_{t'}= \emptyset$ for $t \neq t'$, $1\leq t, t'\leq nm$ and   $\cup_{t=1}^{nm}\mathcal{D}_t=\mathcal{D}$.
Our strategy thus avoids double counting.

\begin{algorithm}
\caption{Algorithm \textbf{SortCount} for Q2 with $K$-NN.} \label{alg:sort-count}
\begin{algorithmic}[1]
\REQUIRE {$\mathbf{S}$, the similarity matrix; $\{y_i\}_{i=1}^n$, where $(\mathbf{x}_i, y_i)\in D$.}
\ENSURE {$\{|\mathcal{D}_y|\}$, for all $y\in\mathcal{Y}$.}

\STATE $\mathbf{A}\gets$ sorted array by lines 1 to 7 of Algorithm~\ref{alg:sort-scan:1-nn};
\STATE $\textbf{counter}_{\alpha}$ $\gets$ \emph{zeros}($n$);
\STATE $\textbf{counter}_{\beta}$ $\gets$ $m \cdot$ \emph{ones}($n$);

\STATE $|\mathcal{D}_y| \gets 0$, for all $y\in\mathcal{Y}$;

\FORALL{$\mathbf{A}[t] \in \mathbf{A}$}
    \STATE $i\gets\mathbf{A}[t].\text{\underline{index}}$;
    \STATE \textbf{counter}$_{\alpha}$[$i$] += 1;  
    \STATE \textbf{counter}$_{\beta}$[$i$] -= 1;
    \STATE $\mathcal{I}_{\alpha}\gets\{j: j\neq i$ and \textbf{counter}$_{\alpha}[j]>0\}$;
    \STATE $\mathcal{I}_{\beta}\gets\{j: j\neq i$ and \textbf{counter}$_{\beta}[j]>0\}$;
    \IF{$|\mathcal{I}_{\beta}|\geq K-1$ and $|\mathcal{I}_{\alpha}| \geq n-K$}
        \FORALL{$(K-1)$-subset $\mathcal{S}_{\beta}$ of $\mathcal{I}_{\beta}$ and $(n - K)$-subset $\mathcal{S}_{\alpha}$ of $\mathcal{I}_{\alpha}$ such that $\mathcal{S}_{\alpha}\cap\mathcal{S}_{\beta}=\emptyset$}
            \STATE $y\gets$ the top $K$ label of $\{\mathbf{x}_i\}\cup\{\mathbf{x}_j: j\in\mathcal{I}_{\beta}\}$;
            \STATE $|\mathcal{D}_y|$ += $\prod_{j\in\mathcal{S}_{\alpha}}\textbf{counter}_{\alpha}[j]\cdot \prod_{j\in\mathcal{S}_{\beta}}\textbf{counter}_{\beta}[j]$;
        \ENDFOR
    \ENDIF
\ENDFOR
\RETURN $\{|\mathcal{D}_y|\}$, for all $y\in\mathcal{Y}$;
\end{algorithmic}
\end{algorithm}

In more detail, in lines 7 and 8, we increase $\textbf{counter}_{\alpha}[i]$ and decrease $\textbf{counter}_{\beta}[i]$.
We define $\mathcal{I}_{\alpha}$ to include all $\mathbf{x}_j$'s such that $j\neq i$ and $\textbf{counter}_{\alpha}[j]>0$.
Clearly, $\mathcal{I}_{\alpha}$ represents the set of $\mathbf{x}_j$'s with similarity scores less than the similarity score of (the current possible version of) $\mathbf{x}_i$.
Similarly, we can define $\mathcal{I}_{\beta}$ (lines 9 and 10).
Given the stringent requirement of insisting $\mathbf{A}[t]$ be at exactly the $K$-th position in the final standing, it must simultaneously hold that $|\mathcal{I}_{\beta}|\geq K-1$ \emph{and} $|\mathcal{I}_{\alpha}|\geq n-K$.
If so, we then enumerate all subsets of $\mathcal{I}_{\beta}$ and $\mathcal{I}_{\alpha}$, with $K-1$ and $n-K$ elements respectively, and check each pair $(\mathcal{S}_{\beta}, \mathcal{S}_{\alpha})$ of such subsets (lines 11 and 12).
Clearly, $\mathcal{S}_{\beta}$ plus $\mathbf{x}_i$ contain exactly the top $K$ elements.
Thus, in line 13 we can simply decide the top $K$ label $y$ (i.e., the most frequent label among the top $K$ elements).
Finally, in line 14 we compute the number of possible worlds that supports this arrangement, which is equivalent to the number of possible worlds subsumed by the pair $(\mathcal{S}_{\beta}, \mathcal{S}_{\alpha})$.

For each $\mathbf{x}_j\in\mathcal{S}_{\beta}$, the corresponding $\textbf{counter}_{\beta}[j]$ is the number of possible versions of $\mathbf{x}_j$ from which we can pick for the top $K-1$ elements.
Similarly, for each $\mathbf{x}_j\in\mathcal{S}_{\alpha}$, the corresponding $\textbf{counter}_{\alpha}[j]$ is the number of possible versions of $\mathbf{x}_j$ from which we can pick for the bottom $n-K$ elements.
As a result, the total number of possible worlds subsumed by $(\mathcal{S}_{\beta}, \mathcal{S}_{\alpha})$ is simply 
$$\prod\nolimits_{j\in\mathcal{S}_{\alpha}}\textbf{counter}_{\alpha}[j]\cdot \prod\nolimits_{j\in\mathcal{S}_{\beta}}\textbf{counter}_{\beta}[j].$$
Figure~\ref{fig:alg-sort-count-k1} illustrates the \textbf{SortCount} algorithm when $K=1$.



\begin{theorem}\label{theorem:alg:sort-count:correctness}
Algorithm~\ref{alg:sort-count} correctly provides answers to Q2 for the counting semantics.
\end{theorem}
The proof is included in Appendix~\ref{proof:theorem:alg:sort-count:correctness}. We now analyze the time complexity of Algorithm~\ref{alg:sort-count}:
\begin{itemize}
    \item Generating the sorted array $\mathbf{A}$ takes $O(nm\log(nm))$ = $O(nm(\log m + \log n))$ time as before.
    \item The time on lines 5 to 14 is dominated by lines 12 to 14. $\mathbf{A}$ has $nm$ entries, and for each $\mathbf{A}[t]$, in the worst case we need to consider all possible $K-1$ subsets from positive entries of $\textbf{counter}_{\beta}$. However, once we fix the subset $\mathcal{S}_{\beta}$, the subset $\mathcal{S}_{\alpha}$ is automatically fixed as well. As a result, we need to consider at most ${n \choose K - 1}$ such pairs $(\mathcal{S}_{\beta}, \mathcal{S}_{\alpha})$. For each pair, line 13 takes $O(K)$ time to determine the label $y$, and line 14 takes $O(n)$ time to multiply the counts. Therefore, the time complexity of lines 12 to 14 is $O(nm{n \choose K - 1}(K + n))$.
\end{itemize}
We can thus conclude that the complexity of Algorithm~\ref{alg:sort-count} is $O(nm(\log m + \log n + {n \choose K - 1}(K + n)))$. Assume that $n$ is large and $K\ll\min\{n, m\}$.
Using Stirling's approximation, $n!\sim\sqrt{2\pi n}\Big(\frac{n}{e}\Big)^n$, we have ${n \choose K - 1}\sim O(n^{K-1})$.
As a result, the time complexity can be simplified to $O(nm(\log m + \log n + n^K))$.
The dominant $n^K$ factor suggests that Algorithm~\ref{alg:sort-count} can only work efficiently for small $K$'s (e.g., $K=1$ or $K=3$) when $n$ is large.


\begin{algorithm}
\caption{Algorithm \textbf{SortCountDP} for Q2 with $K$-NN and binary classification.} \label{alg:sort-count:dp:binary}
\begin{algorithmic}[1]
\REQUIRE {$\mathbf{S}$, the similarity matrix; $\{y_i\}_{i=1}^n$, where $(\mathbf{x}_i, y_i)\in D$.}
\ENSURE {$\{|\mathcal{D}_y|\}$, for all $y\in\mathcal{Y}$.}

\STATE $\mathbf{A}\gets$ sorted array by lines 1 to 7 of Algorithm~\ref{alg:sort-scan:1-nn};
\STATE $\textbf{counter}_{\alpha}$ $\gets$ \emph{zeros}($n$);
\STATE $\textbf{counter}_{\beta}$ $\gets$ $m \cdot$ \emph{ones}($n$);

\STATE $|\mathcal{D}_y| \gets 0$, for all $y\in\mathcal{Y}$;
\FORALL{$\mathbf{A}[t] \in \mathbf{A}$}
    \STATE $i\gets\mathbf{A}[t].\text{\underline{index}}$;
    \STATE \textbf{counter}$_{\alpha}$[$i$] += $1$;  
    \STATE \textbf{counter}$_{\beta}$[$i$] -= $1$;
    \STATE Group the pairs $\{(\textbf{counter}_{\alpha}[i], \textbf{counter}_{\beta}[i])\}_{i=1}^n$ into $\mathcal{G}_0$ (with label $0$) and $\mathcal{G}_1$ (with label $1$);
    \STATE Compute $\mathbf{C}_0(i,j)$ using dynamic programming for $1\leq i\leq |\mathcal{G}_0|$ and $1\leq j\leq\min\{K-1, |\mathcal{G}_0|\}$ (Equation~\ref{eq:recurrence});
    \STATE Compute $\mathbf{C}_1(i,j)$ similarly;
    \FORALL{$l$ $0$'s and $(K-1-l)$ $1$'s, $0\leq l\leq K-1$}
        \STATE $y\gets$ top $K$ label from $y_i$ and the $K-1$ labels;
        \STATE $|\mathcal{D}_y|$ += $\mathbf{C}_0(1, l)\cdot\mathbf{C}_1(1,K-1-l)$;
    \ENDFOR
\ENDFOR

\RETURN $\{|\mathcal{D}_y|\}$, for all $y\in\mathcal{Y}$;
\end{algorithmic}
\end{algorithm}

\vspace{0.5em}
\noindent
\textbf{(Optimization using Dynamic Programming)}
We can further reduce the time complexity of Algorithm~\ref{alg:sort-count}.
In Algorithm~\ref{alg:sort-count}, $|\mathcal{D}_y|$ can be updated multiple times due to the fact that different top $K$ arrangements may lead to the same conclusion that $y$ is the most frequent label.
As an example, consider $\mathcal{Y}=\{0, 1\}$ and $K=3$. Suppose that the current element $\mathbf{A}[t]$ has label $0$ and we need to pick two elements from $\mathcal{I}_{\beta}$.
Since we only care about the label $y$ that would be chosen from these top $K$ elements, it does not matter \emph{which} two elements we pick from $\mathcal{I}_{\beta}$.
Rather, it is the \emph{distribution} (i.e., histogram) of the top $K$ labels that matters.
In this example, if both elements have label $0$, then $y=0$; if both elements have label $1$, then $y=1$; and if one element has label $0$ while the other has label $1$, then $y=0$ again.

Therefore, instead of determining the distribution \emph{afterwards} (i.e., after we choose the top $K-1$ elements from $\mathcal{I}_{\beta}$), we can determine it \emph{beforehand}, which automatically determines the label $y$ in question as well.
Given that we have $|\mathcal{Y}|$ labels, the total number of distributions (of the top $K-1$ labels from $\mathcal{I}_{\beta}$) is restricted to ${(K-1) + |\mathcal{Y}| - 1 \choose |\mathcal{Y}| - 1}$.\footnote{This is equivalent to the number of \emph{non-negative} integer solutions to the equation $z_1+\cdots+z_{|\mathcal{Y}|-1}=K-1$.}
This number is pretty small given that $K$ and $|\mathcal{Y}|$ are usually both small.
For the previous example where $K=3$ and $|\mathcal{Y}|=2$, the total number of distributions is therefore ${(3-1) + 2-1 \choose 2-1} = 3$, matching our analysis.

Our remaining task is to compute the number of possible worlds for each distribution.
Note that there is \emph{overlap} in this computation when considering different distributions.
Continuing with our example, suppose that the two elements we pick from $\mathcal{I}_{\beta}$ are $\mathbf{x}_1$ and $\mathbf{x}_2$, with corresponding labels $y_1=0$ and $y_2=1$.
Clearly, $\mathbf{x}_1$ contributes to two distributions $\{0, 0\}$ (i.e. two $0$'s) and $\{0, 1\}$ (i.e., one $0$ and one $1$), whereas $\mathbf{x}_2$ also contributes to two distributions $\{0, 1\}$ and $\{1, 1\}$ (i.e., two $1$'s).
We can therefore further use dynamic programming to exploit this computation overlap, as presented by Algorithm~\ref{alg:sort-count:dp:binary} for the binary classification case.

%Specifically, assume that $|\mathcal{Y}|=2$.
We group the pairs $\{(\textbf{counter}_{\alpha}[i], \textbf{counter}_{\beta}[i])\}_{i=1}^n$ by the corresponding label $y_i$ (either $y_i=0$ or $y_i=1$).
Let the two groups be $\mathcal{G}_0$ and $\mathcal{G}_1$, respectively.
Our goal is to compute the number of possible worlds that support each distribution of the $K-1$ labels taken from $\mathcal{I}_{\beta}$.
We further break down this computation task based on the number of the $K-1$ labels belonging to $\mathcal{G}_0$ or $\mathcal{G}_1$.

Suppose that we need to pick $l$ labels from $\mathcal{G}_0$ (and $K-1-l$ labels from $\mathcal{G}_1$).
Without loss of generality, assume that $|\mathcal{G}_0|=N$ and the pairs in $\mathcal{G}_0$ are $(\textbf{counter}_{\alpha}[1], \textbf{counter}_{\beta}[1])$, ..., $(\textbf{counter}_{\alpha}[N], \textbf{counter}_{\beta}[N])$.
Let $\mathbf{C}_0(i,j)$ be the number of possible worlds by picking $j$ labels from $\textbf{counter}_{\beta}[i, ..., N]$, where $0\leq j \leq \min\{N, K-1\}$.
The remaining $N-j$ labels are picked from $\textbf{counter}_{\alpha}$.
We have the following recurrence relationship:
\begin{equation}\label{eq:recurrence}
\mathbf{C}_0(i, j) = \textbf{counter}_{\alpha}[i]\cdot\mathbf{C}_0(i+1, j) + \textbf{counter}_{\beta}[i]\cdot\mathbf{C}_0(i+1, j-1).
\end{equation}
Clearly, there are two options --- we either pick $\textbf{counter}_{\beta}[i]$ or not.
If we do not pick it, then we instead pick $\textbf{counter}_{\alpha}[i]$ and pick $j$ elements from $\textbf{counter}_{\beta}[i+1, ..., N]$ --- the number of possible worlds in this case is thus $\textbf{counter}_{\alpha}[i]\cdot\mathbf{C}_0(i+1, j)$;
on the other hand, if we pick it, then we are left with picking $j-1$ elements from $\textbf{counter}_{\beta}[i+1, ..., N]$ --- the number of possible worlds in this case is then 
$\textbf{counter}_{\beta}[i]\cdot\mathbf{C}_0(i+1, j-1)$.
The base conditions for Equation~\ref{eq:recurrence} are the following:
\begin{enumerate}
    \item $\mathbf{C}_0(i, j)=\textbf{counter}_{\alpha}[i]\cdot\mathbf{C}_0(i+1, j)$, if $j=0$;
    \item $\mathbf{C}_0(i, j)=0$, if $j>N-i$;
    \item $\mathbf{C}_0(N+1,0)=1$.
\end{enumerate}
Clearly, the entry $\mathbf{C}_0(1, l)$ is the number of possible worlds if we pick $l$ labels from $\mathcal{G}_0$. Note that we only need to compute $\mathbf{C}_0$ once using dynamic programming --- all $\mathbf{C}(1, l)_0$ with $0\leq l\leq K-1$ can then be looked up from the computed $\mathbf{C}$.
We thus see that dynamic programming helps avoid duplicating computations across different distributions (i.e. with different $l$'s).

We can use the same approach to compute the number of possible worlds that support picking $K-1-l$ labels from $\mathcal{G}_1$. We use $\mathbf{C}_1$ to denote the corresponding matrix and the entry $\mathbf{C}_1(1, K-1-l)$ is the one to look up.

\begin{example}
Let us continue with our previous example when $|\mathcal{Y}|=2$ and $K=3$.
For any current $\mathbf{A}[t]$, we are interested in the distribution of the $K-1=2$ labels taken from $\mathcal{I}_{\beta}$, based on the current $\textbf{counter}_{\alpha}$ and $\textbf{counter}_{\beta}$.
Clearly there are only three possible cases for the two labels: (1) two $0$'s; (2) one $0$ and one $1$; and (3) two $1$'s. Using the above dynamic programming approach yields the number of possible worlds for each case: (1) $\mathbf{C}_0(1, 2)$ and $\mathbf{C}_1(1, 0)$ since we need two $0$'s; (2) $\mathbf{C}_0(1, 1)$ and $\mathbf{C}_1(1,1)$ since we need one $0$ and one $1$; and $\mathbf{C}_0(1, 0)$ and $\mathbf{C}_1(1,2)$ since we need no $0$'s but two $1$'s.
\end{example}

We now analyze the time complexity of Algorithm~\ref{alg:sort-count:dp:binary}:
\begin{itemize}
    \item Generating the sorted array $\mathbf{A}$ again takes $O(nm\log(nm))$ = $O(nm(\log m + \log n))$ time as before.
    \item The time on lines 5 to 14 is dominated by computing the dynamic programming matrices $\mathbf{C}_0$ and $\mathbf{C}_1$ (lines 10 and 11). The time complexity in the worst case is $O(nK)$ for each $\mathbf{A}[t]$. As a result the overall time complexity is $O(mn^2K)$.
\end{itemize}
Therefore, the time complexity of Algorithm~\ref{alg:sort-count:dp:binary} is $O(mn(\log m+\log n + nK))$.
This is a dramatic reduction from that of Algorithm~\ref{alg:sort-count}, albeit only for the case of binary classification.


%\subsubsection{Enumeration Semantics}

%We only need minor modification to Algorithm~\ref{alg:sort-count} to make it work for the enumeration semantics.
%Rather than just maintaining a counter for the number of possible worlds with smaller/larger similarity scores, we simply keep track of those possible worlds directly.
%We then return all possible combinations of the corresponding possible worlds at line 14 of Algorithm~\ref{alg:sort-count} by performing a Cartesian product rather than just multiplying the counts.

\fi


==> [arXiv] Certain Prediction/Experiments.tex <==
% !TEX root = CC.tex
\section{Experiments}\label{sec:evaluation}

We now conduct an extensive set of experiments to compare CPClean with other data cleaning approaches in the context of K-nearest neighbor classifiers.


% evaluate our proposal along two dimensions:
% \begin{itemize}%[wide,labelindent=0pt]
%     \itemsep0em
%     \item \emph{End-to-End Performance (Section~\ref{subsec:end-to-end})}
%         how does CPClean compare with other algorithms in terms of improving the performance of downstream ML models.
%     \item \emph{Abaltion Analysis}: (Section~\ref{subsec:ablation}) how effective is our  approach to make all examples in $D_{\text{val}}$  CP'ed?
%     % \item \emph{Evaluating the Decision Problem (Section~\ref{subsec:decision-evaluation}).} XXX
%     % \item \emph{Evaluating the Optimization Problem (Section~\ref{subsec:optimization-evaluation})} how effective is our approach to make all examples in  $D_{\text{val}}$  CC'ed.
% \end{itemize} 



\begin{table}[t!]
\centering
\scalebox{0.8}{
\begin{tabular}{l|cccc}
\hline
\textbf{Dataset} & \textbf{Error Type} & \textbf{\#Examples} & \textbf{\#Features}&\textbf{Missing rate} \\ \hline
\at{BabyProduct}~\cite{babyproduct} & real &3042  &7 &11.8\% \\ 
\at{Supreme}~\cite{supreme} & synthetic &3052  &7&20\%  \\ 
\at{Bank}~\cite{DELVE} & synthetic & 3192 & 8&20\% \\ 
\at{Puma}~\cite{DELVE} & synthetic & 8192 & 8&20\% \\ \hline
\end{tabular}
}
\caption{Datasets characteristics}
\label{tbl:datasets}
\vspace{-5mm}
\end{table}

\subsection{Experimental Setup}


\stitle{Hardware and Platform.} All our experiments were performed on a machine with a 2.20GHz Intel Xeon(R) Gold 5120 CPU.

\stitle{Datasets.} One main challenge of evaluating data cleaning solutions is the lack of datasets with ground truth, and hence most data cleaning work resort to synthetic error injection. This is especially true in the context of incomplete information: a dataset with missing values is not likely to come with ground truth. In this work, besides three datasets with synthetic errors, we manage to find one dataset with \textit{real} missing values, where we are able to obtain the \textit{ground truth} via manual Googling. We
summarize all datasets in Table~\ref{tbl:datasets}. 

% \xc{Describe all datasets here}.
The \at{BabyProduct} dataset  contains various baby products of different categories (e.g., bedding, strollers).  Since the dataset was scraped from websites using Python scripts~\cite{babyproduct}, many records have missing values, presumably due to extractor errors.
%%%
We designed a classification task to predict whether a given baby product has a high price or low price based on other attributes (e.g. weight, brand, dimension, etc), and we selected a subset of product categories whose price difference is not so high so as to make the classification task more difficult.
%%
For records with missing brand attribute, we then perform a Google search using the product title to obtain the product brand. For example, one record titled ``{\em Just Born Safe Sleep Collection Crib Bedding in Grey}'' is missing the product brand, and a search reveals that the brand is ``Just Born.''

%is missing; By searching the title on Google, we found out the brand to be "MLB".) %\xc{@Peng, give an example from the dataset here}). 
%We focus on repairing missing  In particular, the ``brand'' attribute for many products contains missing values. 



%81\% of which have missing value at the ``brand" attribute.  For ease of cleaning, we randomly selected three categories (Baby Bedding, Nursing, and Bath Tubs) and only kept the 3042 products (after removing duplicates) in the three categories. After that, we manually fill in the missing values one by one using google. 

%The Supreme, Bank and Puma datasets are originally clean so we artificially inject missing values to them. 


We also use three datasets (\at{Supreme}, \at{Bank}, \at{Puma}), originally with no missing values, to inject synthetic missing values. Our goal is to inject missing values in the most realistic way possible and also to ensure that the missing values can have a large impact on classification accuracy. We follow the popular ``Missing Not At Random'' assumption~\cite{rubin1976inference}, where the probability of missing may be higher for more sensitive/important attributes. For example, high income people are more likely to not report their income in a survey. 
%For example, in clinical surveys, critical information is more likely to be missing than others~\cite{kaushal2014missing}, for example, blood sugar values are more likely to be missing than age because certain groups of people may not be tested for blood sugar. 
We first assess the relative importance of each feature in a classification task (by measuring the accuracy loss after removing a feature), and use the relative feature importance as the relative probability of a feature missing. We can then inject missing values into a dataset for any given missing rate (we use 20\% in our experiment). 



% We also ensure that the overall missing 

% To make the distribution of the injected missingness as realistic as possible, we consider a typical cause of missing value in practice: In surveys, people tend to not fill in sensitive personal information such as salary, age and disease history, which are usually more informative for the survey. 
% In this example, the probability of being missing is dependent on the attribute and values in important attributes are more likely to be missing. Following this example, we inject missing values according to attribute importance. Specifically, we weight each attribute $A_i$ by the accuracy decrease $\delta_{A_i}$ of removing the attribute in a KNN classification task. Next, we normalize the weights to be $\delta_{A_i}'=\delta_{A_i}/\sum_j^M \delta_{A_j}$ to represent the importance of each attribute, where $M$ is the number of attributes. We inject missing value to each cell of attribute $A_i$ with a probability of $Mr_{\text{mv}}\delta_{A_i}'$, ensuring the overall missing rate to be a predefined value $r_{\text{mv}}$. We choose $r_{\text{mv}}=20\%$, which is a common missing rate in real world~\cite{saar2007handling}.



\stitle{Model.} We use a KNN classifier with K=3
and use Euclidean distance 
as the similarity function.
%
%, where the label of an example is predicted as the most common one among its top 3 nearest neighbors in the training set measured by euclidean distance. 
%%%
For each dataset, we randomly select 1,000 examples as the validation set and 1,000 examples as the test set. The remaining examples are used as the training set.


%\subsubsection{Different types of missing mechanisms}
%The mechanism of missing values are generally categorized into three types~\cite{rubin1976inference,little2019statistical}: Missing Completely At Random (MCAR), Missing At Random (MAR), and Missing Not At Random (MNAR). To investigate how our method performs with the presence of different types of missing mechanisms, we inject missing values using each mechanism respectively to X clean datasets. We control the amount of missing values with a missing rate $r_{\text{mv}}$, i.e. the percentage of cells with missing values among all cells. The description and injection procedures for each type are as follows:
%\begin{itemize}
%\item MCAR. In this type, for each cell, the probability of being missing is independent of any observed or unobserved data. Therefore, we inject missing value to each cell independently with a probability $r_{\text{mv}}$, the overall missing rate.
%\item MAR. In this type, for each cell, the probability of being missing is only dependent on the observed data, i.e. the non-missing data such as attributes. A typical example is that people tend to not fill in sensitive personal information such as salary, age and disease history in surveys, resulting in more missing values in these attributes. Actually, these attributes are usually more informative for the survey. In this example, the probability of being missing is dependent on the attribute and values in important attributes are more likely to missing. Following this example, we would like to inject missing values according to attribute importance. Specifically, we weight each attribute $A_i$ by the accuracy decrease $\delta_{A_i}$ of removing the attribute in a KNN classification task. Next, we normalize the weights to be $\delta_{A_i}'=\delta_{A_i}/\sum_j^M \delta_{A_j}$ to represent the importance of each attribute, where $M$ is the number of attributes. We inject missing value to each cell of attribute $A_i$ with a probability of $Mr_{\text{mv}}\delta_{A_i}'$, ensuring the overall missing rate to be $r_{\text{mv}}$.

%\item MNAR. In this type, for each cell, the probability of being missing is dependent on the unobserved data or the missing value itself. For simplicity, we would like to design an injection strategy so that the probability of missing to be dependent on the value of each cell. To achieve this, we first measure the impact of the value in each cell $(i,j)$ by the accuracy decrease $\delta_{i,j}$ of classifying tuple $i$ using KNN when replacing the value with NaN (which is repaired by filling in the mean for numeric attribute or majority class for categorical attribute). Next, we normalize the weights to be $\delta_{i,j}'=\delta_{i,j}/(\sum_i^N\sum_j^M \delta_{i,j})$. We insert missing value to each cell $(i,j)$ with a probability of $MNr_{\text{mv}}\delta_{i,j}'$, ensuring the overall missing rate to be $r_{\text{mv}}$.
 
%\end{itemize}


\stitle{Cleaning Algorithms Compared.} We compare the following approaches for handling missing values in the training data.
\begin{itemize}[leftmargin=*]
   \item \underline{\emph{Ground Truth}}: This method uses the ground-truth version of the dirty data, and shows the performance upper-bound. %In other words, it uses a human cleaner to clean 100\% of all dirty records. 
    \item \underline{\emph{Default Cleaning}}: This is the default and most commonly used way for cleaning missing values in practice, namely, missing cells in a numerical column are filled in using the mean value of the column, and those in a categorical column are filled using the most frequent value of that column.
     \item \underline{\emph{CPClean}}: This is our proposal, which needs a candidate repair set $\mathcal{C}_i$ for each example with missing values. For missing cells in numerical columns, we consider five candidate repairs: the minimum value, the 25-th percentile, the mean value, the 75-th percentile and the maximum value of the column. For missing cells in categorical columns, we also consider five candidate repairs: the top 4 most frequent categories and a dummy category named ``other category". If a record $i$ has multiple missing values, then the Cartesian product of all candidate repairs for all missing cells forms $\mathcal{C}_i$. 
     We simulate human cleaning by picking the candidate repair that is closest to the ground truth.
     %Recall that \at{CPClean} only cleans a fraction of data examples defined by the cleaning strategy $\pi$. For the remaining uncleaned cells, we can use any candidate repairs. In our experiments, we fill in the uncleaned cells with the default cleaning method.
    \item \underline{\emph{HoloClean}}: This is the state-of-the-art probabilistic data cleaning method~\cite{rekatsinas2017holoclean}. 
    As a weakly supervised machine learning system, it leverages multiple signals (e.g. quality rules, value correlations, reference data) to build a probabilistic model for imputing and cleaning data. Note that the focus of HoloClean is to find the most likely fix for a missing cell in a dataset without considering how the dataset is used by downstream classification tasks.  
    \item \underline{\emph{BoostClean}}: This is the state-of-the-art automatic data cleaning method for ML~\cite{krishnan2017boostclean}. At a high level, it selects, from a predefined set of cleaning methods, the one that has the maximum validation accuracy on the validation set. To ensure fair comparison, we use the same cleaning method as in CPClean, i.e., the predefined cleaning methods include cleaning a numerical column with missing values using 25-th percentile, the mean value, etc. We also use the same validation set as in CPClean.
    \item \underline{\emph{RandomClean}}: While CPClean uses the idea of sequential information maximization to select which examples to clean, \emph{RandomClean} simply selects an example randomly  to clean.  
    
    %This is the state-of-the-art automatic data cleaning method for ML~\cite{krishnan2017boostclean}. At a high level, it selects, from a predefined set of cleaning methods, the one that has the maximum validation accuracy on the validation set. To ensure fair comparison, we use the same cleaning method as in CPClean, i.e., the predefined cleaning methods include cleaning a numerical column with missing values using 25-th percentile, the mean value, etc. We also use the same validation set as in CPClean.
    
    %It  automatically selects an ensemble of error detection and repair combinations using statistical boosting. 
    
    
    %Recall that our algorithm can return any world among all partially cleaned possible worlds.  
    %After all validation examples are CP'ed, we can return any one of the worlds from the resulting space. In other words, we can impute the remaining missing cells with any candidates.

    %set the parameter in the stopping criteria to be 10.
    %We will also compare different versions: \emph{CC-Entropy}  \emph{CC-Random} 
    % \item \emph{ActiveClean (AC)}: 
    % \item \emph{Random Cleaning (RC)}: In each iteration, this method randomly picks a dirty example to clean until all examples are cleaned. We run this method 20 times and report the average result.
    %and it stops when all the examples are cleaned.
\end{itemize}

\stitle{Performance Measures.} Besides the cleaning effort spent, we are mainly concerned with the test accuracy of models trained on datasets cleaned by different cleaning methods. Instead of reporting exact test accuracies for all methods, we only report them for \emph{Ground Truth} and \emph{Default Cleaning}, which represents the upper bound and the lower bound, respectively. For other methods, we report the percentage of closed gap defined as:
\begin{small}
    $$ \textit{gap closed by X} = \frac{\text{ accuracy(X) -  accuracy(\emph{Default Cleaning})}}{\text{ accuracy(\emph{Ground Truth}) -  accuracy(\emph{Default Cleaning})}}.$$
\end{small}{}

%There are two main performance measures we evaluate: 

% \begin{itemize}
%     \item \emph{Accuracy:} the accuracy of the downstream KNN model on unseen test data. In the algorithms compared, \emph{GT} and \emph{DC} usually has the highest test accuracy and the lowest test accuracy respectively, while other methods usually lie in the \textit{gap} of \emph{DC} and \emph{GT}. To have a better comparison between different methods, we compute the percentage of \textit{gap closed} by each method, which is defined as follow:
%     %we scale the test accuracy using the test accuracy of  \emph{DC} and \emph{GT}. 
%     $$ \textit{gap closed \%} = \frac{\text{Test accuracy - \emph{DC} Test accuracy}}{\text{\emph{GT} test accuracy - \emph{DC} Test accuracy}} \times 100\%$$
%     We report the test accuracy of \emph{GT} and \emph{DC} and for other methods, we report the percentage of \textit{gap closed}.
%     \item \emph{Cleaning efforts}: the number of examples cleaned by human. We report the percentage of dirty examples cleaned in our experiments. 
% \end{itemize}

% ; and (3) the \emph{running time} of different cleaning algorithms.

\subsection{Experimental Results}
\label{subsec:end-to-end}

\begin{table*}[!ht]
\centering
\scalebox{0.65}{
\begin{tabular}{c|cc|c|c|cc|cc}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \emph{Ground Truth} & \emph{Default Cleaning} & \emph{BoostClean} & \emph{HoloClean} & \multicolumn{4}{c}{\emph{CPClean}}
\\ \cline{2-9} 
 & \textbf{Test Accuracy} & \textbf{Test Accuracy} & \textbf{Gap Closed} & \textbf{Gap Closed} & \textbf{Gap Closed } & \textbf{Examples Cleaned } 
 &
 \textbf{Gap Closed } &
 \textbf{Examples Cleaned }
 \\ \hline
BabyProduct & 0.668 & 0.589 & 1\% & 1\% & 99\% & 64\% & 72\% & 20\% \\ 
Supreme & 0.968 & 0.877 & 12\% & -4\% & 100\% & 15\% & 100\% & 20\% \\ 
Bank & 0.643 & 0.558 & 20\% & 11\% & 102\% & 93\% & 52\% & 20\% \\ 
Puma & 0.794 & 0.747 & 28\% & -64\% & 102\% & 63\% & 40\% & 20\%\\ \hline
\end{tabular}
}
\caption{End-to-End Performance Comparison}
\label{table:end_to_end_performance}
% \vspace{-6mm}
\end{table*}
% \begin{table*}[!ht]
% \centering
% \scalebox{0.8}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{1}{|l|}{\multirow{}{}{\textbf{Dataset}}} & \textbf{GT} & \textbf{DC} & \textbf{BC} & \textbf{HC} & \multicolumn{2}{c|}{\textbf{CP}} & \multicolumn{2}{c|}{\textbf{CP-Early Stopping}} \\ \cline{2-9} 
% \multicolumn{1}{|l|}{} & \textbf{\begin{tabular}[c]{@{}c@{}}Test \\ Accuracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Test \\ Accuracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gap \\ Closed (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gap \\ Closed (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gap \\ Closed (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\ Examples \\ Cleaned (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gap \\ Closed (\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# Examples \\ Cleaned (\%)\end{tabular}} \\ \hline
% Supreme & 0.968 & 0.877 & 12\% & -4\% & 100\% & 15\% & 55\% & 1\% \\ \hline
% Bank & 0.643 & 0.558 & 20\% & 11\% & 102\% & 93\% & 52\% & 17\% \\ \hline
% BabyProduct & 0.667 & 0.589 & 1\% & 1\% & 99\% & 64\% & 82\% & 10\% \\ \hline
% Puma & 0.794 & 0.747 & 28\% & \textcolor{red}{?}\% & 102\% & 63\% & \% & \% \\ \hline
% \end{tabular}
% }
% \caption{End-to-End Performance of CC and Automatic Cleaning Methods}
% \label{table:end_to_end_performance}
% \end{table*}

\stitle{Model Accuracy Comparison.} Table \ref{table:end_to_end_performance} shows the end-to-end performance of our method and other automatic cleaning methods. We can see that the missing values exhibit different degress of impact on these datasets (the gap between \emph{Ground Truth} and \emph{Default Cleaning}). We can also observe that \emph{HoloClean}, the state-of-the-art standalone data cleaning approach performs poorly --- the gap closed can even be negative. This suggests that performing data cleaning on a data without considering how it is used later may not necessarily improve downstream model performance. On the other hand, we observe that \emph{BoostClean} shows a consistently positive impact on model performance by using the validation set to pick the most useful cleaning method. In all cases, \emph{CPClean} is able to close ~100\% of gap without manual cleaning of all dirty data. In fact, on \at{Supreme}, \emph{CPClean} only requires the manual cleaning of 15\% of missing records to close 100\% gap. We can also see from Table \ref{table:end_to_end_performance} that, by cleaning only 20\% of all dirty data, i.e., terminating the cleaning process at 20\% mark even if not all validation examples are CP'ed, \emph{CPClean} is able to close 66\% gap on average. 


%As we can see, although BoostClean (BC) and HoloClean (HC) are automatic cleaning methods which requires no human cleaning effort, they can only close a small portion of the gap. In Supreme and Puma, the gap closed by HoloClean is even negative. This is because the values imputed with HoloClean in these datasets are far away from the ground truth, which makes the performance even worse than the default cleaning method. However, by cleaning a fraction of the data, our algorithm can close almost 100\% of the gap for all the datasets. For example, for Supreme, CPClean closes 100\% of the gap by cleaning only 15\% of the dirty data. In other words, the classifier trained on the output dataset of CPClean with 15\% of dirty data cleaned is as good as the classifier trained on the ground truth dataset that requires to clean all the data.  Therefore, our algorithm dramatically outperforms other cleaning methods.


% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/entropy_vs_random/Supreme_MAR_cc_acc.png} 
%     \caption{Supreme}
%     \end{subfigure}
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/entropy_vs_random/Bank_MAR_cc_acc.png}  
%     \caption{Bank}
%     \end{subfigure}
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/entropy_vs_random/BabyProduct_real_cc_acc.png} 
%     \caption{BabyProduct}
%     \end{subfigure}
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/entropy_vs_random/puma8NH_MAR_cc_acc.png} 
%     \caption{Puma}
%     \end{subfigure}
%     \vspace{-3mm}
%     \caption{Comparison with Random Cleaning}
%     \vspace{-4mm}
%     \label{fig:cc_vs_random_cc_acc}
% \end{figure}


\begin{figure}[t!]
    \label{fig:vary_val}
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/\figfmt/comparison-with-random-cleaning}
    % \vspace{-10mm}
    \caption{Comparison with Random Cleaning}
    % \vspace{-4mm}
    \label{fig:cc_vs_random_cc_acc}
\end{figure}{}

\stitle{Early Termination.} If users have a limited cleaning budget, they may choose to terminate \emph{CPClean} early. To study the effectiveness of \emph{CPClean} in prioritizing cleaning effort, we compare it with \emph{RandomClean} that randomly picks an example to clean at each iteration. The results for \emph{RandomClean} are the average of 20 runs.
%To study the effectiveness of our algorithm for making all examples in $D_{val}$ CP'ed and improving the test accuracy, we next compare our algorithm with random cleaning, where at each iteration, we randomly select a dirty example to clean until all the validation examples become CP'ed. We run the random cleaning 20 times and report the average results.

The red lines in Figure \ref{fig:cc_vs_random_cc_acc} show the percentage of CP'ed examples in the validation set as more and more examples are cleaned. As we can see, \emph{CPClean} (solid red line) dramatically outperforms the \emph{RandomClean} (dashed red line) both in terms of  the number of training examples cleaned so that all validation examples are CP'ed and in terms of the rate of convergence. For example, for \at{Supreme}, \emph{CPClean} requires the cleaning of 15\% examples while \emph{RandomClean} requires cleaning almost all training examples. 

%. With the same number of cleaning examples, our algorithm always make much more validation examples CP'ed than random cleaning. To make the entire validation CP'ed, random cleaning needs to clean almost all the data, while our algorithm only needs to clean a fraction of the data. 

The blue lines in Figure \ref{fig:cc_vs_random_cc_acc} show the percentage of gap closed for the test set accuracy. Again, we can observe that \emph{CPClean} significantly outperforms \emph{RandomClean}. 
%of our method and random cleaning with an increasing number of examples cleaned. 
%As we can see, our method generally can close much more gap than random cleaning with the same number of cleaned examples. 
For example, with 50\% of data cleaned in 
\at{Bank}, \emph{RandomClean} only closes about 65\% of the gap, whereas \emph{CPClean} closes almost 100\% of the gap. 
%Therefore, in practice, if the budget of cleaning effort is not enough for CPClean to make all examples CP'ed, CPClean is still useful. In this case, we can stop the algorithm earlier as there is no cleaning budget. Although the output dataset is not guaranteed to be as good when the ground truth dataset, it performs much better than randomly cleaning the same number of examples in the dataset.


% Therefore, our algorithm can dramatically outperform them with a small amount of human cleaning. 

% with only cleaning a fraction of the data. 
%  The classifier trained on the output dataset of $CPClean$ closes 100\% gap, which means the test accuracy is as good as \emph{GT}, which needs to clean all the data.  Although Boost Clean and HoloClean requires no human cleaning effort, Boost Clean closes 12\% gap and HoloClean even performs worse than default cleaning. However, our method 

% \stitle{Early stopping.} 
%With early stopping criteria (CP-Early Stopping), the cleaning effort can be reduced significantly, while we can still close a large percentage of the gap. For example, in BabyProduct dataset, we can close 82\% of the gap by cleaning only 10\% of data. A

\iffalse
\begin{table}[!h]
\centering
\scalebox{0.7}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \textbf{Q1} & \multicolumn{3}{c|}{\textbf{Q2}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}CPClean \\ (per iteration)\end{tabular}}} \\ \cline{2-5}
 & \textbf{MinMax} & \textbf{SortCount} & \textbf{SortCountDP} & \textbf{SortCountDPDC} &  \\ \hline
BabyProduct & 0.006s & \textgreater{}100s & 7s & 0.3s & 3s \\ \hline
Supreme & 0.007s & \textgreater{}100s & 9s & 0.6s & 35s \\ \hline
Bank & 0.004s & \textgreater{}100s & 8s & 0.5s & 9s \\ \hline
Puma & 0.02s & \textgreater{}100s & \textgreater{}100s & 6.2s & 50s \\ \hline
\end{tabular}
}
\caption{Running time \textcolor{red}{maybe we can remove this?}}
\label{table:running time}
\end{table}

\stitle{Efficiency of Answering Q1 and Q2:} \xc{@Peng, rmember to update this when text is fixed.} Table \ref{table:running time} shows the time of running queries on one validation example and the time of one iteration of CPClean. As we can see, for Q1, the running time of MinMax algorithm is less than 0.02 seconds; For Q2, the original SortCount takes a long time. With our optimization using dynamic programming (SortCountDP), the running time is reduced to about 10 seconds for datasets with about 3000 examples.  With our optimization using a binary tree (SortCountDPDC), the running time is further reduced to less than 1 seconds for datasets with 3000 examples and about 6 seconds for datasets with 8000 examples.

Q1 and Q2 are used to pick an example to clean at each iteration of \emph{CPClean}. We hence also report the average running time for selecting an example at each iteration in \emph{CPClean}. As shown in Table \ref{table:running time}, the time \emph{CPClean} spends in picking an example is acceptable, considering human cleaning usually incurs high costs (we spent about  3 minutes per record on averagein manually cleaning  \at{BabyProduct}). 

\fi

%the time needed for cleaning the selected example by human (about 3 minutes in our experiments). 
%is 35 seconds for Supreme, 3 seconds for BabyProduct, 9 seconds for Bank and 50 seconds for Puma. We think this is acceptable considering the time needed for cleaning the selected example by human (about 3 minutes in our experiments). 

\begin{figure}[t!]
    \label{fig:vary_val}
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/\figfmt/varying-validation-set-size}
    % \vspace{-10mm}
    \caption{Varying size of $D_{val}$.}
    \label{fig:vary_val}
\end{figure}{}

\stitle{Size of the Validation Set $D_{val}$.}  We vary the size of $D_{val}$ to understand how it affects the result. As shown in Figure \ref{fig:vary_val}, as the size of validation set increases, both the test accuracy gap closed and the cleaning effort spent first increase and then become steady. This is because, when the validation set is small, it is easier to make all validation examples CP'ed (hence the smaller cleaning effort). However, a small validation set may not be representative of some unseen test set, and hence may not close the accuracy gap on test set. In all cases, we observe that 1K validation set is sufficiently large and further increasing it does not improve the performance.

%Therefore, by making all validation examples CP'ed, even though CPClean has the same validation accuracy as the ground truth, its test accuracy may not be as good as the ground truth. For all datasets in our experiments, when the size is greater than $1000$, the gap closed is close to 100\% and the performance of CPClean becomes insensitive to the size of validation set.




% We vary the hyperparameter for early stopping to understand how the results will be affected. Recall that our algorithm stops when the validation accuracy does not increase by $T$ iterations. Figure \ref{fig:early_stop_hyperparameter} shows the percentage of gap closed and examples cleaned varying $T$. As expected, when we increase $T$, the number of cleaned examples will also be increased since the stopping criteria becomes stricter. We observe that the gap closed by our algorithm will only increase or keep constant as $T$ increases. Therefore, in practice, we can set $T$ to be as large as possible based on our cleaning budget. 

% \begin{figure*}[!h]
%     \centering
%     \begin{subfigure}{.5\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/early_stop/Supreme_early_stop.png}  
%     \caption{Supreme}
%     \end{subfigure}
%     \begin{subfigure}{.5\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/early_stop/Bank_early_stop.png}  
%     \caption{Bank}
%     \end{subfigure}
%     \begin{subfigure}{.5\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/early_stop/BabyProduct_early_stop.png}  
%     \caption{BabyProduct}
%     \end{subfigure}
%     \caption{Varying Hyperparameter for Early Stopping}
%     \label{fig:early_stop_hyperparameter}
% \end{figure*}





%stop the algorithm earlier and this . 


% In BabyProduct, we observe that the performance of random cleaning can drop significantly from cleaning 50\% examples to 60\% examples, which may be caused by Simpson's Paradox mentioned in \cite{krishnan2016activeclean}. However, the performance our method does not have significant drop as cleaning more and more examples.

 
%  \begin{figure*}[!ht]
%     \centering
%     \begin{subfigure}{.5\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/entropy_vs_random/Supreme_MAR_cc.png}  
%     \caption{Supreme}
%     \end{subfigure}
%     \begin{subfigure}{.5\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/entropy_vs_random/Bank_MAR_cc.png}  
%     \caption{Bank}
%     \end{subfigure}
%     \begin{subfigure}{.5\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/entropy_vs_random/BabyProduct_real_cc.png}  
%     \caption{BabyProduct}
%     \end{subfigure}
%     \caption{Optimization Performance Comparison with Random Cleaning}
%     \label{fig:cc_vs_random_cc}
% \end{figure*}






% \xc{Table or graph: show the end-to-end test accuracy of all competing methods. Show the test accuracy for DC and GT, but for other cleaning methods, show the gap closed. 
% For CC, we need to pick a $\alpha$ and $\rho$ that is reasonable as the default setting that works for all datasets. For CC, we not only need to show the test accuracy, but also the percentage of dirty records cleaned.}



% \begin{table}[!h]
% \centering
% \scalebox{0.7}{
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multirow{ }{}{Dataset} & \multirow{ }{}{\begin{tabular}[c]{@{}c@{}}Injection\\ Method\end{tabular}} & \multirow{}{}{Gap} & BC & \multicolumn{2}{c|}{CC} \\ \cline{4-6} 
%  &  &  & \begin{tabular}[c]{@{}c@{}}Gap Closed \\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Gap closed \\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\# Cleaned \\ Examples (\%)\end{tabular} \\ \hline
% kin8nm & MCAR & 0.06 & NA & 33\% & 57\% \\ \hline
% kin8nm & MAR & 0.095 & 26\% & 79\% & 51\% \\ \hline
% kin8nm & MNAR & 0.085 & NA & 29\% & 62\% \\ \hline
% puma8NH & MCAR & 0.005 & NA & 500\% & 54\% \\ \hline
% puma8NH & MAR & 0.115 & 0\% & 61\% & 56\% \\ \hline
% puma8NH & MNAR & 0.105 & 19\% & 48\% & 58\% \\ \hline
% BabyProduct & real & 0.115 & 50\% & 108\% & 48\% \\ \hline
% \end{tabular}
% }
% \end{table}

% \xc{Explanation: The main point of this experiment is to show that CC is able to close most of the gap and cleans only a fraction of the data. We also need to explain the intricacies and differences in performance in different datasets.}

% \stitle{End-to-end for Logistic Regression.} \xc{Table or graph: use the cleaned dataset via KNN to train another ML model LR. Here, we should add comparison with AC. Same type of table/figure as above.}

% \xc{Explanation: the point here is to show that though we only support KNN, the cleaned dataset can be used for training other downstream ML models, and it hopefully still outperforms cleaning algorithms specifically designed for LR such as AC.}

% \subsection{Evaluating the Decision Problem}
% \label{subsec:decision-evaluation}

% \stitle{Accuracy of Our Sampling Algorithm.} To study the accuracy of our virtual sampling algorithm, we compare it with the physical sampling algorithm. The physical sampling algorithm randomly samples a number of worlds (e.g. $1000$) from the space and then counts the percentage of worlds having validation accuracy greater than a threshold. Figure \ref{fig:virtual_vs_real} shows the results of two methods on the BabyProduct dataset with different thresholds. As we can see, the results of the virtual sampling are very close to the results of the physical sampling, suggesting that our virtual sampling algorithm is almost as good as the physical sampling algorithm in terms of estimating the probability.

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=.6\columnwidth]{Figures/vitual_vs_real.png}
%     \caption{Virtual Sampling vs. Physical Sampling}
%     \label{fig:virtual_vs_real}
% \end{figure}



% \xc{The point of this experiment is to show that even though we do not require physical sampling of all possible worlds, our virtual sampling is almost as good as the physical sampling algorithm in terms of estimating the percentage of worlds having validation accuracy greater than some threshold.}

% \stitle{Goodness of the Decision.} We vary the accuracy improvement $\alpha$ to show the effectiveness of decision probability. The results for different datasets with different types of injection are shown in Figure \ref{fig:decision_goodness}. As expected, the probability decreases as $\alpha$ increases. For each synthetic dataset, we observe that with the same $\alpha$, MNAR always has the highest probability, while MNAR always has the lowest probability, which suggests that the accuracy is more likely to be improved by cleaning missing values with MNAR injection and less likely to be improved by cleaning missing values with MCAR injection. Also, we notice that datasets that have a large gap between ground truth and default cleaning tend to have a larger probability. For example, BabyProduct has a larger gap than puma8NH and its probability tends to be higher. Note that the distribution of missing values or the gap is unknown before the data is cleaned. However, the decision probability provides a good measurement about them. Using the decision probability, the user can easily make decision about whether to clean the data. For example, consider $\rho = 0.5$ on BabyProduct datset, which means the the user would like to clean the data if the probability of achieving the goal is greater than 50\%. If $\alpha = 0.1$, which means user's goal is to improve the accuracy by 10\% and, the decision probability would suggest the user clean the data, but if $\alpha = 0.2$, which means user's goal is to improve the accuracy by 20\%, the decision probability would suggest the user not clean the data.


% and the probability tends to decrease faster when missing values have a large impact on the ML models (i.e. the gap between ground truth and default clean is large). 
% \begin{figure}[!h]
%     \centering
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/decision_goodness/puma8NH.png}  
%     \caption{}
%     \end{subfigure}
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/decision_goodness/kin8nm.png}  
%     \caption{}
%     \end{subfigure}
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/decision_goodness/BabyProduct.png}  
%     \caption{}
%     \end{subfigure}
%     \caption{Decision Probability}
%     \label{fig:decision_goodness}
% \end{figure}{}

% \xc{Varying $\alpha$ and varying $\rho$ here to show that the cleaning decision can change depend on user expectations. } 

% \xc{Show for different $\alpha$ and different $\rho$, we may stop early in the cleaning process, but will end up with lower test accuracy. } 

% \begin{figure}[!h]
%     \centering
%     \begin{subfigure}{.49\columnwidth}
%     \includegraphics[width=\columnwidth]{Figures/entropy_vs_random/BabyProduct.png} 
%     \caption{C.C.}
%     \label{fig:entropy_vs_random_cc}
%     \end{subfigure}
%     \caption{Compare CC and CC-Random}
%     \label{fig:entropy_vs_random}
% \end{figure}{}

% \xc{Graph here: x-axis is the number of cleaned examples, y-axis here is the percentage of validation examples that are consistently classified. Maybe a second y-axis here to show the computation time elapsed to show that CC-TopK is much faster than CC.} 

% \xc{Another graph here: x-axis here is the number of cleaned examples, and y-axis is the test accuracy. Not sure if this is necessary, maybe only show early stopping as below if this graph is not good.}



% %We start by evaluating the accuracy and efficiency of our algorithms on three queries. Then we present end-to-end experiments to see whether the results from these queries can guide data cleaning for machine learning.


% \subsection{Expected Outcomes of Experiments by Xu}

% In terms of end to end experiments: 
% \begin{itemize}

% \item Datasets: take a clean dataset, inject missing values using different distributions. These are going to be synthetic datasets with known ground-truth. 

% ML algorithms: try different ML algorithms. DT, KNN, LR

% \item Compared with NoClean (dirty data), ideally, we want to show that BoostClean, ActiveClean, CCClean, and NaiveClean (cleaning using a common default method like mean imputation) all does better. And ground-truth clean data ideally would lead to the best accuracy. Compared with BoostClean, ActiveClean, we want to show we need to clean a lesser number of records and achieve a higher end model accuracy.

% \item For those datasets, where cleaning ends up to be not producing better results, we want to show that our "feasibility" question is able to capture it, i.e., for every experiment, attach the feasibility score to it. 

% \item We also would like to do experiments on datasets with no known ground-truth. The idea is to take a dataset in a public domain (e.g., Movie), and create a classification task. In order to come up with candidate fixes for a dataset, you can use all the known domain values, or values from another table in an ER dataset.  The key is to make sure that the ground-truth is likely to be present in the candidates fixes presented to the users. The ground-truth missing values in movies should be easy to identify by users. 

% \item We can also show that a dataset cleaned with kNN classifier would also produce better results for other classifiers. 



% \end{itemize}


% In terms of experiments to test properties of our algorithms.

% \begin{itemize}
% \item Approximate algorithms give good guarantees when we increase sample size. for computing feasibility answers

% \item Test different versions of cleaning (top-k v.s. entropy), show the trade-off. 
% \end{itemize}

% \subsection{Setup}

% \stitle{Datasets:} We downloaded 8 classification datasets from Kaggle competitions and UCI repository. The details of each dataset are shown in \Cref{table:datasets}.

% \begin{savenotes}
% \begin{table}[!h]
% \centering
% \caption{Datasets}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{Datasets} & \textbf{\#examples} & \textbf{\#features} & \textbf{\#classes} \\ \hline
% Titanic\footnote{https://www.kaggle.com/c/titanic} & 891 & 11 & 2 \\ \hline
% Housing\footnote{https://www.kaggle.com/c/house-prices-advanced-regression-techniques} & 1,460 & 80 & 2 \\ \hline
% EEG\footnote{https://archive.ics.uci.edu/ml/datasets/EEG+Eye+State}& 14,980 & 14 & 2 \\ \hline
% USCensus\footnote{https://archive.ics.uci.edu/ml/datasets/census+income} & 32,561 & 14 & 2 \\ \hline
% Physics\footnote{https://www.kaggle.com/c/flavours-of-physics/} & 67,553 & 50 & 2 \\ \hline

% \end{tabular}
% \label{table:datasets}
% \end{table}
% \end{savenotes}

% \stitle{Errors:} We consider missing values and outliers. We injected missing values or outliers into the training set in each dataset. We randomly select 5\% entries in the training sets and replace them with NaN for missing values or 3 times the highest feature value for outliers.

% \stitle{ML Models:} For general classifier, we consider both Logistic Regression, SVM, DT and KNN (K=3). 

% \stitle{Training:} We split each dataset into train/val/test sets by 60\%/20\%/20\%. We used scikit-learn to train models.

% \stitle{Repairing:} For numerical features, 5 values from min to max.  For categorical features, 5 most frequent classes.


% % \textbf{Logistic Regression:}
% % Logistic regression is a binary classifier that uses a Sigmoid function to create a linear classification boundary. Logistic regression uses optimization methods to determine the best regression coefficient of the function based on the training data . 
% % \\
% % \textbf{KNN Classifier:}
% % KNN classifier uses a distance metric (Euclidean distance in our experiments), and the number of nearest neighbors ($k$) to calculate the distance between records in the training set. After calculating the distance it then retrieves the $k$ nearest neighbors. Once the algorithm has found those neighbors, it can classify a record in the test set by computing its distance to other training records and using the class labels of the nearest neighbors to determine the label class of the unknown record \cite{hastie1996discriminant}.  


% % We select 5 UCI  Each dataset is described as follows.

% % \noindent
% % \textbf{EEG:} This is a dataset of 14,980 EEG recordings. Each record has 14 EEG attributes. The classification task is to predict whether the eye-state is closed or open. This dataset contains numerical outliers. We inject mislabels into this dataset by randomly flip labels. 

% % \noindent
% % \textbf{USCensus:}  This dataset contains 32,561 US Census records for adults. Each record has 14 attributes including age, education, sex, etc. The classification goal is to predict whether the adult earns more than \$50,000. This dataset contains missing values. 

% % \noindent
% % \textbf{Titanic:}  This dataset contains 891 records and 11 attributes from the Titanic including name, sex, age, etc. The classification task is to determine whether the passenger survived or not. This dataset has a significant number of missing values.

% % \noindent
% % \textbf{Marketing:} This dataset consists of 8,993 data about household income from a survey. Each record has 14 demographic attributes including sex, age, education, etc. The classification task is to predict if the annual household income is less than \$25000. This dataset contains missing values.

% % \noindent
% % \textbf{Sensor:} The original sensor dataset contains 928,991 sensor recordings with eight attributes including temperature, humidity, light, etc. Because of the large size, we only used recordings from sensor 1 and sensor 2 and sampled the dataset to include 1 observation per hour, and day for each sensor. The sampled dataset contains 62,076 records. The classification task is to predict whether the readings came from a particular sensor (sensor 1 or sensor 2). This dataset contains outliers.


% \subsection{3 Queries}

% \subsubsection{Methods}

% For Q1 and Q2, we compare the following methods:

% \begin{itemize}
%     \item Approximate Algorithm
%     \item Exact Solution. For general classifier, we set p = 1000 to estimate the exact solution. For KNN, we use the results from efficient KNN algorithms.
    
% \end{itemize}

% For Q3, we consider the following methods:

% \begin{itemize}
% \item Random selection
% \item Minimum Expected Entropy
% \item Top K in best scenario (KNN only)
% \item Minimum True Entropy (KNN only)
% \end{itemize}


% \subsubsection{Evaluation Metrics}
% We evaluate the algorithms of three queries using the test set. 

% \begin{itemize}
%     \item For Q1, since approximate algorithm can only produce false positives, we use false positive rate to evaluate the accuracy of the approximate algorithm.
%     \item For Q2, we use the average difference of entropy. 
%     \item For Q3, we use the average number of examples to clean.
% \end{itemize}

% \subsubsection{Results}



% \subsection{End-to-end Experiments}
% \subsubsection{Methods}
% We compare the following methods:

% \begin{itemize}
%     \item Dirty 
%     \item Oracle
%     \item Classical Cleaning (Mean, Median imputation... )
%     \item KNN Q3 results by making validation set C.C..
%     \item Logistic Regression Q3 results by making validation set C.C..
%     \item Active Clean with Logistic Regression
%     \item Boost Clean
% \end{itemize}{}
% \subsubsection{Evaluation Metrics}

% To evaluate the end to end performance, we use accuracy and examples to clean.

% \subsubsection{Results}

% \stitle{Logistic Regression}


% \stitle{KNN}

==> [arXiv] Certain Prediction/GenericSolution.tex <==
% !TEX root = CC.tex
\section{Application: Data Cleaning for ML}\label{sec:cc:general}

In this section, we show how to use the proposed CP framework to design an effective data cleaning solution, called \at{CPClean}, for the important application of data cleaning for ML. We assume as input a dirty training set $\mathcal{D}_{train}$ with unknown ground truth $D^*$ among all
possible worlds $\mathcal{I}_\mathcal{D}$. 
Our goal is to select a version $D$ from $\mathcal{I}_\mathcal{D}$, such that
the classifier trained on 
$\mathcal{A}_D$ has the 
same validation accuracy as the classifier trained on the ground
truth world $\mathcal{A}_{D^*}$. 

\stitle{Cleaning Model.} 
Given a dirty dataset $\mathcal{D} = \{(\mathcal{C}_i, y_i)\}_{i\in[N]}$,
in this paper, we focus on the 
scenario in which 
the candidate set $\mathcal{C}_i$
for each data example
is created by automatic data 
cleaning algorithms or
a predefined noise model. For each 
uncertain data example $\mathcal{C}_i$,
we can ask a human 
to provide its true value $x_i^* \in \mathcal{C}_i$. Our goal is 
to find a good strategy to prioritize 
which dirty examples to be cleaned. That is, a cleaning strategy of
$T$ steps can be defined as
\[
\pi \in [N]^T,
\]
which means that in the first
iteration, we clean the example 
$\pi_1$ (by querying human to obtain the ground
 truth value of $\mathcal{C}_{\pi_1}$;
 in the second iteration, we
 clean the example 
$\pi_2$; and so on.
%%%
Applying a cleaning strategy $\pi$ will generate  a \textit{partially
cleaned} dataset $\mathcal{D}_{\pi}$
in which all cleaned candidate
sets $\mathcal{C}_{\pi_i}$
are replaced by $\{x_{\pi_i}^*\}$.

% \paragraph*{Principle: Entropy
% Minimization}
% The theory of submodular functions enables the analysis for the performance of the most informative selection policies. Several studies have applied such theory to identify near optimal solutions to information gathering problem, and show that exploiting information measures is beneficial~\cite{Krause2014SubmodularFM, Fujii, Esfandiari2019AdaptivityIA, ChenK13, Dasgupta2004AnalysisOA,ZhengAlice2012Entropy}.
% %, including~\cite{Krause2014SubmodularFM, Fujii, Esfandiari2019AdaptivityIA, ChenK13, Dasgupta2004AnalysisOA} and~\cite{ZhengAlice2012Entropy}. 
% In the context of data cleaning, the mutual information violates the adaptive submodularity condition. We, in this work, leverage of the theory of {\it sequential information maximization} introduced by~\cite{Chen2015SequentialIM}, and adapt its information gathering strategy for data cleaning. 

\stitle{Formal Cleaning Problem Formulation.} The question we need to address is \textit{"What is a successful cleaning
strategy?"} Given a validation set
$D_{val}$, the view of \at{CPClean} 
is that a successful cleaning strategy
$\pi$ should be the one that 
produces a partially cleaned 
dataset $\mathcal{D}_\pi$ in which 
all validation examples $t \in D_{val}$
can be certainly predicted.
In this case, picking any
possible world defined by 
$\mathcal{D}_\pi$, i.e., $\mathcal{I}_{\mathcal{D}_\pi}$,
will give us a dataset that
has the same accuracy, on the
validation set, as the ground truth world
$D^*$. This can be defined
 precisely as follows.

We treat each candidate set
$\mathcal{C}_i$ as a random variable
$\mathbf{c}_i$, taking values in 
$\{x_{i, 1}, ..., x_{i, M}\}$. 
We write $\mathbf{D} = \{
(\mathbf{c}_i, y_i)\}_{i \in [N]}$.
Given a cleaning strategy $\pi$
we can define the conditional entropy
of the classifier prediction 
on the validation set as
% \begin{eqnarray}
% & \mathcal{H}(
% \mathcal{A}_{\mathbf{D}}(D_{val})| 
% \mathbf{c}_{\pi_1} = x_{\pi_1}^*, ...,
% \mathbf{c}_{\pi_T} = x_{\pi_T}^*
% ) \\
% & \coloneqq 
% \frac{1}{|D_{val}|}\sum_{t \in D_{val}}
% \mathcal{H}(
% \mathcal{A}_{\mathbf{D}}(t)| 
% \mathbf{c}_{\pi_1} = x_{\pi_1}^*, ...,
% \mathbf{c}_{\pi_T} = x_{\pi_T}^*
% ) 
% \label{eqn:conditional_entropy}
% \end{eqnarray}

\begin{equation}
\mathcal{H}(
\mathcal{A}_{\mathbf{D}}(D_{val})| 
\mathbf{c}_{\pi_1}, ...,
\mathbf{c}_{\pi_T}
)
\coloneqq 
\frac{1}{|D_{val}|}\sum_{t \in D_{val}}
\mathcal{H}(
\mathcal{A}_{\mathbf{D}}(t)| 
\mathbf{c}_{\pi_1} , ...,
\mathbf{c}_{\pi_T} 
).
\label{eqn:conditional_entropy}
\end{equation}


Naturally, this gives us a principled
objective for finding a ``good''
cleaning strategy that minimizes the human cleaning effort: 
\begin{eqnarray*}
& \min_\pi & \text{dim}(\pi)\\
& s.t.,  &
% \mathcal{H}(
% \mathcal{A}_{\mathbf{D}}(D_{val})| 
% \mathbf{c}_{\pi_1} = x_{\pi_1}^*, ...,
% \mathbf{c}_{\pi_T} = x_{\pi_T}^*
\mathcal{H}(
\mathcal{A}_{\mathbf{D}}(D_{val})| 
\mathbf{c}_{\pi_1} = x_{\pi_1}^*, ...,
\mathbf{c}_{\pi_T} = x_{\pi_T}^*
) = 0.
\end{eqnarray*}
If we are able to find a cleaning 
strategy in which 
\[
\mathcal{H}(
\mathcal{A}_{\mathbf{D}}(D_{val})| 
\mathbf{c}_{\pi_1} = x_{\pi_1}^*, ...,
\mathbf{c}_{\pi_T} = x_{\pi_T}^*
) = 0,
\]
we know that this 
strategy would produce a partially 
cleaned dataset $\mathcal{D}_{\pi}$
on which all validation examples
can be CP'ed.
Note  that we can use 
the query $Q2$ to compute this conditional 
entropy:
\begin{equation*}
\mathcal{H}(
\mathcal{A}_{\mathbf{D}}(t)| 
\mathbf{c}_{\pi_1} = x_{\pi_1}^*, ...,
\mathbf{c}_{\pi_T} = x_{\pi_T}^*
)
~ =
-
\sum_{l \in \mathcal{Y}}
\frac{Q2(\mathcal{D}_\pi, t, y)}{|\mathcal{D}_\pi|} \log \frac{Q2(\mathcal{D}_\pi, t, y)}{|\mathcal{D}_\pi|}
\end{equation*}

\vspace{0.5em}
\noindent
{\bf Connections to ActiveClean.} 
The idea of prioritizing 
human cleaning effort for
downstream ML models is not new ---
ActiveClean~\cite{krishnan2016activeclean} explores
an idea with a similar goal. 
However, there are some
important differences 
between our framework and 
ActiveClean. The most 
crucial one is that 
our framework relies on 
\textit{consistency} of predictions
instead of the \textit{gradient},
and therefore, we do not
need labels for the
validation set and our algorithm can be used 
in ML models that cannot be 
trained by gradient-based
methods. The KNN classifier
is one such example. 
Since both frameworks 
essentially measure some
notion of ``local sensitivity,''
it is interesting future work 
to understand how to combine them.
%these two frameworks.

\subsection{The CPClean Algorithm} 
\label{sec:seq-info-max}

Finding the solution to the
above objective is, not
surprisingly, NP-hard~\cite{DBLP:journals/ior/KoLQ95}. In this paper, 
we take the view of 
sequential information maximization introduced by~\cite{Chen2015SequentialIM}
and \update{adapt} the \update{respective} greedy algorithm
for this problem. We first describe 
the algorithm, and then \update{review}
the theoretical analysis of its behavior.

\stitle{Principle: Sequential Information Maximization.}
Our goal is to find a cleaning
strategy that \textit{minimizes} the 
\textit{conditional entropy} as fast 
as possible. An equivalent view of 
this is to find a cleaning
strategy that \textit{maximizes}
the \textit{mutual information}
as fast as possible. 
% To see
% why this is the case, note that
% \begin{align*}
% % ~ & I(\mathcal{A}_{\mathbf{D}}(D_{val});
% % \mathbf{c}_{\pi_1}, ...,
% % \mathbf{c}_{\pi_T}
% % ) \\
% % = &
% % \mathcal{H}(
% % \mathcal{A}_{\mathbf{D}}(D_{val}))
% % - 
% % \mathcal{H}(
% % \mathcal{A}_{\mathbf{D}}(D_{val})| 
% % \mathbf{c}_{\pi_1} = x_{\pi_1}^*, ...,
% % \mathbf{c}_{\pi_T} = x_{\pi_T}^*
% % ) 
% & I(\mathcal{A}_{\mathbf{D}}(D_{val});
% \mathbf{c}_{\pi_1}, ...,
% \mathbf{c}_{\pi_T}
% ) \\
% & = 
% \mathcal{H}(
% \mathcal{A}_{\mathbf{D}}(D_{val}))
% - 
% \mathcal{H}(
% \mathcal{A}_{\mathbf{D}}(D_{val})| 
% \mathbf{c}_{\pi_1}, ...,
% \mathbf{c}_{\pi_T}
% ).
% \end{align*}
% where the first term 
% $\mathcal{H}(
% \mathcal{A}_{\mathbf{D}}(D_{val}))$
% is a constant independent of the
% cleaning strategy. 
% @Bojan
While we use the view of minimizing conditional entropy in implementing the CPClean algorithm, the equivalent view of maximizing mutual information will be useful in analyzing theoretical guarantees about CPClean.

Given 
the current $T$-step cleaning
strategy $\pi_1, ... ,\pi_T$, our goal 
is to greedily find the \textit{next}
data example to clean $\pi_{T+1} \in [N]$
that minimizes the
entropy conditioned on the partial observation as fast as possible:
\[
\pi_{T+1} = \arg\min_{i \in [N]}
\mathcal{H}(
\mathcal{A}_{\mathbf{D}}(D_{val})| 
\mathbf{c}_{\pi_1} = x_{\pi_1}^*, ...,
\mathbf{c}_{\pi_T} = x_{\pi_T}^*,
\mathbf{c}_{i} = x_{i}^*).
\]

%\vspace{0.5em}
\noindent
{\bf Practical Estimation.} The question thus becomes how to estimate
\[
\mathcal{H}(
\mathcal{A}_{\mathbf{D}}(D_{val})| 
\mathbf{c}_{\pi_1} = x_{\pi_1}^*, ...,
\mathbf{c}_{\pi_T} = x_{\pi_T}^*,
\mathbf{c}_{i} = x_{i}^*) ?
\]
The challenge is that when we are trying to decide which example to clean, we do not know the ground truth for item $i$, $x_i^*$. As a result, we need to
assume some priors on how likely
each candidate value $x_{i,j}$ 
is the ground truth $x_i^*$.
In practice, we find that a 
uniform prior already works well;
this leads to the following 
expected value:
\begin{align}
\frac{1}{M} \sum_{j \in [M]}
\mathcal{H}(
\mathcal{A}_{\mathbf{D}}(D_{val})| 
\mathbf{c}_{\pi_1} = x_{\pi_1}^*, ...,
\mathbf{c}_{\pi_T} = x_{\pi_T}^*,
\mathbf{c}_{i} = x_{i, j}).
\label{eqn:expected_entropy}
\end{align}
The above term can thus be calculated by invoking the $Q2$ query.% as discussed before.





\begin{algorithm}[t!]
\small
\caption{Algorithm \at{CPClean}.} \label{alg:ccclean}
\begin{algorithmic}[1]
\REQUIRE {$\mathcal{D}$, incomplete training set;  $D_{val}$, validation set.}
\ENSURE {$D$, a dataset in 
$\mathcal{I_{\mathcal{D}}}$ s.t. $\mathcal{A}_{D}$ and $\mathcal{A}_{D^*}$ have same validation accuracy}
\STATE $\pi \gets [ ]$

\FOR{$T = 0$ to $N-1$}

\IF{$D_{val}$ all CP'ed}
\STATE \textbf{break}
\ENDIF
    \STATE $min\_entropy \gets \infty$
    \FORALL{$i \in [N] \backslash \pi $}
    \STATE $entropy = \frac{1}{M} \sum\limits_{j \in [M] }  \mathcal{H}(
\mathcal{A}_{\mathbf{D}}(D_{val})| 
\mathbf{c}_{\pi_1} = x_{\pi_1}^*, ..., \mathbf{c}_{\pi_{T}} = x_{\pi_{T}}^*,\mathbf{c}_{i} = x_{i, j})$ 
    % 
    % \FORALL{$(\mathbf{x}_j, y_j) \in D_{val}$}
    %     \STATE $entropy = entropy + \mathbb{E}[I(\mathbf{x}_i, \mathbf{x}_j, \mathcal{W_{\pi}})] / |D_{val}|$
    % \ENDFOR
    \IF{$entropy < min\_entropy$}
        \STATE $\pi_{T+1} \gets i$, $min\_entropy \gets entropy$
    \ENDIF
    \ENDFOR
    \STATE $\mathbf{x}_{\pi_{T+1}}^* \gets$ obtain the ground truth of $\mathcal{C}_{\pi_{T+1}}$ by human

\ENDFOR
\RETURN Any world $D \in \mathcal{I}_{\mathcal{D}_{\pi}}$ 

\end{algorithmic}
\end{algorithm}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/\figfmt/alg-info-gain-s}
    % \vspace{-1.5em}
    \caption{CPClean via sequential info. maximization.}
    \label{fig:seq-info-max}
\end{figure}


\vspace{0.5em}
\noindent
{\bf CPClean.} The pseudocode for \at{CPClean} is shown in Algorithm \ref{alg:ccclean}. The algorithm starts with an empty cleaning strategy (line 1). In each iteration, given the current cleaning strategy $\pi_1, ..., \pi_{T}$, we compute the expected value of entropy conditioned on cleaning one extra training example (lines 6-7). We select the next example to clean $\pi_{T+1}$ that minimizes the entropy (lines 8-9). We then ask a human to clean the selected example (line 10). The greedy algorithm terminates when all validation examples become CP'ed (line 3). Finally, we return any world $D$ among all possible partially cleaned worlds $\mathcal{I}_{\mathcal{D}_{\pi}}$ (line 12). Since all the validation examples are CP'ed with $\mathcal{I}_{\mathcal{D}_{\pi}}$, classifier trained on any world in $\mathcal{I}_{\mathcal{D}_{\pi}}$, including the unknown ground truth world $D^*$, has the same validation accuracy. Therefore, $\mathcal{A}_{D}$ has the same validation accuracy as $\mathcal{A}_{D^*}$.

%Given a space , a training set and a validation set, our algorithm in Algorithm \ref{alg:ccclean} starts from an empty ${\pi}$ (Line 1).



\begin{example}  Figure~\ref{fig:seq-info-max} shows an example of how \at{CPClean} selects the next data example to clean in each iteration via sequential information maximization. Assume there are two dirty examples, $\mathcal{C}_1$ and $\mathcal{C}_2$, in the training set and each example has two candidate repairs. Therefore, there are four possible clean versions after cleaning the next data point, based on which data point is selected to be cleaned and which candidate repair is the ground truth. For example, the first table at step 1 shows the clean version after cleaning $
\mathcal{C}_1$ if $x_{1, 1}$ is the ground truth. Assume that we have two validation examples. We run the counting query (Q2) on each possible version w.r.t. each validation example as shown in step 2. Then we can compute the entropy of predictions on validation examples as shown in step 3 and 4. The results show that if $\mathcal{C}_1$ is selected to be cleaned, the entropy may become $0$ or $0.17$ depending on which candidate repair is the ground truth. We assume that each of the two candidate repairs has 50\% chance to be the ground truth. Therefore, the expected entropy after cleaning $\mathcal{C}_1$ is $(0 + 0.17) /2 = 0.09$ (step 5). Similarly, we compute the expected entropy after cleaning $\mathcal{C}_2$ as $0.17$. Since $\mathcal{C}_1$ has a lower expected entropy, we select $\mathcal{C}_1$ to clean. 

%.  We run the counting query (Q2) w.r.t each world and each validation example as shown in step 2. Then we compute the entropy of predictions on the validation examples for each possible world as shown in step 4 and step 5. 

% We first compute the expected entropy for $\mathbf{x_1}$: There are two possible space after cleaning $\mathbf{x_1}$ based on which candidate repair is assumed to be the ground truth. We run our counting query on the two possible space and compute the entropy over all validation examples. The results are 0 and 0.28 respectively. Therefore, the expected entropy after cleaning $\mathbf{x_1}$ example is $(0 + 0.28)/2 = 0.14$. Similarly, we compute the expected entropy of $\mathbf{x}_2$ as $0.28$. Since $\mathbf{x}_1$ has a smaller expected entropy, we select $\mathbf{x}_1$ as the example to clean. 
%By running counting query on the current space and using Equation \ref{Eq:entropy}, we compute the entropy before cleaning $\mathbf{x_1}$ as 0.5. Hence,the expected information gain of $\mathbf{x}_1$ w.r.t the first validation example is $0.5-0.31 = 0.19$.
% Similarly, we compute the information gain of $\mathbf{x}_1$ w.r.t the second validation example as $0.29$. Therefore, the average expected entropy of $\mathbf{x}_1$ is $(0.29 + 0.31)/2 = 0.3$.

\end{example}


%\vspace{-0.5em}
\noindent
{\bf Complexity of CPClean.} In each iteration of Algorithm~\ref{alg:ccclean}, we need to (1) automatically select a tuple; and (2) ask human to clean the selected tuple. To select a tuple, we need to first check  whether $|D_{val}|$ are all CP'ed (line 3), which invokes the $Q1$ query $O(|D_{val}|)$ times. If not all $D_{val}$ are CP'ed, we need to compute expected value of entropy $O(N)$ times (line 6). Computing the expected value of entropy (line 7) needs to invoke the $Q2$ query $O(M|D_{val}|)$ times. Therefore, when the downstream ML model is KNN, using our SS algorithm for $Q1$ and $Q2$, the complexity for selecting a tuple at each iteration is $O(N^2M^2|D_{val}| \times(\log (MN) + K\log N))$. The quadratic complexity in tuple selection is acceptable in practice, since  human involvement is generally considered to be the most time consuming part in practical data cleaning~\cite{DBLP:books/acm/IlyasC19}.

\vspace{0.5em}
\noindent
{\bf Theoretical Guarantee.} The theoretical analysis of this algorithm, while resembling that of~\cite{Chen2015SequentialIM}, is non-trivial. We provide the main \update{theoretical analysis} here and leave the proof to the appendix.

%Assuming all priors we assumed is correct, we then observe the following theoretical guarantee.
\begin{corollary}\label{Corollary: theoretical guarantee of cleaning}
Let the optimal cleaning policy that minimizes the cleaning effort while consistently classifying the test examples be denoted by $D_{\text{Opt}}\subseteq D_{train}$ with limited cardinality $t$,
such that 
% $$D_{\text{Opt}} =  \argmax_{D_{\pi} \subseteq \mathcal{D}_{train}, |D_{\pi}|\leq T}  I(\mathcal{A}_{\mathbf{D}}(D_{val});
% \mathbf{c}_{\pi_1}, ...,
% \mathbf{c}_{\pi_t})$$ where $t\leq T$.
$$D_{\text{Opt}} =  \argmax_{D_{\pi} \subseteq \mathcal{D}_{train}, \ |D_{\pi}|\leq t}  I(\mathcal{A}_{\mathbf{D}}(D_{val});
D_{\pi}).$$ 
The sequential information maximization strategy %studied for data cleaning
%, similarly as in different settings in~\cite{Chen2015SequentialIM}, 
follows a near optimal strategy where the information gathering satisfies
\begin{equation*}
\begin{split}
I(\mathcal{A}_{\mathbf{D}}(D_{val});
\mathbf{c}_{\pi_1}, ...,
\mathbf{c}_{\pi_T})
 \geq I(\mathcal{A}_{\mathbf{D}}(D_{val});
D_{\text{Opt}})(1-\exp{(-{T}/{\theta t'})})
\end{split}
\end{equation*}
where 
% $\theta=\big(\max_{v\in D_{\text{train}}}I(\mathcal{A}_{\mathbf{D}}(D_{val}); v)\big)^{-1}$ and $t'=t\min\{\log |\mathcal{Y}|, \log m \}$.
\begin{align*}
 &\theta=\left(\max_{v\in \mathcal{D}_{\text{train}}}I(\mathcal{A}_{\mathbf{D}}(D_{val}); v)\right)^{-1}
\\
t'=t\min\vspace{-1em}\{&\log |\mathcal{Y}|, \log M \}, \ \ \mathcal{Y}:\text{label space}, \ M: |\mathcal{C}_i|. 
\end{align*}
\end{corollary}
The above result, similarly as in~\cite{Chen2015SequentialIM}, suggests that data cleaning is guaranteed to achieve near-optimal information gathering up to a logarithmic factor $\min(\log |\mathcal{Y}|, \log M)$ when leveraging the sequential information strategy.


\iffalse


%The naive automatic solution is to train $|\mathcal{W}|$ models and select one that has the maximum validation accuracy on $D_{val}$. This is obviously an infeasible solution due to the huge space of $\mathcal{W}$ --- for example, a dataset that has 200 missing values, where each missing value has 5 candidate repairs, would generate $5^{200}$ possible worlds.  

Training all $|\mathcal{W}|$ possible models and selecting one with the maximum validation accuracy is obviously infeasible --- for example, a dataset that has 200 missing values, where each missing value has 5 candidate repairs, would generate $5^{200}$ possible worlds.  
%%
Therefore, current automatic solutions either directly choose a world in $\mathcal{W}$ heuristically without using validation set (e.g., using mean or median for missing value imputation), or use the validation set to select a best world from a significantly reduced subset of worlds in $\mathcal{W}$, which likely does not contain $\mathbf{w}_g$ any more (e.g., BoostClean~\cite{krishnan2017boostclean} limits $\mathcal{W}$ by considering only those worlds where all errors are cleaned the same way). The apparent drawback of automatic cleaning solutions is the lack of any guarantee on the returned model. 
%%%%
On the other hand, the naive human-involved solution would ask a human oracle to manually clean all dirty tuples to recover $\mathbf{w}_g$ directly, which is also expensive considering the high cost of human cleaners. 

Given the drawback of current cleaning solutions, we therefore consider the following question: \textit{can we avoid the manual cleaning of all examples to reach a world that is guaranteed to be as good as the ground-truth world in terms of the generalization error of the derived models?} Our consistent classification framework provides a positive answer. To see this, consider the ideal scenario where all examples in $D_{val}$ are CC'ed, which means that all worlds in $\mathcal{W}$, including $\mathbf{w}_g$, have the same predictions for all examples in $D_{val}$. In this case, no manual cleaning is necessary at all as randomly picking a world in $\mathcal{W}$ is as good as $\mathbf{w}_g$. But what if the examples in $D_{val}$ are not all CC'ed? In this scenario, we can manually clean some examples. As more examples are cleaned, the space will become smaller and the non-CC'ed examples can become CC'ed. In the extreme case, if we clean all the examples, the space will only consist of one world $\mathbf{w}_g$ and all examples in $D_{val}$ will trivially become all CC'ed. Note that $\mathbf{w}_g$ is always contained in the space when we clean examples. Therefore, once all examples are CC'ed, randomly picking a world from the space is still as good as $\mathbf{w}_g$. Naturally, the follow-up question we need to consider is: \textit{how can we minimize the number of manually cleaned examples so that all examples in $D_{val}$ are CC'ed?} Formally, this question can be written as an optimization problem named {\em CC-optimization} problem, which is described as follows:

\begin{align}
\hspace{-1cm} \text{(CC-optimization)} \qquad{} \min &~~ |D_{\pi}| \label{eqn:optimization_problem} \\  
\mbox{s.t.} ~~ &  Q1(\mathbf{x}, \mathcal{W}_{\pi}, \mathcal{A}) = true, \ \forall \mathbf{x}\in D_{\text{val}} \label{eqn:optimization_problem_condition}\\
& D_{\pi} \subseteq D_{train}
\end{align}

where $D_{\pi}$ is the set of the examples that we would like to clean and $\mathcal{W}_{\pi}$ is the resulting space after we clean examples in $D_{\pi}$.

\begin{theorem}
The CC-optimization problem is NP-hard.
\end{theorem}

\xc{Merve: Can you provide a quick proof of this in the appendix?}


%, i.e., the maximum accuracy on a unseen test set $D_{test}$. Following standard practice in ML, we use a separate labeled validation set $D_{val}$ to estimate the performance of a model on $D_{test}$. 


%As an application, in this section, we propose a novel ``DC for ML'' framework built on top of the two CC primitive queries.

%discuss in more detail on addressing the two problems in ``DC for ML,'' i.e., decision and optimization, using consistent classification. 
%As we have mentioned before, our ``DC for ML'' framework is built on top of solutions to the three fundamental CC queries.
%Given that exact solutions to the three CC queries are inefficient in general, we further introduce sampling-based, approximate approaches. 


%\subsection{Revisiting the Workflow}


% %We have presented our overall ``DC for ML'' workflow in Figure~\ref{fig:cc-workflow}. 
% We set aside a small validation set $D_{\text{val}}$ that is assumed clean. We use $D_{\text{val}}$ to estimate the expected impact of cleaning on ML for a given $D$ and ${\cal A}$.
% %which provides vital signals to the decision problem.
% Only if the observed impact over $D_{\text{val}}$ is significant enough should we proceed with further cleaning efforts.
% %the optimization problem.

% %\vspace{-0.5em}
% \subsection{Assessing the Impact of Data Cleaning} 
% As discussed, cleaning may not necessarily improve ML model performance. Let $\Delta(\textbf{x},y)$ be the expected \emph{change of accuracy} after cleaning for an example $(\textbf{x},y) \in D_{\text{val}}$. We first check whether each example in the validation set can be CC'ed using Q1:
% \begin{itemize}
%     \item If an example can be CC'ed, then $\Delta(\textbf{x},y) = 0$.
%     \item If an example cannot be CC'ed,  we run Q2 to obtain the number of worlds where we end up with the correct prediction, i.e., the label $y$ in $D_{\text{val}}$, and we have 
% $$\Delta(\textbf{x},y) = \frac{\text{Q2}(\mathbf{x}, y, \mathcal{W}, {\cal A})}{|\mathcal{W}|} - \mathbb{I}(h(\textbf{x}) = y),$$ 
% where $\mathbb{I}$ is the identity function that returns 1 if the prediction by $h$ (i.e., the classifier trained on top of the original, uncleaned $D$) is correct and 0 otherwise.
% \end{itemize}
% We assume that %the worlds are assigned to a uniform prior model, that is, 
% every possible world in $\mathcal{W}$ is equally likely to be the ground truth (produced by some cleaning strategy).
% We further assume that the unseen test set is drawn from the same distribution that generates $D_{\text{val}}$. 

% %\mg{I thought the input set to the algorithm will be the inconsistently classified features in $D_{val}$ anyway?}

% %{\color{purple} We assume that the worlds are assigned to a uniform prior model, that is, every possible world in $\mathcal{W}$ is equally likely the {\it true} cleaning strategy.}
% Let $\Delta_i$ be the expected change of accuracy for the $i^{\text{th}}$ example in $D_{\text{val}}$ after cleaning, where the expectation is taken over all possible worlds.
% Since the data examples from $D_{\text{val}}$ are i.i.d., the $\Delta_i$'s are also i.i.d. random variables.\footnote{$\Delta_i$ should be viewed as a random variable since $D_{\text{val}}$ is a random sample drawn from the underlying data distribution.}
% %In more detail, the $\Delta_i$'s remain independent but do not conform to the same distribution --- one can conclude this by observing that the expected accuracy of different examples in $D_{\text{val}}$ can be different.
% As a result, we can bound the gap between the accuracy change observed on $D_{\text{val}}$ and the true accuracy change using Hoeffding's inequality (ref. Lemma 4.5 of~\cite{UMLbook}):
% \begin{lemma}[Hoeffding's Inequality]
% Let $\theta_1$, ..., $\theta_m$ be a sequence of i.i.d. random variables and assume that for all $i$, $\E[\theta_i]=\mu$ and $\Pr[a\leq\theta_i\leq b]=1$. Then, for any $\epsilon >0$,
% $$\Pr[|\frac{1}{m}\sum\nolimits_{i=1}^m\theta_i - \mu|>\epsilon]\leq 2\exp{\Big(-\frac{2m\epsilon^2}{(b-a)^2}\Big)}.$$
% \end{lemma}
% Specifically, let $|D_{\text{val}}|=m$ and let $\bar{\Delta}$ be the empirical mean of $\Delta_1$, ..., $\Delta_m$, i.e., $\bar{\Delta}=\frac{1}{m}\sum_{j=1}^m\Delta_j$. Clearly $-1\leq\Delta_j\leq 1$ for $1\leq j\leq m$. By Hoeffding's inequality, it follows that
% \begin{proposition}\label{proposition:accuracy-change}
% Define $\mu=\E[\bar{\Delta}]=\E[\Delta_j]$. We have
% $$\Pr[|\bar{\Delta} - \mu|>\epsilon]\leq 2\exp{\Big(-m\epsilon^2 / 2\Big)}.$$
% \end{proposition}
% %\mg{Maybe we shall change the theorem to the proposition? Let me know if you think it makes sense then I can edit here.}
% Note that $\mu$ is the true accuracy change (i.e., change over the generalization error) between an ``average'' classifier trained on top of a possible world from $\mathcal{W}$ and the classifier trained over the original noisy $D$.
% Proposition~\ref{proposition:accuracy-change} states that the accuracy change observed over $D_{\text{val}}$ can be close to the true accuracy change $\mu$, with high probability, if $D_{\text{val}}$ is sufficiently large.
% More specifically, with probability at least $1-\delta$ where $\delta \in (0, 1)$, we can guarantee that $|\bar{\Delta}-\mu|\leq\epsilon$ if the size of the validation set satisfies
% $$|D_{\text{val}}|=m\geq (2/\epsilon^2)\ln(2/\delta).$$
% For example, if we set $\epsilon=0.1$ and $\delta=0.1$, then $|D_{\text{val}}|\geq 600$.
 
%\ww{Give an explicit expression of $\Delta_i$. I don't quite understand the ``expected change'' here. Why do we need the subscript $i$ here? Do you mean that we may have multiple sampled $D_{val}$ with the same size and try to estimate the expected accuracy change for each record in $D_{val}$?}

%\begin{theorem}
%Let $\overline{\Delta}$ and $s$ be the sample mean and standard deviation of $\Delta_i$ for all $|D_{\text{val}}|$ examples. Then the expected impact of cleaning $D$ on the ML algorithm ${\cal A}$ is $[\overline{\Delta} - s, \overline{\Delta} + s]$ with XXX confidence. 
%\end{theorem}

%\textcolor{red}{Xu: Wentao, can you fill in the above theorem, basically it's estimating population mean from sample mean}

%If every example can be CC'ed, then cleaning surely has no impact 


%\vspace{-0.5em}


%If users are satisfied with the information regarding expected impact of cleaning provided by the estimators employed in addressing the decision problem, then we proceed to 


%The core question thus becomes \textit{``can we avoid the manual cleaning of all examples to reach a world that is as good as''} ${\mathbb{w}_g}$? 

%We propose a new approach to minimize the 



%The optimization problem tries to select the minimum amount of examples in the training set $D$ that need to be cleaned so that all examples in $D_{\text{val}}$ can become CC'ed.

%using the cleaning query (Q3). %for each example in the validation set. 


\subsection{The CCClean Algorithm} 
\label{sec:seq-info-max}


%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
%merves part
%{\color{purple}
%\subsubsection{Sequential Information Maximization}

Given the hardness of the CC-optimization problem, we propose an intuitive and efficient greedy algorithm called \at{CCClean} that follows a sequential cleaning strategy: we start with an empty $D_{\pi}$ and then at each iteration, we select one example that is most valuable in terms of making all examples CC'ed to clean. We repeat this process until all the examples in $D_{val}$ become CC'ed. The question is: \textit{how to measure the benefit of cleaning an example in terms of making $(\mathbf{x}, y)$ CC'ed?}

% Formally, let $\pi^{[k]}$ denote the policy at $k$-th iteration. We have $\pi^{[0]}=\emptyset$. For $k= 1, 2, \dots, l$, we can update the policy by

Let us consider one validation example $(\mathbf{x}, y)$ for now. We first introduce the {\em entropy} of predictions of $(\mathbf{x}, y)$ w.r.t the current space $\mathcal{W}$, which is defined as follows.

\begin{definition}[Entropy]
Given an example $(\mathbf{x}, y) \in D_{val}$ and a space $\mathcal{W}$, the entropy of predictions of $(\mathbf{x}, y)$ w.r.t the space $\mathcal{W}$ can be computed as:
\begin{align}\label{Eq:entropy}
    E(\mathbf{x}, \mathcal{W}) = \sum_{c \in {\cal Y}} -p_c \log_2{p_c}
\end{align}{}

where $p_c$ is the probability of class $c$ over all predictions of $(\mathbf{x}, y)$ w.r.t to $\mathcal{W}$ and can be computed using our counting query as :
$$p_c = -\frac{|\text{Q2}(\mathbf{x}, c, \mathcal{W}, {\cal A})|}{|\mathcal{W}|}$$
% $$E(\mathbf{x}, \mathcal{W}) = \sum_{c \in {\cal Y}} -\frac{|\text{Q2}(\mathbf{x}, c, \mathcal{W}, {\cal A})|}{|\mathcal{W}|} Pr(\frac{|\text{Q2}(\mathbf{x}, c, \mathcal{W}, {\cal A})|}{|\mathcal{W}|})$$
\end{definition}
The entropy is an non-negative value that measures the uncertainty of the predictions of $(\mathbf{x}, y)$. 
The more uncertain the predictions of $(\mathbf{x}, y)$ are, the higher the entropy is. The entropy $E(\mathbf{x}, \mathcal{W}) = 0$ if and only if $(\mathbf{x}, y)$ is CC'ed. Therefore, we can replace the condition in Equation \ref{eqn:optimization_problem_condition} by Equation  \ref{eqn:optimization_problem_condition2} and our goal of making $(\mathbf{x}, y)$ CC'ed as early as possible is equivalent to reducing  $E(x, \mathcal{W_{\pi}})$ to zero as soon as possible.
\begin{align}\label{eqn:optimization_problem_condition2}
    \mbox{s.t.} ~~ & E(\mathbf{x}, \mathcal{W_{\pi}}) = 0, \forall \mathbf{x}\in D_{\text{val}}
\end{align}

Hence, we can measure the benefit of cleaning an example by the reduction in entropy before and after cleaning it. In the nomenclature of information theory, the reduction in entropy is equivalent to the information gain, which is defined as:

\begin{definition}[Information Gain]
Given an example $(\mathbf{x}, y) \in D_{val}$, an example $(\mathbf{x_i}, y_i) \in D_{train} \backslash D_{\pi}$, and a space $\mathcal{W_{\pi}}$, the information gain of $(\mathbf{x_i}, y_i)$ can be computed as:
\begin{equation}\label{Eq:information_gain}
 I(\mathbf{x}_i, \mathbf{x}, \mathcal{W_{\pi}}) = E(\mathbf{x}, \mathcal{W_{\pi}}) - E(\mathbf{x}, \mathcal{W}_{{\pi \cup \{(\mathbf{x}_i^*, y_i)\}}}) 
\end{equation}

where $\mathcal{W}_{{\pi \cup \{(\mathbf{x}_i^*, y_i)\}}})$ denotes the space after cleaning $(\mathbf{x}_i, y_i)$.

\end{definition}

However, since the ground truth of an example is unknown before it is cleaned, the space after cleaning $\mathbf{x}_i$ (i.e. $\mathcal{W}_{\pi \cup (\textbf{x}_{i}^*, y_{i})}$) is also unknown.  To solve this problem, we assume that each candidate repair has an equal probability to be the ground truth. That is,

$$\mathbb{P}(\mathbf{x}^*_{i}=\mathbf{x}_{ik}) = \frac{1}{|\mathcal{C}_i|}$$

With this assumption, we can compute the expected value of the entropy as:

\begin{align}\label{Eq:expected_entropy}
\mathbb{E}[E(\mathbf{x}, \mathcal{W}_{\pi\cup (\textbf{x}_{i}^*, y_{i}))]} = \frac{1}{|\mathcal{C}_i|} \sum\limits_{j=1}^{|\mathcal{C}_i|}E(\mathbf{x}, \mathcal{W}_{\pi \cup (\textbf{x}_{ij}, y_{i})})
\end{align}
where $\mathcal{W}_{\pi \cup (\textbf{x}_{ij}, y_{i})}$  denote the space after cleaning $\mathbf{x}_i$ supposing that $\mathbf{x}_i^* = \mathbf{x}_{ij}$. 

In other words, we compute the entropy of predictions of $(\mathbf{x}, y)$ w.r.t each possible space after cleaning $(\mathbf{x}_i, y_i)$ and use the average value as the expected value of the entropy.

% the expected entropy of $(\mathbf{x}, y)$ after cleaning $(\mathbf{x}_i, y_i) $is the average entropy w.r.t all possible space after cleaning 

 We can further compute the expected value of information gain from Equation \ref{Eq:information_gain}. Since $E(\mathbf{x}, \mathcal{W}_{\pi})$ is constant, we have: 

\begin{align}\label{expected_info_gain}
    \mathbb{E}[I(\mathbf{x}_i, \mathbf{x}, \mathcal{W_{\pi}})] = E(\mathbf{x}, \mathcal{W_{\pi}}) - \frac{1}{|\mathcal{C}_i|} \sum\limits_{j=1}^{|\mathcal{C}_i|}E(\mathbf{x}, \mathcal{W}_{\pi \cup (\textbf{x}_{ij}, y_{i})})
\end{align}

Note that the expected information gain does not need  the ground truth. Therefore, we can compute it for each example without cleaning the example and we then select the example with highest expected information gain to clean. For a validation set that has more than one example, we compute the expected information gain with respect to each example in the validation set. We then select the example that has the highest average expected information gain over all validation examples to clean.

We summarize our greedy algorithm in Algorithm \ref{alg:ccclean}. Given a space, a training set and a validation set, we start from an empty $D_{\pi}$ (Line 1). At each iteration, we compute the average expected information gain for each training example w.r.t all validation examples (Line 4-7). We then select the example that has the highest average expected information gain to clean (Line 8). The greedy algorithm terminates when all validation examples become CC'ed (Line 4). Finally, we return  a world $\mathbf{w}_s$ randomly sampled from the resulting consistent space.


\begin{algorithm}
\caption{Algorithm \at{CCClean}.} \label{alg:ccclean}
\begin{algorithmic}[1]
\REQUIRE {The space $\mathcal{W}$, $D_{train}$, and $D_{val}$}
\ENSURE {A world $\mathbf{w}_s$ in 
$\mathcal{W}$}
\STATE $D_{\pi} \gets \emptyset$
\WHILE{\NOT $D_{val}$ all CC'ed}
    \STATE $max\_gain \gets -\infty$
    \FORALL{$(\mathbf{x}_i, y_i) \in D_{train} \backslash D_{\pi}$}
    \STATE $gain = 0$
    \FORALL{$(\mathbf{x}_j, y_j) \in D_{val}$}
        \STATE $gain = gain + \mathbb{E}[I(\mathbf{x}_i, \mathbf{x}_j, \mathcal{W_{\pi}})] / |D_{val}|$
    \ENDFOR
    \IF{$gain > max\_gain$}
        \STATE $(\mathbf{x}_s, \mathbf{y}_s) \gets (\mathbf{x}_i, y_i)$, $max\_gain \gets gain$
    \ENDIF
    \ENDFOR
    \STATE $\mathbf{x}_s^* \gets$ ask human to clean $\mathbf{x}_s$
    \STATE $D_{\pi} \gets D_{\pi} \cup \{(\mathbf{x}_s^*, y_s)\}$
\ENDWHILE
\STATE Random sample a world $\mathbf{w}_s$ from $\mathcal{W}_{\pi}$

\end{algorithmic}
\end{algorithm}

\begin{example} (\textcolor{red}{Need to update the figure}) We show how \at{CCClean} works using examples in Figure~\ref{fig:seq-info-max}. 
Assume there are two dirty examples $\mathbf{x}_1$, $\mathbf{x}_2$ in the training set and each example has two candidate repairs. We first compute the expected information gain for $\mathbf{x_1}$ w.r.t to the first validation example: There are two possible space after cleaning $\mathbf{x_1}$ based on which candidate repair is assumed to be the ground truth. We run our counting query on the two possible space and compute the entropy  using Equation \ref{Eq:entropy}. The results are 0.28 and 0.34 respectively. Therefore, the expected entropy after cleaning $\mathbf{x_1}$ is $(0.28 + 0.34)/2 = 0.31$. By running counting query on the current space and using Equation \ref{Eq:entropy}, we compute the entropy before cleaning $\mathbf{x_1}$ as 0.5. Hence,
the expected information gain of $\mathbf{x}_1$ w.r.t the first validation example is $0.5-0.31 = 0.19$. Similarly, we compute the information gain of $\mathbf{x}_1$ w.r.t the second validation example as $0.17$. Therefore, the average expected information gain of $\mathbf{x}_1$ is $(0.17 + 0.19)/2 = 0.18$. Similarly, we compute the average expected information gain of $\mathbf{x}_2$ as $0.1$. Since $\mathbf{x}_1$ has a higher information gain, we select $\mathbf{x}_1$ as the example to clean.
\end{example}



%In practical data cleaning~\cite{DBLP:books/acm/IlyasC19}, human involvement is generally considered to be the most time consuming part. Therefore, we 

\stitle{Complexity of CCClean.} In each iteration of Algorithm~\ref{alg:ccclean}, we need to (1) automatically select a tuple; and (2) ask human to clean the selected tuple. To select a tuple, we need to first check  whether $|D_{val}|$ are all CC'ed (Line 2), which invokes the checking query $O(|D_{val}|)$ times. If not all $D_{val}$ are CC'ed, we need to compute the expected information gain $O(n|D_{val}|)$ times (Line 4-6). According to Equation \ref{expected_info_gain}, computing the expected information gain (Line 7) needs the entropy computation $m+1$ times, which invokes the counting query $O(m)$ times. Therefore, the complexity for selecting a tuple at each iteration is $O(nm|D_{val}| + n^2m^2|D_{val}| \times(\log m+\log n + nK))$ when the downstream ML model is KNN. The quadratic complexity in tuple selection is acceptable in practice, since  human involvement is generally considered to be the most time consuming part in practical data cleaning~\cite{DBLP:books/acm/IlyasC19}.

%% Therefore, in each iteration, we need $O(nmD_{val} + n^2m^2|D_{val}| \times(\log m+\log n + nK))$

% \begin{itemize}
%     \item At each iteration, to check whether $|D_{val}|$ are all CC'ed (Line 2), we need to invoke the checking query $O(|D_{val}|)$ times. 
%     \item At each iteration, we need to compute the expected information gain $O(n|D_{val}|)$ times (Line 4-6). According to Equation \ref{expected_info_gain}, computing the expected information gain (Line 7) needs to compute $m+1$ entropies, which needs to invoke the counting query $O(m)$ times. Therefore, at each iteration, we need to invoke the counting query $O(nm|D_{val}|)$ times.
%     \item There are at most $n$ iterations, since all the examples will be cleaned after $n$ iterations and $D_{val}$ will then become trivially all CC'ed.
% \end{itemize}

% Hence, the algorithm \ref{alg:ccclean} needs to invoke the checking query $O(nD_{val})$ times and counting query $O(n^2m|D_{val}|)$ times. The time complexity is $O(n^2mD_{val} + n^3m^2|D_{val}| \times(\log m+\log n + nK))$.

% The algorithm is dominated by computing the expected information gain (Line 7). 


% \begin{align}\label{expected_info_gain}
%     \mathbb{E}[I(\mathbf{x}_i, D_{val}, \mathcal{W_{\pi}})] = \frac{1}{|D_{val}|}\sum\limits _{\mathbf{x}_j \in D_{val}}\mathbb{E}[I(\mathbf{x}_i, \mathbf{x}_j, \mathcal{W_{\pi}})]
% \end{align}


% We then select the example that has the largest average information gain over all validation examples. That is,
% \begin{align}\label{Eq:selective_sampling_expected_all}
%     (\textbf{x}_{k}, y_{k}) =& \argmax_{(\textbf{x}_{i}, y_{i})\in D_{\text{train}} \backslash D_{\pi}} \frac{1}{|D_{val}|}\sum\limits_{\mathbf{x}_j \in D_{val}} \mathbb{E}[I(\mathbf{x}_i, \mathbf{x}_j, \mathcal{W}_{\pi})]
% \end{align}




% replace the entropy in Equation \ref{Eq:information_gain} with its expected value in \ref{Eq:expected_entropy}. Since $E(\mathbf{x}, \mathcal{W}_{\pi})$ is constant, the result is the expected information gain of $(\mathbf{x_i}, y_i)$. Then at each iteration, we select the example $(\textbf{x}_{k}, y_{k})$ that has the largest expected information gain to clean. That is,
% \begin{align}\label{Eq:selective_sampling_expected}
%     (\textbf{x}_{k}, y_{k}) =& \argmax_{(\textbf{x}_{i}, y_{i})\in D_{\text{train}} \backslash D_{\pi}} \mathbb{E}[I(\mathbf{x}_i, \mathbf{x}, \mathcal{W}_{\pi})]
% \end{align}

% Then at each iteration, we would like to select the example $(\textbf{x}_{k}, y_{k})$ with the largest information gain to clean. That is,

% \begin{equation}\label{Eq:selective_sampling}
%     (\textbf{x}_{k}, y_{k})= \argmax_{(\textbf{x}_{i}, y_{i})\in D_{\text{train}} \backslash D_{\pi}} I(\textbf{x}_{i}, \mathbf{x}, \mathcal{W}_{\pi})
% \end{equation}





% \begin{equation}\label{Eq:update_rule}
% \begin{split}
%      \pi^{[k+1]} \leftarrow \pi^{[k]} \cup \{(\textbf{x}^*_k, y_k)\}
% \end{split}
% \end{equation}

% Therefore, we would like to select an example in $D_{train}$ to clean such that the reduction of the entropy is maximized. 

% If , then $E(\mathbf{x}, \mathcal{W}) = 0$. We would like to find a minimal cleaning policy $\pi$ such that the entropy becomes zero after cleaning the data.

% 
% reduce the entropy to zero with minimal number of cleaning examples.


% to prioritize human cleaning efforts so that all examples in $D_{val}$ can become  CC'ed as early as possible. 


% \begin{algorithm}
% \caption{Algorithm \at{CCClean}.} \label{alg:}
% \begin{algorithmic}[1]
% \REQUIRE {The space $\mathcal{W}$, $D_{train}$, and $D_{val}$}
% \ENSURE {A world $\mathbf{w}_s$ in $\mathcal{W}$}
% \FORALL{$(x_i, y_i) \in D_{train}$}
%     \FORALL{$(x, y) \in D_{val}$}
%         \STATE
%     \ENDFOR
% \ENDFOR
% \STATE 
% \end{algorithmic}
% \end{algorithm}


% where,
% \begin{equation}\label{Eq:selective_sampling}
%     (\textbf{x}_{k}, y_{k})= \argmax_{(\textbf{x}_{i}, y_{i})\in D_{\text{train}} \backslash D_{\pi}^{[k]}} Entropy(\mathbf{x}, \mathcal{W}_{\pi^{[k]}}) - Entropy(\mathbf{x}, \mathcal{W}_{\pi^{[k]} \cup (\textbf{x}_{i}^*, y_{i})})
% \end{equation}


% Formally, given a cleaning policy $\pi$ and a selected example $(\mathbf{x}_k, y_k)$, we define the reduction of the entropy after cleaning the example as the information gain by cleaning the example, denoted as $I(\mathbf{x}, \mathcal{W}, k)$.





% let $\pi^{[k]}$ denote the cleaning policy at $k$-th iteration and let $(\mathbf{x}^{[k]}, y^{[k]})$ denote the selected example at $k$-th iteration. The update rule for a policy 

% \begin{equation}\label{Eq: selected example}
%     (\textbf{x}_{k}, y_{k})= \argmax_{(\textbf{x}_{i}, y_{i})\in D_{\text{train}} \backslash D_{\pi}^{[k]}} Entropy(\mathbf{x}, \mathcal{W}_{\pi \}) - Entropy(\mathbf{x}, \mathcal{W}_{\pi})
% \end{equation}


% We keep track of the validation accuracy 

%Also, it is not necessary to make all examples CC'ed  




\subsection{CCClean Guarantees and Optimizations}

In this section, we first provide theoretical analysis regarding the size of the validation set needed. We then show that the number of examples cleaned by CCClean is guaranteed to be within a small constant factor of the optimal solution. 
%Finally, we provide a simple hyperparameter that allows the cleaning process to stop earlier to further reduce the human cleaning efforts. 
%Finally, we provide 

%Despite it being a greedy algorithm, the number of examples cleaned by CClean is within a small constant bound with respect to the optimal so

\subsubsection{The Size of Validation Set}


Let $D^*$ be the unknown ground-truth clean data for $D$, 
and let $h^* = {\cal A}(D^*)$ be the unknown classifier trained on top of $D^*$. 
On the other hand, we are interested in the ``final'' classifier $h^f$ trained on any remaining possible world in ${\cal W}$ when all examples in $D_{\text{val}}$ are CC'ed.
What is the performance gap between $h^*$ and $h^f$?

We study this question by measuring the test accuracy gap (or equivalently, the gap over generalization error) between $h^*$ and $h^f$.
Specifically, let the test accuracy of $h^*$ and $h^f$ be $\theta^*$ and $\theta^f$, respectively.
Notice that the validation accuracy $\theta^f_{\text{val}}$ of $h^f$ and $\theta^*_{\text{val}}$ of $h^*$ is the same, as all examples $D_{\text{val}}$ are CC'ed by $h^f$.
\begin{theorem}\label{theorem:gap-opt-cc-ground-truth}
Given $\epsilon>0$, it follows that
$$\Pr[|\theta^f-\theta^*|>\epsilon]<4\exp{\Big(-m\epsilon^2/2\Big)}.$$
\end{theorem}
As before, given $0<\delta<1$, with probability at least $1-\delta$ we have $|\theta^f-\theta^*|\leq\epsilon$ if provided with a validation set of size
$$|D_{\text{val}}|\geq\frac{2}{\epsilon^2}\ln\frac{4}{\delta}.$$
For example, if we set $\epsilon=\delta=0.1$, then a validation set with 738 examples would be sufficient to guarantee $|\theta^f-\theta^*|\leq 0.1$ with probability at least 0.9.

\xc{Can we have a better estimate here? 0.1 difference seems high.}


\subsubsection{Guarantees on the Cleaning Effort}


We describe an approach for the optimization problem that follows a \emph{sequential information maximization} strategy. 
%Specifically, our approach aims to clean the rows in a dataset $D_{\text{train}}$ such that the ML model is able to consistently classify a test example $\mathbf{x}$ by minimizing the cleaning effort.
%Towards that, 
Our objective is, under constraints, to maximize the \emph{mutual information} between the training data points cleaned by a data cleaning policy $\pi$ denoted by $D_{\pi}$, and the prediction $h_{\mathbf{w}_{\pi}}(\mathbf{x})$ of an unknown validation data point $\mathbf{x}$, where $\mathbf{w}_{\pi}$ is a possible world in $\mathcal{W}_{\pi}$ such that 
\begin{equation}\label{Eq: objective function pure}
    \max_{D_{\pi}\subseteq D_{\text{train}}} {I}(h_{\mathbf{w}_{\pi}}(\textbf{x}); D_{\pi})
\end{equation}
while the size of $D_{\pi}$ not exceeding a cleaning budget $l$. 

Here, we consider a setting where we have direct access to $D_{\text{val}}$, and focus on cleaning the rows of $D_{\text{train}}$ to maximize the empirical average of the \emph{information gain} between the set of cleaned rows $D_{\pi}$ and predictions on $D_{\text{val}}$ using the partially cleaned training data. That is, by denoting 
$$I(h_{\mathbf{w}_{\pi}}({D_{\text{val}}}); D_{\pi})\coloneqq\frac{1}{|D_{\text{val}}|} \sum_{\textbf{x}_{\text{val}}\in D_{\text{val}}}I(h_{\mathbf{w}_{\pi}}(\textbf{x}_{\text{val}}); D_{\pi}),$$ we approximate (\ref{Eq: objective function pure}) as
\begin{equation}\label{Eq: objective function}
    \max_{D_{\pi}\subseteq D_{\text{train}}}I(h_{\mathbf{w}_{\pi}}({D_{\text{val}}}); D_{\pi}) \quad\text{ s.t. }\quad |D_{\pi}|\leq l.
\end{equation}
%such that $|D_{\pi}|\leq l$.

\noindent
\textbf{(Sequential Information Maximization)}
We follow a sequential information maximization strategy, where the training data points that are most informative about $D_{\text{val}}$ are sequentially cleaned. 
%the dirty training instance $\textbf{x}_i \in D_{\text{train}}\backslash D_{\pi}^{[k]}$, which will bring the largest information gain to the objective function in (\ref{Eq: objective function}), is sequentially requested to be cleaned. Upon receiving the cleaned row $\textbf{x}^{[k]}$, $\mathcal{Q}_3$ updates the possible worlds by removing the worlds that has $\textbf{x}^{[k]} \neq \textbf{x}_{\pi}^{[k]}$. 
Formally, we introduce our cleaning methodology as follows.

Let $\tilde{\mathbf{x}}_i$ denote a random variable defined over the clean space of $\mathbf{x}_i$ such that $(\tilde{\mathbf{x}}_i, y_i) \in \mathcal{C}_i$. For $D_{\pi}^{[0]}=\emptyset$, and $k= 1, 2, \dots, l$, update rule for a policy $\pi$ is given by
\begin{equation}\label{Eq: update rule}
\begin{split}
    % D^{[k+1]}_{\pi} \leftarrow \mathcal{Q}_3(D_{\text{val}}, \mathcal{W}^{[k]}_{\pi}|\mathcal{C}^*_{i^*}\leftarrow \mathcal{C}_{i^*}, \mathcal{A})
     D^{[k+1]}_{\pi} \leftarrow D^{[k]}_{\pi} \cup \{(\textbf{x}^*_k, y_k)\}
\end{split}
\end{equation}
where 
\begin{equation}\label{Eq: selective sampling}
    (\textbf{x}_{k}, y_{k})= \argmax_{(\textbf{x}_{i}, y_{i})\in D_{\text{train}} \backslash D_{\pi}^{[k]}} I(h_{\mathbf{w}_{\pi}}(D_{\text{val}}); (\tilde{\mathbf{x}}_i, y_i)|D_{\pi}^{[k]}).
\end{equation}
To simplify our update rule, we note the following expansion
\begin{equation*}
    \begin{split}
        I(h_{\mathbf{w}_{\pi}}(\textbf{x}_{\text{val}}); (\tilde{\mathbf{x}}_i, y_i)|D_{\pi}^{[k]})=&\\
        \mathcal{H}(h_{\mathbf{w}_{\pi}}(\textbf{x}_{\text{val}})|D_{\pi}^{[k]})-\mathcal{H}&(h_{\mathbf{w}_{\pi}}(\textbf{x}_{\text{val}})|D_{\pi}^{[k]}\cup \{(\tilde{\mathbf{x}}_i, y_i)\}).
    \end{split}
\end{equation*}
We further let $$\mathcal{H}(h_{\mathbf{w}_{\pi}}(D_{\text{val}})|D_{\pi})=\frac{1}{|D_{\text{val}}|} \sum_{\textbf{x}_{\text{val}}\in D_{\text{val}}} \mathcal{H}(h_{\mathbf{w}_{\pi}}(\textbf{x}_{\text{val}})|D_{\pi})$$ 
and rewrite (\ref{Eq: selective sampling}) as
\begin{equation}\label{Eq: selective sampling entropy}
\begin{split}
    (\textbf{x}_{i^*}, y_{i^*})= \argmin_{(\textbf{x}_{i}, y_{i})\in D_{\text{train}} \backslash D_{\pi}^{[k]}} \mathcal{H}(h_{\mathbf{w}_{\pi}}(D_{\text{val}})|D_{\pi}^{[k]}\cup \{(\tilde{\mathbf{x}}_i, y_i)\}).
    \end{split}
\end{equation}

% as $$D^{[k+1]}_{\pi} \leftarrow \mathcal{Q}_3(D_{\text{val}}, \mathcal{W}^{[k]}_{\pi}|\textbf{x}_{\text{train}}^{[k]} = \text{clean}(\textbf{x}_{\text{train}}^{[k]}), \mathcal{A})$$
% % \begin{equation}\label{Eq: update rule entropy}
% %     D^{[k+1]}_{\pi} \leftarrow Q3(D_{\text{val}}, \mathcal{W}^{[k]}_{\pi}|\{x^{[k]}=x^{[k]}_c\}, \mathcal{A})
% % \end{equation}
% with $\mathbf{x}_{\text{train}}^{[k]} = \arg\min_{\textbf{x}_{\text{xx}} \in D_{\text{val}}}  \mathcal{H}(D_{\text{val}}|D^{[k]}_{\pi})$.

\noindent
\textbf{(The Cleaning Policy)} 
%We define the entropy of our dirty training set $D_{\text{train}}$ to express the amount of uncertainty of class prediction on a validation set $D_{\text{val}}$. 
Let $h_{\mathbf{w}_{\pi}}({\bf x}_{\text{val}})$ for $\mathbf{w}_{\pi} \in \mathcal{W}_{\pi}$ denote the prediction of a test data point ${\bf x}_{\text{val}} \in D_{\text{val}}$. By definition, we have
\begin{equation*}
\begin{split}
\mathcal{H}(h_{\mathbf{w}_{\pi}}(\textbf{x}_{\text{val}})|D_{\pi}) =&\\ 
-\sum_{c \in \mathcal{Y}} \mathbb{P}(h_{\mathbf{w}_{\pi}}&(\mathbf{x}_{\text{val}})=c|D_{\pi})\log \mathbb{P}(h_{\mathbf{w}_{\pi}}(\mathbf{x}_{\text{val}})=c|D_{\pi})  
\end{split}
\end{equation*}
where
\begin{equation*}
    \begin{split}
        \mathbb{P}(h_{\mathbf{w}_{\pi}}(\mathbf{x}_{\text{val}})=c|D_{\pi})&= \mathbb{E}_{\mathbf{w}_{\pi}}[\mathbbm{1}[h_{\mathbf{w}_{\pi}}(\mathbf{x}_{\text{val}})=c]]\\
        &= \sum_{\mathbf{w}_{\pi}\in \mathcal{W}_{\pi}} \mathbb{P}(\mathbf{w}_{\pi})\mathbbm{1}[h_{\mathbf{w}_{\pi}}(\mathbf{x}_{\text{val}})=c].
    \end{split}
\end{equation*}
We assign a uniform prior to $\mathbf{w}_{\pi}$, i.e., $\mathbb{P}(\mathbf{w}_{\pi})=\frac{1}{|\mathcal{W}_{\pi}|}$. Therefore,

\begin{equation}\label{Equation: exact posterior}
    \begin{split}
        \mathbb{P}(h_{\mathbf{w}_{\pi}}(\mathbf{x}_{\text{val}})=c|D_{\pi})
        = \frac{\#\{\mathbf{w}_{\pi}: h_{\mathbf{w}_{\pi}}(\mathbf{x}_{\text{val}})=c\}}{|\mathcal{W}_{\pi}|}.
    \end{split}
\end{equation}
% If the test data point $\mathbf{x}$ can be consistently classified (i.e. models trained on all possible worlds return the same label) then all partitions of $w_i\in \mathcal{W}$ are empty sets, except for a single one which equals to $\mathcal{W}$. This would lead to the entropy $E(\mathcal{W})$ being equal to zero.
A natural stopping criterion is $l^*=\argmin_{k\in \mathbb{N}^+, k\leq l} k$ such that $Q1(\mathbf{x}, \mathcal{W}_{\pi}^{[k]}, A)=\verb|true|, \ \forall \mathbf{x}\in D_{\text{val}}$.

% This notion gives us the stopping criterion for an iterative cleaning algorithm. This algorithm chooses a data point $(\mathbf{x}_i, y_i) \in D$ to be cleaned by passing it to an oracle that selects one data repair $c$ which in turn transforms the set $\mathcal{C}_i$ into a singleton set $\mathcal{C}_i = \{ (\mathbf{x}_{ic}, y_i) \}$. Then, the algorithm recomputes the entropy and halts if the entropy is zero.
\vspace{0.5em}
\noindent
\textbf{(Guarantees)} We define the optimal cleaning policy that minimizes the cleaning effort while consistently classifying the test examples as follows:
%The performance of a cleaning policy revolves around the success for minimizing the cleaning effort while consistently classifying the test examples. Towards that, we define the optimal policy as follows.
\begin{definition}\label{Definition: optimal policy}
We define the optimal set of size $k$ by $D_{\text{opt}}^{[k]}$ such that $D_{\text{opt}}^{[k]}= \argmax_{D \subseteq D_{\text{train}}} I(h_{\mathbf{w}}; D)$ where $|D|\leq k$.
\end{definition}

\begin{theorem}\label{Theorem: theoretical guarantee of cleaning}
\begin{equation}
\begin{split}
    &{I}(h_{\mathbf{w}_{\pi}}(D_{\text{val}}); D_{\pi}^{[l]})\\
    & \hspace{1em }\geq {I}(h_{\mathbf{w}_{{\text{opt}}}}(D_{\text{val}}); D_{\text{opt}}^{[k]}) \Big(1-\exp{\Big(-\frac{l}{k\gamma \min\{\log|\mathcal{Y}|, \log m\}}\Big)}\Big).
    \end{split}
\end{equation}
where $\gamma=\big(\max_{v\in D_{\text{train}}}I(h_{\mathbf{w}_{\text{opt}, \pi}}(D_{\text{val}});v)\big)^{-1}$.
\end{theorem}




% \noindent
% \textbf{(Approximation of the Conditional Entropy)} The update rule introduced in (\ref{Eq: selective sampling entropy}) comes with its own drawback. The computation of the posterior in (\ref{Equation: exact posterior}) is over all possible worlds, which possess exponential complexity in the size of clean space, i.e., $$|\mathcal{W}_{\pi}|=|\prod\nolimits_{i\in D_{\pi}} \mathcal{C}^*_i\cdot\prod\nolimits_{j\in D_{\text{train}\backslash D_{\pi}}} \mathcal{C}_j|.$$
% Here, we resort to an approximate approach where we compute the entropy over the i.i.d. samples $\mathbf{w}_s \in \mathcal{W}_s$ of $\mathbf{w}_{\pi} \in \mathcal{W}_{\pi}$. We then approximate $\mathbb{P}(h_{\mathbf{w}_{\pi}}(\mathbf{x}_{\text{val}})=c|D_{\pi})$ by $ \mathbb{P}(h_{\mathbf{w}_{s}}(\mathbf{x}_{\text{val}})=c|D_{\pi})$ s.t.
% \begin{equation}\label{Equation: approximate posterior}
%     \begin{split}
%          \mathbb{P}(h_{\mathbf{w}_{s}}(\mathbf{x}_{\text{val}})=c|D_{\pi})= \frac{\#\{\mathbf{w}_{s}: h_{\mathbf{w}_{s}}(\mathbf{x}_{\text{val}})=c\}}{|\mathcal{W}_{s}|}.
%     \end{split}
% \end{equation}



%\mg{I temporarily removed the complexity discussion here, we will discuss it with Bojan about the story.}
% Our aim is to compute the approximate expected entropy after cleaning the data point $\mathbf{x}_i$:
% \begin{equation} \label{eq:approx-after-entropy}
%     \mathbb{E} \left[ E(\mathcal{W}', \mathbf{x}_i) \right] = \frac{1}{|\mathcal{C}_i|} \sum_{(\mathbf{x},y) \in \mathcal{C}_i} E(\mathcal{W}' \ | \ \mathbf{x}_i = \mathbf{x})
% \end{equation}
% Note that this sum has $O(|\mathcal{C}_i|) = O(m)$ elements. Each element of the sum represents the entropy after assigning one specific repair to data point $\mathbf{x}_i$:
% \begin{equation} \label{eq:approx-after-entropy-2}
%     E(\mathcal{W}' \ | \ \mathbf{x}_i = \mathbf{x}_{ic}) = - \sum_{y \in \mathcal{Y}} \mathbb{P}(y \ | \ \mathbf{x}_i = \mathbf{x}_{ic}) \log \mathbb{P}(y \ | \ \mathbf{x}_i = \mathbf{x}_{ic})
% \end{equation}
% This sum has $O(|\mathcal{Y}|) = O(L)$ elements. To compute each conditional probability, use the following ratio:
% \begin{equation*}
%     \mathbb{P}(y \ | \ \mathbf{x}_i = \mathbf{x}_{ic}) = \frac{|\mathcal{W}'_{y \ | \ \mathbf{x}_i = \mathbf{x}_{ic}}|}{|\mathcal{W}'|}
% \end{equation*}
% The quantity in the numerator is the number of possible worlds from our subsample $\mathcal{W}'$ that satisfy both of the following conditions: (1) the algorithm predicts the $y$ for the test data point; \emph{and} (2) the data repair that replaces the data point $\mathbf{x}_i$ is exactly $\mathbf{x}_{ic}$. In other words:
% \begin{equation} \label{eq:w-set-given-x}
%     \mathcal{W'}_{y \ | \ \mathbf{x}_i = \mathbf{x}_{ic}} :=
%         \{ D_i \in \mathcal{W}' : \mathcal{A}(D_i)(\mathbf{x}) = y \ \land \ (\mathbf{x}_{ic}, \cdot) \in D_i \}
% \end{equation}
% This set has $O(|\mathcal{W}'|)$ elements, which equals to the time complexity for computing its size in the most naive approach. We can notice that the sum in Equation~\ref{eq:approx-after-entropy-2} already partitions the set $\mathcal{W}'$ based on the label $y$, so that all set enumerations in Equation~\ref{eq:w-set-given-x} are over mutually distinct subsets. As a result, if we use a vector of size $L$ to do the counting per each possible label, we can compute Equation~\ref{eq:approx-after-entropy-2} in $O(|\mathcal{W}'|)$ time. As a result, to find the next data point to clean as defined in Equation~\ref{eq:min-after-entropy}, we need to compute Equation~\ref{eq:approx-after-entropy} for every training data point. The total time complexity of this operation is $O(n \cdot m \cdot |\mathcal{W}'|)$.

% We are left with the question of the size of the sampled subset. In order to be sure that our partitioning by specific data repairs will yield a positive number of elements in each partition, the size of $\mathcal{W}'$ has to be at least $O(m)$. The constant multiplier needs to be sufficient to ensure an acceptably low error probability.












%  \subsubsection{Early Stopping}
 
%  \textcolor{red}{Peng: I think the early stopping does not fit the story since it has no guarantee and it needs  a ``base" world.} \at{CCClean} can make all examples in $D_{val}$ CC'ed efficiently. However, as we will show in our experiments, when the validation set and the space are very large, some datasets still need to clean over 90\% of the data to make all examples CC'ed, which may exceed the cleaning budget in practice. Therefore, we may need to stop earlier before all examples become CC'ed. We propose an early stopping strategy: we start from a \textit{base world} $\mathbf{w}_b \in \mathcal{W}$ (e.g. the world with mean imputation). At each iteration of \at{CCClean}, after we select and clean an example, we also update $\mathbf{w}_b$ by replacing the corresponding example in $\mathbf{w}_b$ with its ground truth. We keep track of the validation accuracy of $\mathbf{w}_b$ at each iteration. When we determine to stop, we return the $\mathbf{w}_b$ at the iteration with the highest validation accuracy.

\fi

==> [arXiv] Certain Prediction/Intro.tex <==
% !TEX root = CC.tex
%\begin{figure*}
%    \centering
%    \includegraphics[width=0.9\textwidth]{Figures/workflow.png}
%    \vspace{-1em}
%    \caption{DC for ML using CC, given a dirty training set $D$ with its possible world $\mathcal{W}$, an ML algorithm ${\cal A}$, and a validation set $D_{\text{val}}$.}
%    \vspace{-1.5em}
%    \label{fig:cc-workflow}
%\end{figure*}

% \the\columnwidth

%\vspace{-1em}
\section{Introduction}

Building high-quality 
Machine learning (ML) applications 
often hinges on the availability of
high-quality data.
However, due to noisy inputs from manual data curation or inevitable errors from automatic data collection/generation programs, in reality, data is unfortunately seldom clean.
Inconsistency and incompleteness are ubiquitous in real-world datasets, and therefore can have an impact on ML applications trained on top of them.
In this paper, we focus on the question:
\textit{Can we reason about the 
impact of data incompleteness on the 
quality of ML models trained over
it?}

\begin{figure}[t]
\centering
\includegraphics[width=0.6\textwidth]{Figures/\figfmt/sure-answer-2}
% \vspace{-1.5em}
\caption{An illustration of the
relationship between \textit{certain answers}
and \textit{certain predictions}.}
\label{fig:sureanswer}
\end{figure}

Figure~\ref{fig:sureanswer} illustrates 
one dataset with
incomplete information. In this example,
we have the incomplete dataset $D$ with
one missing cell (we will
focus on cases in which there are 
\textit{many} cells with incomplete information) --- the 
age of Kevin is not 
known and therefore is set as \texttt{NULL} (@). 
Given an ML training algorithm $\mathcal{A}$,
we can train an ML model over $D$, $\mathcal{A}_D$, and given a clean test
example $t$, we can get the prediction of 
this ML model $\mathcal{A}_D(t)$. The focus 
of this paper is to understand \textit{how much impact
the incomplete information (@) has
on the prediction $\mathcal{A}_D(t)$}. This 
question is not only of theoretical interest
but can also have interesting practical implications ---
for example, if we know that,
for a large enough number of samples of
$t$, the incomplete information
(@) does not have an impact on $\mathcal{A}_D(t)$
at all, spending the effort of cleaning or acquiring
this specific piece of missing information will
not change the quality of downstream ML models.

%\vspace{0.5em}
%\noindent
%{\bf \textit{The Statistics View:
%Learning Over Incomplete Information.}}
%The statistics community has been focusing on 
%the problem of learning/analytics over
%incomplete data for decades. There are two lines
%of work that are in particular related to our work. Under different assumptions
%on the missing information (e.g., missing
%at random), one can reason about the behavior
%of \textit{some} downstream classifiers
%with respect to the missing values. Such an
%analysis often states results in the 
%asymptotic regime~\cite{XXX, YYY, ZZZ, WWW, FFF}.
%On the other hand, there is a range of 
%work trying to design novel ML models
%and training mechanisms that are \textit{more} 
%robust to the incomplete information.
%One such example is  
%multiple imputation~\cite{XX,XX,XX},
%in which one samples multiple possible
%values of the incomplete information and
%conducts analytics over each possible 
%value and then aggregates.
%
%
%\xc{The transition from previous paragraph to the goal paragraph is not clear. Multiple imputation is not so slow either? Also why the focus on finite data regime?
%Our focus should perhaps be (1) building a theoretical foundation and (2) proposing efficient algorithms for understanding the impact of incomplete data on ML?
%}
%
%\vspace{0.5em}
%\noindent
%{\bf \textit{Our Goal.}}
%In this work, we take a different view
%and focus more on the \textit{algorithmic} perspective of this problem
%(it is \textit{algorithmic} in the sense that one can apply our algorithm to
%make, e.g., some
%version of the multiple imputation algorithm much faster): We are interested
%in the finite data regime, in which we are
%given an incomplete dataset with
%finite number of samples. Our goal is to
%reason how \textit{robust}/\textit{resilient} 
%a given ML training algorithm is to 
%the data incompleteness \textit{on this %specific
%given dataset} and how to efficiently enable 
%such reasoning, which is often computationally 
%hard.

\vspace{0.5em}
\noindent
{\bf \textit{Relational Queries over 
Incomplete Information}.}
This paper is %heavily
inspired by
%by the database community, which is
%no stranger to
the \textit{algorithmic}
and \textit{theoretical} foundations of 
running {\em relational queries
over incomplete information}~\cite{Alicebook}.
In traditional database theory,
there are multiple ways of representing
incomplete information, starting from the 
Codd table, or the conditional table (c-table),
all the way to the recently studied probabilistic 
conditional table (pc-table)~\cite{PDBBOOK}. Over
each of these representations of
incomplete information,
one can define the corresponding 
semantics of a relational query.
In this paper, we focus on the 
weak representation system built upon
the Codd table, as illustrated in 
Figure~\ref{fig:sureanswer}.
Given a Codd table
$T$ with constants and $n$ variables
over domain $\mathcal{D}_v$
(each variable only appears once and
represents the incomplete information
at the corresponding cell),
it represents $|\mathcal{D}_v|^n$
many \textit{possible worlds} $rep(T)$,
and a query $\texttt{Q}$
over $T$ can be defined as
returning the \textit{certain answers}
that \textit{always} appear in the answer of 
$\texttt{Q}$ over each possible 
world:
%\vspace{-0.5em}
\[
sure(\texttt{Q}, T) = \cap\{\texttt{Q}(I) | I \in rep(T)\}.
\]
Another line of work with similar
spirit is \textit{consistent query
answering}, which was first introduced
in the seminal work by Arenas, Bertossi, and Chomicki~\cite{DBLP:conf/pods/ArenasBC99}.
Specifically, given an inconsistent 
database instance $D$, it defines a set of repairs $\mathcal{R
}_D$, each of which is a consistent database instance.
Given a query $\texttt{Q}$, a tuple $t$ is a {\em consistent answer}
to $\texttt{Q}$ if and only if $t$ appears in \textit{all 
answers} of $\texttt{Q}$ evaluated on every consistent 
instance $D' \in \mathcal{R}_D$. 

Both lines of work lead to a similar way of
thinking in an effort to reason about
data processing over incomplete information, i.e., 
{\em to reason about 
certain/consistent answers over all possible 
instantiations of incompleteness and uncertainty.}

\vspace{0.5em}
\noindent
{\bf \emph{Learning Over
Incomplete Information: Certain
Predictions (CP).}}
%
The traditional database view provides us a powerful
tool to reason about the impact of data incompleteness 
on downstream operations.
In this paper, we take a natural step and 
extend this to machine learning (ML) --- given a Codd table $T$,
its $|\mathcal{D}_v|^n$ many
possible worlds $rep(T)$, and
an ML classifier $\mathcal{A}$, 
one could train one 
ML model $\mathcal{A}_{I}$ for each
possible world $I \in rep(T)$. 
Given a test example
$t$, we say that $t$ can be {\em certainly predicted (CP'ed)} if 
$\forall I \in rep(T)$, $\mathcal{A}_{I}(t)$ always 
yields the same class label,
as illustrated in Figure~\ref{fig:sureanswer}.
This notion of certain prediction (CP) offers a canonical view of the impact from training classifiers on top of incomplete data.
Specificlly, we consider the following two 
CP queries:

\begin{itemize}
    %\vspace{-0.5em}
    \item[\textbf{(Q1)}] \textbf{Checking Query} --- Given a test data example, determine whether it can be CP'ed or not;
    % \vspace{-0.5em}
    \item[\textbf{(Q2)}] \textbf{Counting Query} --- Given a test data example that \emph{cannot} be CP'ed, for each possible prediction, compute the number of classifiers that \textit{support} this prediction.
\end{itemize}

When no assumptions are made about the classifier, Q1 and Q2 are,
not surprisingly, hard.
In this paper, we focus on (1)
developing efficient 
solutions to both Q1 and Q2
for a specific family of classifiers,
while (2) in the meantime,
trying to understand the
empirical implication and
application of CP to
the emerging research topic of
\textit{data cleaning for machine learning}.

\vspace{0.5em}
\noindent
{\bf \emph{Efficient CP
Algorithm for Nearest Neighbor 
Classifiers.}} We first study 
efficient algorithms to answer
both CP queries for 
%some family
%of classifiers. Specifically,
%we focus on 
K-nearest neighbor (KNN) classifier, one of the most popular classifiers used in practice.
Surprisingly, we show that,
\textit{both CP queries can 
be answered in polynomial time,
in spite of there being exponentially
many possible worlds}!

Moreover, these algorithms can be made 
very efficient. For example,
given a Codd table with $N$ rows and at most $M$ possible versions for rows with missing values, 
%with $n$ rows and $d$ columns and $nd$ variables
%over domain $\mathcal{D}_v$,
we show that answering 
both queries only take 
$\mathcal{O} \left(N \cdot M \cdot (\log(N\cdot M) +  K \cdot \log N ) \right)$. For Q1 in the binary 
classification case, we can
even do 
$\mathcal{O} (N \cdot M)$!
This makes it possible to efficiently
answer both queries for the KNN classifier,
a result that is both 
\textit{surprising} (at least to us),
\textit{new}, and
\textit{technically non-trivial}.

%\noindent
{\em \underline{Discussion}: Relationship with 
answering KNN queries 
over probabilistic databases.} As we will see
later, our result can be used to
evaluate a KNN classifier over a 
tuple-independent database,
in its standard semantics~\cite{10.1145/2213556.2213588,10.1145/2955098,10.5555/1783823.1783863}.
Thus we hope to draw the reader's attention 
to an interesting line of work of
evaluating KNN
\textit{queries} over a probabilistic database
in which the user wants the system to return 
the probability of a given (in our setting,
training) tuple that is 
in the top-K list of a query. 
Despite the similarity of the naming
and the underlying data model,
we focus on a different problem in this paper
as we care about the result of a KNN \textit{\underline{classifier}} instead of a KNN \textit{\underline{query}}.
Our algorithm is very different and heavily  relies on the structure of the classifier.
%\ww{Should we move this discussion to related work?}

\vspace{0.5em}
\noindent
{\bf \emph{Applications to Data Cleaning for Machine Learning.}} The above 
result is not only of theoretical 
interest, but also has an interesting
empirical implication --- \textit{intuitively,
the notion of CP provides us a way 
to measure the relative importance 
of different variables in the Codd table
to the downstream classification accuracy}.
\update{Inspired by this intuition,
we study the efficacy of CP in the imporant application of ``data cleaning for machine learning (DC for ML)''~\cite{krishnan2017boostclean,DBLP:journals/pvldb/KrishnanWWFG16}.
Based on the CP framework,
we develop a novel algorithm CPClean that
prioritizes manual cleaning 
efforts given a dirty dataset.}

Data cleaning (DC) is often an important prerequisite step in the entire pipeline of an ML application.
Unfortunately, most existing work
considers DC as a standalone exercise without considering its impact on downstream ML applications
(exceptions include exciting seminal work such as
ActiveClean~\cite{DBLP:journals/pvldb/KrishnanWWFG16} and BoostClean~\cite{krishnan2017boostclean}). Studies have shown that such \emph{oblivious} data cleaning may not necessarily improve downstream ML models' performance~\cite{li2019cleanml}; worse yet, it can sometimes even degrade ML models' performance due to Simpson's paradox~\cite{DBLP:journals/pvldb/KrishnanWWFG16}. 
We propose a novel ``DC for ML'' framework built on top of certain predictions.
In the following discussion, we assume a standard setting for building ML models, where we are given a training set $D_{\text{train}}$ and a validation set $D_{\text{val}}$ that are drawn independently from the same underlying data distribution.
We assume that $D_{\text{train}}$ may contain missing information  whereas $D_{\text{val}}$ is complete.

The intuition of our framework is
as follows.
When the validation set is sufficiently large, if Q1 returns \verb|true| for every data example $t$ in $D_{\text{val}}$, then with high probability cleaning $D_{\text{train}}$ will not have impact on the model accuracy.
In this case we can immediately finish without any human cleaning effort.
Otherwise, some data examples cannot be CP'ed, and our goal is then to 
clean the data such that all these
examples can be CP'ed.
\emph{Why is this sufficient}?
The key observation is that, as long as a tuple $t$ can be CP'ed, 
the prediction will remain
the same regardless of further cleaning efforts.
That is, even if we clean the whole $D_{\text{train}}$, the prediction for $t$ (made by the classifier using the \emph{clean} $D_{\text{train}}$) will remain the same, simply because the final clean version is one of the possible worlds of $D_{\text{train}}$ that has been included in the definition of CP!

To \emph{minimize} the number of tuples in $D_{\text{train}}$ being cleaned until all data examples in $D_{\text{val}}$ are CP'ed, we further propose a novel optimization algorithm based on
the principle of \emph{sequential information maximization}~\cite{Chen2015SequentialIM}, exploiting the counts in Q2 for each example in $D_{\text{val}}$ that cannot be certainly predicted.
The optimization algorithm is \emph{iterative}: Each time we pick the next example in $D_{\text{train}}$ (to be cleaned) based on its potential impact on the ``degree of certainty'' of $D_{\text{train}}$ after cleaning (see Section~\ref{sec:seq-info-max} for more details).
%
%As depicted in Figure~\ref{fig:cc-workflow}, we employ a (sufficiently large) validation/test set $D_{\text{val}}$ to forecast the generalization error of the ML model built (using algorithm $\mathcal{A}$, e.g., $K$-nearest neighbor).


%\vspace{0.5em}
%\noindent
%Our experimental evaluation shows that our ``DC for ML'' framework built on top of consistent classification can significantly outperform existing work across a variety of real-world datasets.
%trying to minimize the cleaning overhead.


%\begin{figure*}
%    \centering
%    \includegraphics[width=0.9\textwidth]{Figures/workflow.png}
%    \vspace{-1em}
%    \caption{The workflow of cleaning for ML under consistent classification, given a dirty training set $D$ with its possible world $\mathcal{W}$, an ML algorithm ${\cal A}$, and a validation set $D_{val}$. }
%    \vspace{-1em}
%    \label{fig:cc-workflow}
%\end{figure*}


%\vspace{0.5em}

%\medskip
% \vspace{-0.5em}
\paragraph*{Summary of Contributions}
In summary, this paper makes the following contributions:
\begin{itemize}
    % \vspace{-0.1em}
    \item [\textbf{(C1)}] We propose \textit{certain predictions}, as well as its two fundamental queries/primitives (checking and counting), as a tool to study the impact of incomplete data on training ML models. 
    % \vspace{-0.1em}
    \item [\textbf{(C2)}] We propose efficient solutions to the two fundamental CC queries for nearest neighbor classifiers, despite the hardness of these two queries in general.
    % \vspace{-0.1em}
    \item [\textbf{(C3)}] We propose a novel ``DC for ML'' approach, CPClean, built on top of the CP primitives that significantly outperforms existing work in terms of classification accuracy, %across a variety of real-world datasets, 
    with mild manual cleaning effort.
\end{itemize}
%\vspace{-0.5em}

%\vspace{-1em}
\paragraph*{Moving Forward}
%As an early effort focusing on the problem
%of ``certain prediction,'' this paper 
%just takes one of the early steps ---
Just like the study of consistent query
answering that focuses on specific
subfamilies of queries, in this paper we have focused on a specific  
type of classifier, namely the
KNN classifier,
in the CP framework.
This allows us to design efficient 
algorithms specific to this workload.
In the future, it is interesting to extend our study to 
a more diverse range of classifiers ---
either to develop efficient exact 
algorithms or to explore efficient 
approximation algorithms. It is also interesting to 
extend our CP-based data cleaning framework
to more types of classifiers.

%\vspace{-1em}
\paragraph*{Paper Organization} This paper is organized as follows.
We formalize the notion of certain
predictions, as well as the two primitive queries Q1 and Q2 ( Section~\ref{sec:preliminary}).
We then propose efficient algorithms
in the context of nearest neighbor classifiers (Section~\ref{sec:cc-knn}).
We follow up by proposing our novel ``DC for ML'' framework exploiting CP (Section~\ref{sec:cc:general}).
We report evaluation results in Section~\ref{sec:evaluation}, summarize related work in Section~\ref{sec:related-work}, and conclude the paper in Section~\ref{sec:conclusion}.

%Specifically, for the decision query \textbf{Q1}, we provide an exact solution that requires only \emph{linear} time with respect to the size of the training data.

% We can also provide exact solutions to \textbf{Q2}, though the efficiency of the solutions depends on which semantic of \textbf{Q2} we choose.
% For example, if we are just interested in providing individual examples of problematic cleaning that leads to inconsistency, then we can leverage the same, scan-based algorithm for answering \textbf{Q1} so that only linear time is required;
% if, on the other hand, we are more interested in the ``counting semantic'' that provides distributional information regarding inconsistency, then we need a more sophisticated, sort-based algorithm whose time complexity depends on not only the data size but also the $K$ in the $K$-NN classifier itself.

% %To improve efficiency, one can further use a simple approximate solution based on sampling -- if approximation is acceptable (see Section~\ref{sec:cc:general}).

%We set aside a small validation set $D_{val}$ (e.g., 20 examples) from the input dataset. Since we know the ground-truth predictions of $D_{val}$, we can estimate the expected impact of cleaning on ML for a given $D$ and ${\cal A}$. 

%\smallskip
%\noindent \underline{(1) Consistent Classification in Cleaning for ML.} Intuitively, data cleaning affects a particular ML algorithm $\mathcal{A}$ (e.g., kNN, logistic regression, etc) if there exists some possible cleaned version $D'$ of a given dataset $D$, such that the ML model trained on the $D'$, denoted as $\mathcal{A}_{D'}$ and the ML model trained on the original instance $D$, denoted as $\mathcal{A}_{D}$, would generate different predictions for some unseen data point $t$, namely, $\mathcal{A}_{D'}(t) \neq \mathcal{A}_D(t)$. 
%%%
%We say that the data point $t$ can be \emph{consistently classified} if for any two versions of the dataset, $D_1, D_2 \in \{D \cup {\cal D}_c\}$, where ${\cal D}_c$ represents all possible clean versions of $D$, we have $\mathcal{A}_{D_1}(t) = \mathcal{A}_{D_2}(t)$.
%%
%Note that ${\cal D}_c$ contains possible candidate repairs of $D$, which are typically generated by automated data cleaning algorithms~\cite{DBLP:books/acm/IlyasC19}, and the costly process of data cleaning is involving human experts to confirm or pick a candidate repair.  The fact that a data point $t$ can be consistently classified suggests that, no matter which candidate repair a human cleaner might pick, the prediction of $t$ will not change, which precisely means that data cleaning has no impact on the ML algorithm $\mathcal{A}$'s prediction of $t$. 

% Given $D$, ${\cal D}_c$, and $\mathcal{A}$, the three questions can be stated as follows under consistent classification: 
% \begin{itemize}
%     \item \textbf{Q1 (Decision)}: Can a data point $t$ be consistently classified?
%     \item \textbf{Q2 (Explanation)}: Why $t$ cannot be consistently classified?
%     \item \textbf{Q3 (Optimization)}: Assuming human cleaner has a unit cost of cleaning every tuple in $D$, how to minimize the number of tuples humans need to clean such that $t$ can be consistently classified. 
% \end{itemize}

% While the semantic of \textbf{Q1} and \textbf{Q3} are clear, \textbf{Q2} can be addressed in multiple ways.
% For example, one could provide an answer to \textbf{Q2} by responding with two possible cleaning outcomes of the training data that lead to contradictory classification results;
% or, alternatively, one could instead respond with the fractions of possible cleaning outcomes that lead to different classification results (e.g., 70\% of the outcomes result in classifying the data point with label ``1,'' whereas the rest 30\% lead to label ``0'').
% In our study, we have further explored these alternative semantics.

% % %Given a dirty database instance $D$, its repairs $\mathcal{R }_D$ and an ML classifier $\mathcal{A}$, one could
% % train one ML model $\mathcal{A}_{D'}$ for each consistent 
% % instance $D' \in \mathcal{R}_D$. Given a test example
% % $t$, we say that $t$ can be {\em consistently classified} if 
% % all $\mathcal{A}_{D'}(t)$ predicts to the same class.


% % Specifically, given an arbitrary data point $x$, a classifier $h$, and a training dataset $D$ for $h$ that needs cleaning, we want to know whether $x$ can be classified consistently by $h$, regardless of how we clean $D$.
% % In other words, how to clean $D$ has no impact on the accuracy of $h$.
% % Clearly, if all data points can be consistently classified, then we do not need to worry about which DL algorithm to choose.



% % \smallskip
% % \noindent \underline{(2) Approximate Solutions for Any ML Models.} 

% The computational complexity to answer the three questions using consistent classification depends on the space of repairs ${\cal D}_c$ of $D$ and the downstream ML algorithm ${\cal A}$. An exact solution to CC for an arbitrary classifier requires a brute-force solution that trains a classifier for every clean world to examine the consistency of the classification results. Hence, we will propose approximate solutions based on sampling. 

% %To improve efficiency, one can further use a simple approximate solution based on sampling -- if approximation is acceptable (see Section~\ref{sec:cc:general}).

% \smallskip
% \noindent \underline{(2) Efficient Solutions to Q1 and Q2 for KNN.}
% \textcolor{red}{Xu: need to provide some graphics here illustrating the key ideas of our algorithms, rather than dry English.}
% Specifically, for the decision query \textbf{Q1}, we provide an exact solution that requires only \emph{linear} time with respect to the size of the training data.
% We can also provide exact solutions to \textbf{Q2}, though the efficiency of the solutions depends on which semantic of \textbf{Q2} we choose.
% For example, if we are just interested in providing individual examples of problematic cleaning that leads to inconsistency, then we can leverage the same, scan-based algorithm for answering \textbf{Q1} so that only linear time is required;
% if, on the other hand, we are more interested in the ``counting semantic'' that provides distributional information regarding inconsistency, then we need a more sophisticated, sort-based algorithm whose time complexity depends on not only the data size but also the $K$ in the $K$-NN classifier itself.

%\smallskip
%\noindent \underline{(2) Addressing the Decision Problem for KNN.}

%\smallskip
%\noindent \underline{(3) Addressing the Optimization Problem for KNN.}


% \smallskip
% \noindent \underline{(3) Efficient Solutions to Q3 for KNN.}

% Finally, while one can in theory obtain an exact solution to \textbf{Q3} by adopting a breadth-first (BFS) kind of search strategy that first tries repairing each individual data point, then pairs of data points, then triples, and so on so forth until a consistent state is reached, such a strategy is time-consuming and probably has little practical interest.
% After all, the overhead of cleaning ten data points may not differ too much from cleaning just five.
% Therefore, we take a more pragmatic attitude here by designing a greedy algorithm that does not guarantee optimality but converges fast in practice.
% In each greedy step, we pick a data point such that cleaning of it can result in maximum information gain (i.e., maximum reduction in the number of possible datasets after cleaning).
% Our evaluation on various datasets with a broad range of data cleaning algorithms has demonstrated the effectiveness of this greedy algorithm.


==> [arXiv] Certain Prediction/Preliminary.tex <==
% !TEX root = CC.tex
%\vspace{-0.5em}
\section{Certain Prediction (CP)}
\label{sec:preliminary}

In this section, we describe the 
\textit{certain prediction} (CP) framework, which 
is a natural extension of the notion 
of \textit{certain answer} for 
query processing over Codd tables~\cite{Alicebook} 
to machine learning.
We first describe our data model and then
introduce two CP queries.

\paragraph*{Data Model} 

We focus on standard supervised ML settings: 
\begin{enumerate}
\item Feature Space $\mathcal{X}$: without 
loss of generality, we assume that every
data example is drawn from a domain $\mathcal{X} = \mathbb{D}^d$, i.e., a $d$ dimensional
space of data type $\mathbb{D}$.
\item Label Space $\mathcal{Y}$: we assume
that each data example can be classified into
one of the labels in $\mathcal{Y}$.
\item Training Set $D_{train} \subseteq 
\mathcal{X} \times \mathcal{Y}$ is drawn
from an \textit{unknown} distribution $\mathcal{P}_{\mathcal{X}, \mathcal{Y}}$.
\item Test Set $D_{test} \subseteq 
\mathcal{X}$
(Validation Set $D_{val}$)
is drawn from the marginal distribution $\mathcal{P}_{\mathcal{X}}$ of the joint distribution $\mathcal{P}_{\mathcal{X}, \mathcal{Y}}$.
\item Training Algorithm $\mathcal{A}$:
A training algorithm $\mathcal{A}$ is
a functional that maps a given training
set $D_{train}$ to a function $\mathcal{A}_{D_{train}}: \mathcal{X} \mapsto \mathcal{Y}$. Given a test example 
$t \in D_{test}$, $\mathcal{A}_{D_{train}}(t)$
returns the prediction of the trained
classifier on the test example $t$.
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/\figfmt/possible-worlds-s}
    % \vspace{-1em}
    \caption{Example of a dataset with incomplete information, its representation as an \emph{incomplete dataset}, and the induced set of \emph{possible worlds}.}
    \label{fig:possible-worlds}
\end{figure}


%\vspace{0.5em}
\noindent
{\bf \emph{Incomplete Information in the Training
Set}} In this paper, we focus on the case in which
there is incomplete information in the
training set. We define an \textit{incomplete
training set} as follows.

Our definition of an incomplete
training set is very similar to a
block tuple-independent 
probabilistic database~\cite{PDBBOOK}.
However,
we do assume that there is no
uncertainty on the label and we do not have 
access to the probability distribution of each tuple.
% Moreover, we will not 
% define the probability
% of each tuple, as this is
% not relevant to this work
% and we
% often cannot acquire it 
% in our data cleaning application.
%
\begin{definition}[Incomplete Dataset] \label{def:incomplete-dataset}
An \emph{incomplete dataset}
\[
\mathcal{D} = \{(\mathcal{C}_i, y_i) : i=1,...,N\}
\]
is a finite set of $N$ 
pairs where each $\mathcal{C}_i = \{ x_{i,1}, x_{i,2}, ... \} \subset \mathcal{X}$ is a finite number 
of possible feature vectors of the $i$-th data example and each $y_i \in \mathcal{Y}$ is its corresponding class label.
\end{definition}

According to the semantics of $\mathcal{D}$, the $i$-th data example can take any of the values from its corresponding 
\textit{candidate set} $\mathcal{C}_i$. The space of all possible ways to assign values to all data points in $\mathcal{D}$ is captured by the notion of possible worlds.
Similar to a block tuple-independent 
probabilistic database,
an incomplete dataset can define a
set of \textit{possible worlds}, each of which is a 
dataset without incomplete information.

\begin{definition}[Possible Worlds] \label{def:clean-world}
Let $\mathcal{D} = \{(\mathcal{C}_i, y_i) : i=1,...,N\}$ be an incomplete dataset. We define the set of possible worlds $\mathcal{I}_\mathcal{D}$, given the incomplete dataset $\mathcal{D}$, as
$$
\mathcal{I}_{\mathcal{D}} \ = \
 \left\{
 D = \{(x_i', y_i')\} :
 |D| = |\mathcal{D}| \wedge 
 \forall i.~x_i' \in \mathcal{C}_i \wedge y_i' = y_i 
 \right\}.
$$
\end{definition}

In other words, a 
\emph{possible world} represents 
one complete dataset $D$ that is generated from $\mathcal{D}$ by replacing every
candidate set $\mathcal{C}_i$ with one of its candidates $x_j \in \mathcal{C}_i$. The set of all distinct datasets that we can generate in this way is referred to as the \emph{set of possible worlds}. If we assume that $\mathcal{D}$ has $N$ data points and the size of each $\mathcal{C}_i$ is bounded by $M$, we can see $|\mathcal{I}_{\mathcal{D}}| = \mathcal{O} (M^N)$. 

Figure~\ref{fig:possible-worlds} provides an example of these concepts. As we can see, our definition of incomplete dataset can represent both possible values for  missing cells and possible repairs for cells that are considered to be potentially incorrect.

\vspace{0.5em}
\noindent
{\bf \emph{Connections to Data Cleaning.}} 
In this paper, we 
use data cleaning as one
application to illustrate the 
practical implication of 
the CP framework. In this setting,
each possible world
can be thought of as one 
possible \emph{data repair} 
of the dirty/incomplete data.
These repairs can be generated in an arbitrary way, possibly depending on the entire dataset~\cite{rekatsinas2017holoclean}, or even some external domain knowledge~\cite{ChuKATARA}. Attribute-level data repairs could also be generated independently and merged together with Cartesian products. 
%The cleaning algorithm then works by accepting an incomplete dataset and for each data point selecting one data repair that corresponds to the ground-truth.

%, ideally the one that represents the ground truth.

We will further  
apply the assumption that any given incomplete dataset $\mathcal{D}$ is \emph{valid}. That is, for every data point $i$, we assume that there exists a \emph{true value} $x_i^*$ that is unknown to us, but is nevertheless included in the candidate set $\mathcal{C}_i$. 
%This is important as a prerequisite for any successful cleaning method. 
This is a commonly used assumption in data cleaning~\cite{DBLP:books/acm/IlyasC19}, where automatic cleaning algorithms are used to generate a set of candidate repairs, and humans are then asked to pick one from the given set.
%%
We call 
$D_\mathcal{D}^*$ the \textit{true 
possible world}, which contains 
the true value for each tuple.
When $\mathcal{D}$ is clear from the context, 
we will also write $D^*$.

%in which we define with the triplet $(\mathcal{X}, \mathcal{Y}, \mathcal{A})$. In this setting, $\mathcal{X}$ is a \textbf{\emph{feature set}} where $x \in \mathcal{X}$ is an arbitrary tuple, $\mathcal{Y}$ is a \textbf{\textit{label set}} which is finite because we are focusing on classification tasks, and $\mathcal{A}$ is a \textbf{\emph{learning algorithm}}. The learning algorithm works by accepting a \textbf{\emph{dataset}} $D = \{ (x_i, y_i) \in \mathcal{X} \times \mathcal{Y} : i = 1,...,N \}$ and returning a \textbf{\emph{classifier}} $h : \mathcal{X} \rightarrow \mathcal{Y}$. In other words, $h = \mathcal{A}(D)$.

%Machine learning models are designed to work with complete datasets, i.e. datasets without any unknown values. However, most real-world data often contains \emph{known unknowns}. These are either explicitly indicated missing values (e.g. $\texttt{null}$ values), or values that we know to be wrong (e.g. if they violate some integrity constraints). In Figure~\ref{fig:possible-worlds} we show an example of such a dataset. The first data point has an explicitly indicated $\texttt{null}$ value. The third data point also has a known unknown value because it is outside of the domain of ZIP codes for the city of Rome. In order for this unknown value to be detected, we assume that there is an integrity constraint that maps city names to sets of valid ZIP codes.


%To use this kind of dataset with a learning algorithm, we would first need to convert it to a complete dataset. One commonly used method is imputation, which involves substituting the unknown values with some replacement value given by our specific imputation method. This method could cause issues by introducing statistical bias into the data. Furthermore, it masks the unknown values and makes them indistinguishable from known values. Another method is to introduce a boolean column that would serve as a missing value indicator used to mark values that were originally unknown. This method relies on the assumption that the learning algorithm can automatically deduce the meaning of the missing value indicator, which may not necessarily be possible.

%In this work, we aim for an explicit treatment of unknown values in a logically coherent manner. Thus, the fact that a value is missing should not be treated as a fact about the world, but merely as a fact about our dataset. As a consequence of this, we have to consider that the field in question can take any value from its domain, subject to explicitly defined restrictions modeled with integrity constraints. To express this notion formally, we generalize the previously defined concept of a dataset $D$.


%The semantics of this incomplete dataset is that $\mathcal{C}_i$ defines the set of possible values that can get assigned to the $i$-th data point. We note that the special case $\mathcal{D} = \{(\mathcal{C}_i, y_i) : i=1,...,N, |\mathcal{C}_i|=1\} $ is equivalent to a regular dataset $D$, which we refer to as a \textbf{\emph{complete dataset}}, or simply, a dataset. This makes $\mathcal{D}$ a generalization of $D$.

%Many other generalizations of the relational model have been developed over the years with the goal of handling incomplete information. Among of the earliest ones is the Codd table that represents unknown values either by $\texttt{null}$ indicators with the interpretation that they could take any valid value from the attribute domain. Our representation is relatively similar to or-sets (proposed by Imielinski et al. in~\cite{Imielinski1991}) because the values of the domain are explicitly given. The main difference is that we are restricting our representation to tuple-level or-sets and we don't permit any nesting of or-sets. Furthermore, as opposed to some more advanced representations, ours does not permit constraints defined jointly over multiple tuples. Instead, we treat all tuples completely independently. This restriction makes our treatment of unknown values \emph{conservative}, compared to other methods.

\subsection{Certain Prediction (CP)}

When we train an ML model over
an incomplete dataset, we can define
its semantics in a way that is very 
similar to how people define 
the semantics for data processing over
probabilistic databases ---
we denote $\mathcal{A}_{D_i}$
as the classifier that was trained on the possible world $D_i \in \mathcal{I}_\mathcal{D}$. 
Given a test data point $t \in \mathcal{X}$, 
we say that it can be \textit{certainly
predicted} (CP'ed) if 
all classifiers trained on 
all different possible worlds
agree on their predictions:

\begin{definition}[Certain Prediction (CP)] \label{def:cc}
Given an incomplete dataset $\mathcal{D}$ with its set of possible worlds $\mathcal{I}_\mathcal{D}$ and a data point $t \in \mathcal{X}$, we say that a label $y \in \mathcal{Y}$ can be \emph{certainly predicted} with respect to a learning algorithm $\mathcal{A}$ if and only if
$$
\forall D_i \in \mathcal{I}_\mathcal{D}, \mathcal{A}_{D_i}(t) = y.
$$
\end{definition}

%\vspace{0.5em}
\noindent
{\bf \emph{Connections to Databases.}} 
The intuition behind this definition is rather 
natural from the perspective of database theory. In the context of Codd table,
each \texttt{NULL} variable 
can take values in its domain, which
in turn defines exponentially many
possible worlds~\cite{Alicebook}. Checking 
whether a tuple is in the answer of
some query \texttt{Q} is to check whether such a 
tuple is in the result of 
each possible
world.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.6\textwidth]{Figures/\figfmt/consistent-classification-overview-4-s}
    % \vspace{-1em}
    \caption{Illustration of certain prediction, and two queries: checking query (Q1) and counting query (Q2).}
    \label{fig:cc}
\end{figure}

\paragraph*{Two Primitive CP Queries}

Given the notion of \textit{certain prediction},
there are two natural 
queries that we can ask.
The query $Q1$ represents a \emph{decision problem} that checks if a given label can be predicted in \textit{all} possible worlds. The query $Q2$ is an extension of that and represents a \emph{counting problem} that returns the number of possible worlds that support each prediction outcome.
Figure~\ref{fig:cc} illustrates both
queries and we formally define
them as follows.

\begin{definition}[Q1: Checking]
Given a data point $t \in \mathcal{X}$, an incomplete dataset $\mathcal{D}$ and a class label $y \in  \mathcal{Y}$, we define a query that checks \emph{if all possible world} permits $y$ to be predicted:
$$
Q1(\mathcal{D}, t, y) := \begin{cases}
	\mathtt{true}, & \mathrm{if} \ \forall D_i \in \mathcal{I}_\mathcal{D}, \mathcal{A}_{D_i}(t) = y; \\
	\mathtt{false}, & \mathrm{otherwise}.
\end{cases}
$$
\end{definition}

\begin{definition}[Q2: Counting]
Given a data point $t \in \mathcal{X}$, an incomplete dataset $\mathcal{D}$ and a class label $y \in  \mathcal{Y}$, we define a query that returns the \emph{number of possible worlds} that permit $y$ to be predicted:
$$
Q2(\mathcal{D}, t, y) := | \{ D_i \in \mathcal{I}_\mathcal{D} : \mathcal{A}_{D_i}(T) = y \}|.
$$
\end{definition}

%\vspace{0.5em}
\noindent
\textbf{\textit{Computational Challenge.}} If we do not make any assumption about the learning algorithm $\mathcal{A}$, we have no way of determining the predicted label $y=\mathcal{A}_{D_i}(t)$ except for running the algorithm on the training dataset. Therefore, for a general classifier treated as a black box, answering both $Q1$ and $Q2$ requires us to apply a brute-force 
approach that iterates over each $D_i \in \mathcal{I}_\mathcal{D}$, produces $\mathcal{A}_{D_i}$, and predicts the label. 
Given an incomplete dataset with
$N$ data examples each of which has
$M$ clean candidates, the computational cost of this naive algorithm for both queries would thus be $\mathcal{O} (M^N)$.

This is not surprising. 
However, 
%Just like traditional database theory, the goal
%of this work is to study both queries
%for a specific family of classifiers.
as we will see later in this paper,
for certain types of classifiers, such as K-Nearest Neighbor classifiers,
we are able to design efficient
algorithms for both queries.

\vspace{0.5em}
\noindent
{\bf \emph{Connections to Probabilistic 
Databases.}}
Our definition of certain prediction 
has strong connection to the theory of probabilistic 
database~\cite{PDBBOOK} --- in fact, Q2 can be seen as a natural 
definition of evaluating
an ML classifier over a block
tuple-independent probabilistic database 
with uniform prior.

% In fact, we can 
% extend our algorithm to handle 
% the case of non-uniform probability
% distributions, thus support
% a standard block
% tuple-independent probabilistic database.

Nevertheless, unlike traditional relational queries over a probabilistic database, our ``query''
is an ML model that has very different structure.
As a result, despite the fact that
we are inspired by many seminal works
in probabilistic database~\cite{10.1145/2213556.2213588,10.1145/2955098,10.5555/1783823.1783863}, 
they are not applicable to our settings and 
we need to develop new techniques.
%and algorithms.
%for our specific setting.

\vspace{0.5em}
\noindent
{\bf \emph{Connections to Data Cleaning.}}
It is easy to see that, if $Q1$
returns \texttt{true} on a test example
$t$, obtaining 
more information (by cleaning) for
the original training set 
will not change the prediction 
on $t$ at all! This is because 
the true possible world $D^*$
is one of the possible worlds in
$\mathcal{I}_\mathcal{D}$.
Given a large enough test set,
if $Q_1$ returns \texttt{true} for
all test examples, cleaning the training set
in this case might not
improve the quality of ML models
at all!

Of course, in practice, it is 
unlikely that all test examples 
can be CP'ed. In this more realistic
case, $Q_2$ provides a ``softer''
way than $Q_1$ to measure the 
\textit{degree of certainty/impact}.
As we will see later, we can use this
as a principled proxy of the impact
of data cleaning on downstream ML
models, and design efficient algorithms to prioritize which uncertain cell 
to clean in the training set.

%\vspace{0.5em}
%\noindent
%{\bf \emph{Connections to Multiple
%Imputation.}} From a statistics
%perspective, $Q2$ can be seen 
%as the exact counterpart of 
%``multiple imputation''~\cite{XXX}
%that only \textit{samples} a set of possible worlds, which is a popular 
%technique to deal with
%missing values in training
%ML models. 
%As a byproduct, our 
%algorithm provides a very
%efficient way for some version
%of multiple imputation problem, \xc{I also have trouble parsing this sentence}
%an interesting result on 
%its own right. 
%\ww{Can we be more specific here about ``some version of multiple imputation problem''?}
%As we will see, this 
%efficient algorithm is 
%crucial to apply 
%our framework 
%to our data cleaning application. 


%In this section we define two types of queries over incomplete datasets. Both of these queries can be used as primitives, not only to implement an augmented classifier $h^{+}$, but also have interesting applications such as data cleaning, which we present in Section 4.

% Clearly, Q2 can have different semantics depending on the content of the \textbf{summary}.
% In this paper, we focus on the following semantics, which we believe are natural and practically useful:
% \begin{enumerate}
%     \item \emph{Representative semantics}, where $\textbf{summary}(\mathcal{D}_y)$ returns one single, representative element $D\in\mathcal{D}_y$;
%     \item \emph{Counting semantics}, where $\textbf{summary}(\mathcal{D}_y)$ returns $|\mathcal{D}_y|$.
%     \item \emph{Enumeration semantics}, where $\textbf{summary}(\mathcal{D}_y)$ returns the entire inconsistency region $\mathcal{D}_y$.
% \end{enumerate}
% Two remarks are in order. First, we intentionally leave some details to be filled in for the representative semantics in terms of picking which element from $D_y$. One can employ various policies, e.g., based on some ranking mechanism or just randomly picking one.
% Second, although the counting semantics and enumeration semantics look quite similar, they can differ in terms of computational complexity.
% While the enumeration semantics could be computationally very inefficient by definition, we can have efficient algorithms for the counting semantics without having to enumerate $\mathcal{D}_y$.


%If the answer to the previous query is negative, then we may want to investigate what has lead to that outcome, which is generally undesirable. We want to study each unique label $y \in \mathcal{Y}$ and define the subset of the clean world that will always produce a classifier which predicts that label for the unseen data example $\mathbf{x}$. More formally, for every $y \in \mathcal{Y}$, we define:
%$$
% \mathcal{D}_y := \{ D \in \mathcal{D} : h_D (\mathbf{x}) = y \}
%$$

%This query has two possible versions:
%\begin{enumerate}
%    \item[Q2.1:] For every $y \in \mathcal{Y}$, return at least one element of $\mathcal{D}_y$.
%    \item[Q2.2:] For every $y \in \mathcal{Y}$, return the size of $\mathcal{D}_y$.
%\end{enumerate}

%\stitle{Cleaning Query (Q3)} \label{sec:cc:query:q3}
%\vspace{-0.5em}

\iffalse
\subsubsection{Cleaning Query (Q3)} \label{sec:cc:query:q3}

Following up with the fact that $\mathbf{x}$ cannot be consistently classified, Q3 then aims to find an optimal way to clean $D$ such that $\mathbf{x}$ can be consistently classified after cleanup while at the same time the number of points in $D$ being cleaned is minimized.

Assume a subset of records $E \subseteq D$ is cleaned by humans. We use $\mathcal{W}_E$ to denote the remaining set of worlds in $\mathcal{W}$ that conforms to the human cleaning decisions in $E$.

% Here, we assume there is an oracle that serves as the ground truth, cleaned version $D^*$ of $D$.
% We can inquire this oracle to return the cleaned version $\mathbf{x}_i^*$ from $D^*$ of a data point $\mathbf{x}_i\in D$ being cleaned.

% Given a subset $E\subseteq D$, we use $\bar{E}$ to represent its complement in $D$.
% Moreover, we use $\bar{\mathcal{E}}\subseteq\mathcal{D}$ to represent the \emph{residual world} after $E$ is cleaned up. 
% In other words, $\bar{\mathcal{E}}$ contains all data points from $\bar{E}$ cleaned by the oracle, and all data points from $\bar{E}$ cleaned in an arbitrary way.
% % More formally, $\bar{\mathcal{E}} = \bar{E} \cup \{ \mathbf{x}_i^* : \mathbf{x}_i \in E \} $.
% We can now define Q3 as follows:

\begin{definition}[Cleaning Query]
Given an $\mathbf{x}\in\mathcal{X}$ that is not consistently classifiable with respect to the possible worlds $\mathcal{W}$ derived from $D$ and the ML algorithm $\mathcal{A}$, 
\[
Q3(\mathbf{x}, \mathcal{W}, {\cal A}) := \argmin_{E \subseteq D} |E|, \text{ s.t., } Q1(\mathbf{x}, \mathcal{W}_E, {\cal A}) = \verb|true|.
\]
\end{definition}
Note that the result of Q3 does not need to be unique.

\mg{Above is the definition of the optimal set. So I think we should define what our Q3 will achieve (will be near optimal instead). I propose this:}

{\color{purple} 
Given a set of possible worlds $\mathcal{W}_{\pi}$ derived from a training set $D_{\text{train}}$ and a policy $\pi$, $\mathcal{Q3}$ aims to clean a set of feature vectors $D_{\pi}$, such that $Q1(\mathbf{x}, \mathcal{W}_{\pi}, \mathcal{A})=\verb|true|, \  \forall \mathbf{x}\in D_{\text{val}}$, while minimizing the amount of human effort for cleaning. More formally, we define the cleaning query as follows.
\begin{definition}[Cleaning Query]
Provided a direct access to the set of features in $D_{val}$ that are not consistently classifiable with respect to the possible worlds $\mathcal{W}$ derived from $D_{\text{train}}$ and the ML algorithm $\mathcal{A}$, we denote the set of training data points cleaned by a policy $\pi$ such that
$$\mathcal{Q}3(D_{\text{val}}, \mathcal{W}_{\pi}, \cal{A})\coloneqq \argmin_{D_{\pi}\subseteq D_{\text{train}}} |D_{\pi}|$$
such that $\mathcal{Q}1(\mathbf{x}, \mathcal{W}_{\pi}, \mathcal{A})=\verb|true|$, $\forall \mathbf{x} \in D_{val}$.
% As we previously introduced, we denote the set of cleaned data points achieved by running a policy $\pi$ a total of $k$ times by $D_{\pi}^{[k]}$.
% We therefore define $\mathcal{Q}3$ as the set of training data points cleaned by a policy $\pi$ such that $$\mathcal{Q}3(D_{\text{val}}, \mathcal{W}_{\pi}, \cal{A})\coloneqq \argmin_{D_{\pi}\subseteq D_{\text{train}}} |D_{\pi}|$$
\end{definition}
}

\fi

% We study general solutions to the CC problem without assumptions on the training set $D$ and the classifier $h$.

% %\subsection{An Exact Approach}

% Apparently, we can apply the following brute-force approach to provide \emph{exact} answers to the CC queries defined previously.

% \begin{procedure}[Exact Approach to Q1 and Q2]\label{proc:brute-force}
% For each possible training set $D_i \in \mathcal{D}$, we train the corresponding classifier $h_i$ and then use $h_{i}$ to make prediction for $\mathbf{x}$.
% \end{procedure}
% We can answer Q1 and Q2 based on the results $\mathcal{H}=\{h_i(\mathbf{x}) \}_{i=1}^{|\mathcal{D}|}$:
% \begin{itemize}
%     \item \emph{Q1} -- check whether $h_1(\mathbf{x})=\cdots=h_{|\mathcal{D}|}(\mathbf{x})$;
%     \item \emph{Q2} -- compute $\mathcal{D}_y$ for each $y\in\mathcal{Y}$ based on $\mathcal{H}$ and use $\mathcal{D}_y$ to generate answers based on different semantics of Q2.
% \end{itemize}
% We need additional effort to answer Q3.
% We can enumerate all subsets of $D$ in a breadth-first manner, i.e., we start from all 1-subsets (i.e., subsets with one single element), and then all 2-subsets (i.e., subsets with two elements), and so on.
% For each subset $E\subseteq D$, we clean $E$ and run Procedure~\ref{proc:brute-force} over $\bar{\mathcal{E}}$.
% We stop whenever we find that $\mathbf{x}$ can be consistently classified.

% Clearly, none of the above algorithms is tractable when $\mathcal{D}$ is large, which is usually the case in practice.
% We next turn to an approximate approach that alleviates the efficiency issue for Q1 and Q2, at the sacrifice of providing exact answers.



% \subsection{Framework Overview}

% We first introduce three fundamental queries in consistent classification with respect to one unseen example $(\mathbf{x},y)$. We then show how the answer of these three queries can be used to address the decision problem and the optimization problem in cleaning for ML using a hold-out validation set. 



==> [arXiv] Certain Prediction/conclusion.tex <==

 \section{Conclusion}\label{sec:conclusion}
 
In this work, we focused on the
problem of understanding the impact
of incomplete information on
training downstream ML models. We present a formal study of this impact by extending the notion of \emph{Certain Answers for Codd tables}, which has been explored by the database research community for decades, into the field of machine learning, by introducing the notion of \emph{Certain Predictions} (CP).
We developed efficient algorithms to analyze the impact via CP primitives, in the context of nearest neighor classifiers.
As an application, we further proposed a novel ``DC for ML'' framework built on top of CP primitives that often significantly outperforms existing techniques in accuracy, with mild manual cleaning effort.

==> [arXiv] Certain Prediction/relatedwork.tex <==

\section{Related Work}\label{sec:related-work}



\stitle{Relational Query over Incomplete Information.} 
This work is heavily inspired by
the database literature of 
handling incomplete information~\cite{Alicebook},
consistent query answering~\cite{DBLP:conf/pods/ArenasBC99,DBLP:conf/icdt/LopatenkoB07,DBLP:series/synthesis/2011Bertossi}, and probabilistic databases~\cite{PDBBOOK}. 
While
these work targets SQL analytics, our proposed consistent prediction query targets ML analytics. 

\stitle{Learning over Incomplete Data.} The statistics and ML community have also studied the problem of learning over incomplete data. Many studies operate under certain missingness assumption (e.g., missing completeness at random) and reason about the performance of downstream classifiers in terms of asymptotic properties and in terms of
different imputation strategies~\cite{10.1007/s00521-009-0295-6}. 
In this work, we focus more on the
algorithmic aspect of this problem
and try to understand how to enable
more efficient manual cleaning
of the data.
Another flavor of work aims at developing ML models that are robust to certain types of noises, and multiple imputation~\cite{10.2307/2291635} is such a method that is most relevant to us. Our CP framework can be seen as an extreme case of multiple imputation (i.e, by trying all possible imputations) with efficient implementation (in KNN), which also enables novel manual cleaning for ML use cases. 

\update{Recently, Khosravi et al.
\cite{DBLP:journals/corr/abs-1903-01620} explored a similar semantics as ours, but for Logistic Regression
models. In this paper, we focus on efficient algorithms for nearest neighbor classifiers.}

%Despite the many fruitful research contributions in the general area of data cleaning, the dirty data problem remains challenging~\cite{DBLP:conf/sigmod/ChuIKW16}. Recent study shows that even the combination of current error detection techniques can still miss many errors in real-world datasets~\cite{abedjan2016detecting}. We refer readers to various surveys and tutorials on the broad topic of data cleaning~\cite{rahm2000data,hellerstein2008quantitative,fan2012foundations,ilyas2015trends}. The recent efforts on data cleaning focus on leveraging advanced ML techniques, including the HoloDetect system that uses few-shot learning and data augmentation for error detection~\cite{DBLP:conf/sigmod/HeidariMIR19}, the HoloClean system that uses probabilistic graph models for inferring the most likely value~\cite{rekatsinas2017holoclean}, deep-learning based methods for duplicate detection~\cite{mudgal2018deep,ebraheem2018distributed}, and the AutoER system that uses generative model for detecting duplicates using zero labeled examples~\cite{wu2019autoer}. 

\stitle{Data Cleaning and Analytics-Driven Cleaning.} The research on data cleaning (DL) has been thriving for many years. Many data cleaning works focus on performing standalone cleaning without considering how cleaned data is used by downstream analytics. We refer readers to a recent survey on this topic~\cite{DBLP:books/acm/IlyasC19}. 
%%
%The research on data cleaning (DL) has been thriving for many years. Data cleaning consists of two phases: \textit{error detection}, where various errors and violations are identified and possibly validated by experts; and \textit{error repair}, where updates are usually suggested to human experts to bring the data to a cleaner state. Many different techniques have been proposed to detect different types of errors, for example, by designing integrity constraints to capture data inconsistencies~\cite{ChuIP13VLDB}, by using quantitative and statistical techniques to detect outliers~\cite{hellerstein2008quantitative}, and by building ML models to detect duplicates~\cite{DBLP:journals/tkde/ElmagarmidIV07}. Various heuristics and techniques have also been proposed to suggest data repairs, for example, by finding the minimal set of updates to resolve violations~\cite{DBLP:conf/icde/xu13}, by performing data transformations~\cite{he2018transform}, by consulting external knowledge bases~\cite{ChuKATARA}, and by using probabilistic graphical models to reason about errors holistically~\cite{DBLP:journals/pvldb/RekatsinasCIR17}. Despite these efforts, data cleaning remains an expensive process, and humans still need to be consulted to confirm the fixes suggested by automatic cleaning algorithms~\cite{DBLP:books/acm/IlyasC19}.

%\stitle{Analytics-Driven Cleaning.} 
As data cleaning itself is an expensive process that usually needs human involvement eventually (e.g., to confirm suggested repairs), the DB community is starting to work on analytics-driven cleaning methods. SampleClean~\cite{DBLP:conf/sigmod/WangKFGKM14} targets the problem of answering SQL aggregate queries when the input data is dirty by cleaning a sample of the dirty dataset, and at the same time, providing statistical guarantees on the query results.
%%
ActiveClean~\cite{DBLP:journals/pvldb/KrishnanWWFG16} is an example of cleaning data intelligently for convex ML models that are trained using gradient descent methods.
%%
%The key insight of ActiveClean is that convex loss models (e.g., linear regression) can be trained and cleaned simultaneously using mini-batch gradient descent. %ActiveClean assumes that the cleaning is performed by a human oracle while CleanML evaluates automatic cleaning algorithms. 
As discussed before, while both ActiveClean and our proposal assume the use of a human cleaning oracle, they are incomparable as they are targeting different ML models. 
%%
BoostClean~\cite{krishnan2017boostclean} automatically selects from a predefined space of cleaning algorithms, using a hold-out validation set via statistical boosting. We show that our proposal significantly outperforms BoostClean under the same space of candidate repairs.
%as we identify the most promising tuple for humans to repair while BoostClean   
%It does show promising results in terms of increased prediction in some datasets. BoostClean only considered \textit{domain value violations} when an attribute value is outside of its value domain and only tested random forest model, while CleanML considers five error types and seven ML models. 
